A 12.4 day periodicity in a close binary system after a supernova

Neutron stars and stellar-mass black holes are the remnants of massive star explosions. Most massive stars reside in close binary systems, and the interplay between the companion star and the newly formed compact object has been theoretically explored, but signatures for binarity or evidence for the formation of a compact object during a supernova explosion are still lacking. Here we report a stripped-envelope supernova, SN 2022jli, which shows 12.4-day periodic undulations during the declining light curve. Narrow H$\alpha$ emission is detected in late-time spectra with concordant periodic velocity shifts, likely arising from hydrogen gas stripped from a companion and accreted onto the compact remnant. A new Fermi/LAT $\gamma$-ray source is temporally and positionally consistent with SN 2022jli. The observed properties of SN 2022jli, including periodic undulations in the optical light curve, coherent H$\alpha$ emission shifting, and evidence for association with a $\gamma$-ray source, point to the explosion of a massive star in a binary system leaving behind a bound compact remnant. Mass accretion from the companion star onto the compact object powers the light curve of the supernova and generates the $\gamma$-ray emission.

==> tables/sn2022jli_phot.tex <==
\begin{deluxetable}{cccc}
\tablecaption{SN\,2022jli photometry}
\tablehead{\colhead{Epoch} & \colhead{AB Magnitude} & \colhead{Source } & \colhead{Filter}
\\ (JD-2,459,700) &  & & }
\tabletypesize{\footnotesize}  %\small
\tablewidth{0pt}
\startdata
8.9154 & 15.366$\pm$0.053 & ASAS-SN & g \\
12.6611 & 15.386$\pm$0.053 & ASAS-SN & g \\
14.6775 & 15.602$\pm$0.171 & ASAS-SN & g \\
16.6692 & 15.737$\pm$0.120 & ASAS-SN & g \\
22.8739 & 15.477$\pm$0.060 & ASAS-SN & g \\
27.6503 & 16.140$\pm$0.113 & ASAS-SN & g \\
31.6665 & 16.245$\pm$0.078 & ASAS-SN & g \\
33.6136 & 16.092$\pm$0.063 & ASAS-SN & g \\
34.6683 & 16.324$\pm$0.125 & ASAS-SN & g \\
35.6096 & 16.005$\pm$0.082 & ASAS-SN & g \\
37.1042 & 15.920$\pm$0.072 & ASAS-SN & g \\
37.6023 & 15.944$\pm$0.066 & ASAS-SN & g \\
38.8515 & 15.774$\pm$0.051 & ASAS-SN & g \\
41.5805 & 15.720$\pm$0.053 & ASAS-SN & g \\
42.9147 & 15.482$\pm$0.039 & ASAS-SN & g \\
47.8300 & 15.275$\pm$0.047 & ASAS-SN & g \\
49.8793 & 15.202$\pm$0.049 & ASAS-SN & g \\
58.9335 & 15.217$\pm$0.035 & ASAS-SN & g \\
61.5420 & 15.384$\pm$0.038 & ASAS-SN & g \\
63.9554 & 15.147$\pm$0.055 & ASAS-SN & g \\
67.7761 & 15.290$\pm$0.041 & ASAS-SN & g \\
71.1037 & 15.251$\pm$0.030 & ASAS-SN & g \\
72.9429 & 15.298$\pm$0.040 & ASAS-SN & g \\
73.8081 & 15.232$\pm$0.070 & ASAS-SN & g \\
76.8817 & 15.208$\pm$0.067 & ASAS-SN & g \\
84.9872 & 15.464$\pm$0.040 & ASAS-SN & g \\
85.4616 & 15.573$\pm$0.051 & ASAS-SN & g \\
86.9723 & 15.413$\pm$0.114 & ASAS-SN & g \\
87.9420 & 15.574$\pm$0.064 & ASAS-SN & g \\
90.9718 & 15.528$\pm$0.042 & ASAS-SN & g \\
92.4687 & 15.772$\pm$0.054 & ASAS-SN & g \\
93.7074 & 15.795$\pm$0.056 & ASAS-SN & g \\
94.7136 & 15.651$\pm$0.046 & ASAS-SN & g \\
95.8213 & 15.631$\pm$0.045 & ASAS-SN & g \\
96.8122 & 15.546$\pm$0.045 & ASAS-SN & g \\
100.6916 & 15.424$\pm$0.080 & ASAS-SN & g \\
104.7242 & 15.722$\pm$0.126 & ASAS-SN & g \\
108.9435 & 15.668$\pm$0.064 & ASAS-SN & g \\
114.6117 & 15.856$\pm$0.064 & ASAS-SN & g \\
115.4898 & 15.957$\pm$0.063 & ASAS-SN & g \\
33.0868 & 15.751$\pm$0.013 & ATLAS & c \\
33.0953 & 15.696$\pm$0.011 & ATLAS & c \\
33.1092 & 15.707$\pm$0.013 & ATLAS & c \\
33.1134 & 15.718$\pm$0.017 & ATLAS & c \\
37.0850 & 15.568$\pm$0.011 & ATLAS & c \\
37.1016 & 15.540$\pm$0.011 & ATLAS & c \\
37.1044 & 15.529$\pm$0.010 & ATLAS & c \\
37.1150 & 15.579$\pm$0.018 & ATLAS & c \\
69.0885 & 15.091$\pm$0.007 & ATLAS & c \\
69.1067 & 15.087$\pm$0.008 & ATLAS & c \\
69.1158 & 15.089$\pm$0.010 & ATLAS & c \\
85.0699 & 15.314$\pm$0.008 & ATLAS & c \\
85.0731 & 15.314$\pm$0.008 & ATLAS & c \\
85.0785 & 15.292$\pm$0.008 & ATLAS & c \\
85.0971 & 15.300$\pm$0.008 & ATLAS & c \\
85.5648 & 15.323$\pm$0.008 & ATLAS & c \\
85.5676 & 15.310$\pm$0.008 & ATLAS & c \\
85.5744 & 15.330$\pm$0.008 & ATLAS & c \\
85.6048 & 15.297$\pm$0.008 & ATLAS & c \\
89.0577 & 15.439$\pm$0.009 & ATLAS & c \\
89.0605 & 15.435$\pm$0.009 & ATLAS & c \\
89.0636 & 15.430$\pm$0.009 & ATLAS & c \\
89.0700 & 15.405$\pm$0.009 & ATLAS & c \\
91.8706 & 15.480$\pm$0.010 & ATLAS & c \\
91.8738 & 15.471$\pm$0.009 & ATLAS & c \\
91.9022 & 15.488$\pm$0.009 & ATLAS & c \\
91.9082 & 15.486$\pm$0.009 & ATLAS & c \\
91.9406 & 15.512$\pm$0.014 & ATLAS & c \\
93.0941 & 15.563$\pm$0.009 & ATLAS & c \\
93.0969 & 15.531$\pm$0.009 & ATLAS & c \\
93.1204 & 15.509$\pm$0.010 & ATLAS & c \\
93.1248 & 15.533$\pm$0.010 & ATLAS & c \\
97.1056 & 15.437$\pm$0.009 & ATLAS & c \\
97.1120 & 15.434$\pm$0.009 & ATLAS & c \\
97.1246 & 15.445$\pm$0.011 & ATLAS & c \\
97.1279 & 15.417$\pm$0.013 & ATLAS & c \\
97.5938 & 15.440$\pm$0.008 & ATLAS & c \\
97.5981 & 15.461$\pm$0.009 & ATLAS & c \\
97.6037 & 15.470$\pm$0.009 & ATLAS & c \\
97.6138 & 15.444$\pm$0.010 & ATLAS & c \\
97.6847 & 15.483$\pm$0.011 & ATLAS & c \\
119.6638 & 15.787$\pm$0.012 & ATLAS & c \\
119.6841 & 15.844$\pm$0.011 & ATLAS & c \\
119.7103 & 15.816$\pm$0.011 & ATLAS & c \\
119.7198 & 15.829$\pm$0.011 & ATLAS & c \\
121.0059 & 15.760$\pm$0.011 & ATLAS & c \\
121.0091 & 15.794$\pm$0.012 & ATLAS & c \\
121.0192 & 15.800$\pm$0.011 & ATLAS & c \\
121.0446 & 15.764$\pm$0.011 & ATLAS & c \\
123.7967 & 15.765$\pm$0.012 & ATLAS & c \\
123.7999 & 15.775$\pm$0.011 & ATLAS & c \\
123.8265 & 15.797$\pm$0.011 & ATLAS & c \\
123.8296 & 15.888$\pm$0.015 & ATLAS & c \\
123.8328 & 15.777$\pm$0.013 & ATLAS & c \\
123.8332 & 15.847$\pm$0.016 & ATLAS & c \\
125.0551 & 15.846$\pm$0.010 & ATLAS & c \\
125.0894 & 15.838$\pm$0.011 & ATLAS & c \\
125.1179 & 15.851$\pm$0.011 & ATLAS & c \\
142.9205 & 16.122$\pm$0.016 & ATLAS & c \\
142.9223 & 16.123$\pm$0.017 & ATLAS & c \\
142.9251 & 16.103$\pm$0.015 & ATLAS & c \\
142.9302 & 16.115$\pm$0.015 & ATLAS & c \\
147.0465 & 16.125$\pm$0.113 & ATLAS & c \\
147.0530 & 15.792$\pm$0.078 & ATLAS & c \\
149.5328 & 16.017$\pm$0.014 & ATLAS & c \\
149.5360 & 16.035$\pm$0.012 & ATLAS & c \\
149.5419 & 16.028$\pm$0.012 & ATLAS & c \\
149.5657 & 16.060$\pm$0.013 & ATLAS & c \\
150.9071 & 16.138$\pm$0.014 & ATLAS & c \\
150.9089 & 16.084$\pm$0.012 & ATLAS & c \\
150.9136 & 16.128$\pm$0.013 & ATLAS & c \\
150.9187 & 16.105$\pm$0.013 & ATLAS & c \\
153.4085 & 16.130$\pm$0.013 & ATLAS & c \\
153.4103 & 16.105$\pm$0.013 & ATLAS & c \\
153.4121 & 16.095$\pm$0.013 & ATLAS & c \\
153.4135 & 16.057$\pm$0.013 & ATLAS & c \\
153.4230 & 16.135$\pm$0.014 & ATLAS & c \\
153.4326 & 16.153$\pm$0.013 & ATLAS & c \\
154.9848 & 16.245$\pm$0.014 & ATLAS & c \\
154.9947 & 16.217$\pm$0.015 & ATLAS & c \\
155.0229 & 16.193$\pm$0.014 & ATLAS & c \\
155.0325 & 16.191$\pm$0.015 & ATLAS & c \\
171.6838 & 16.342$\pm$0.018 & ATLAS & c \\
171.6893 & 16.250$\pm$0.016 & ATLAS & c \\
171.7198 & 16.235$\pm$0.015 & ATLAS & c \\
171.7229 & 16.268$\pm$0.017 & ATLAS & c \\
172.8815 & 16.281$\pm$0.016 & ATLAS & c \\
172.9161 & 16.255$\pm$0.016 & ATLAS & c \\
172.9193 & 16.243$\pm$0.016 & ATLAS & c \\
172.9293 & 16.280$\pm$0.015 & ATLAS & c \\
175.6624 & 16.313$\pm$0.015 & ATLAS & c \\
175.6665 & 16.324$\pm$0.016 & ATLAS & c \\
175.6918 & 16.320$\pm$0.014 & ATLAS & c \\
175.6973 & 16.320$\pm$0.017 & ATLAS & c \\
176.8836 & 16.410$\pm$0.017 & ATLAS & c \\
176.8868 & 16.347$\pm$0.016 & ATLAS & c \\
176.8927 & 16.376$\pm$0.016 & ATLAS & c \\
176.9028 & 16.344$\pm$0.018 & ATLAS & c \\
179.6305 & 16.374$\pm$0.017 & ATLAS & c \\
179.6638 & 16.429$\pm$0.017 & ATLAS & c \\
179.6670 & 16.407$\pm$0.016 & ATLAS & c \\
179.6724 & 16.413$\pm$0.016 & ATLAS & c \\
180.9260 & 16.408$\pm$0.017 & ATLAS & c \\
180.9296 & 16.453$\pm$0.017 & ATLAS & c \\
180.9359 & 16.448$\pm$0.019 & ATLAS & c \\
180.9605 & 16.494$\pm$0.020 & ATLAS & c \\
197.3426 & 16.554$\pm$0.022 & ATLAS & c \\
197.3453 & 16.589$\pm$0.021 & ATLAS & c \\
197.3512 & 16.558$\pm$0.019 & ATLAS & c \\
197.3611 & 16.567$\pm$0.019 & ATLAS & c \\
198.8420 & 16.632$\pm$0.020 & ATLAS & c \\
198.8531 & 16.629$\pm$0.019 & ATLAS & c \\
198.8578 & 16.608$\pm$0.020 & ATLAS & c \\
198.8690 & 16.607$\pm$0.020 & ATLAS & c \\
201.3322 & 16.625$\pm$0.021 & ATLAS & c \\
201.3354 & 16.675$\pm$0.025 & ATLAS & c \\
201.3426 & 16.597$\pm$0.026 & ATLAS & c \\
201.3526 & 16.668$\pm$0.026 & ATLAS & c \\
202.8783 & 16.752$\pm$0.022 & ATLAS & c \\
202.9049 & 16.700$\pm$0.021 & ATLAS & c \\
202.9184 & 16.717$\pm$0.022 & ATLAS & c \\
205.3154 & 16.787$\pm$0.044 & ATLAS & c \\
205.3195 & 16.873$\pm$0.033 & ATLAS & c \\
205.3263 & 16.786$\pm$0.039 & ATLAS & c \\
206.8016 & 16.865$\pm$0.023 & ATLAS & c \\
206.8044 & 16.900$\pm$0.023 & ATLAS & c \\
206.8142 & 16.901$\pm$0.021 & ATLAS & c \\
206.8245 & 16.800$\pm$0.022 & ATLAS & c \\
227.5653 & 16.989$\pm$0.025 & ATLAS & c \\
227.5689 & 17.031$\pm$0.028 & ATLAS & c \\
227.5740 & 17.037$\pm$0.029 & ATLAS & c \\
227.5860 & 16.977$\pm$0.139 & ATLAS & c \\
228.7701 & 17.016$\pm$0.026 & ATLAS & c \\
228.7742 & 16.991$\pm$0.029 & ATLAS & c \\
228.7875 & 17.047$\pm$0.029 & ATLAS & c \\
228.7947 & 17.058$\pm$0.028 & ATLAS & c \\
231.5376 & 17.112$\pm$0.039 & ATLAS & c \\
231.5408 & 17.108$\pm$0.038 & ATLAS & c \\
231.5462 & 17.072$\pm$0.037 & ATLAS & c \\
231.5611 & 17.016$\pm$0.027 & ATLAS & c \\
264.3062 & 17.009$\pm$0.062 & ATLAS & c \\
25.6585 & 14.786$\pm$0.007 & ATLAS & o \\
25.6657 & 14.775$\pm$0.007 & ATLAS & o \\
25.6826 & 14.796$\pm$0.012 & ATLAS & o \\
37.6553 & 14.867$\pm$0.007 & ATLAS & o \\
37.6739 & 14.861$\pm$0.008 & ATLAS & o \\
37.6854 & 14.882$\pm$0.015 & ATLAS & o \\
45.0839 & 14.578$\pm$0.009 & ATLAS & o \\
45.0959 & 14.517$\pm$0.009 & ATLAS & o \\
45.1065 & 14.563$\pm$0.008 & ATLAS & o \\
45.1101 & 14.538$\pm$0.008 & ATLAS & o \\
47.0924 & 14.489$\pm$0.009 & ATLAS & o \\
47.0965 & 14.520$\pm$0.009 & ATLAS & o \\
47.1034 & 14.494$\pm$0.008 & ATLAS & o \\
47.1159 & 14.496$\pm$0.019 & ATLAS & o \\
54.0836 & 14.482$\pm$0.005 & ATLAS & o \\
54.0868 & 14.464$\pm$0.006 & ATLAS & o \\
54.0966 & 14.463$\pm$0.005 & ATLAS & o \\
54.1023 & 14.454$\pm$0.005 & ATLAS & o \\
55.0878 & 14.434$\pm$0.006 & ATLAS & o \\
55.0925 & 14.483$\pm$0.006 & ATLAS & o \\
55.1004 & 14.475$\pm$0.006 & ATLAS & o \\
55.1018 & 14.464$\pm$0.006 & ATLAS & o \\
55.1105 & 14.455$\pm$0.006 & ATLAS & o \\
55.1119 & 14.427$\pm$0.006 & ATLAS & o \\
55.1183 & 14.481$\pm$0.009 & ATLAS & o \\
55.1197 & 14.467$\pm$0.011 & ATLAS & o \\
67.0909 & 14.630$\pm$0.006 & ATLAS & o \\
67.1128 & 14.646$\pm$0.008 & ATLAS & o \\
67.1160 & 14.631$\pm$0.010 & ATLAS & o \\
67.1203 & 14.640$\pm$0.011 & ATLAS & o \\
69.6153 & 14.702$\pm$0.006 & ATLAS & o \\
69.6255 & 14.684$\pm$0.007 & ATLAS & o \\
69.6403 & 14.707$\pm$0.006 & ATLAS & o \\
69.6452 & 14.698$\pm$0.007 & ATLAS & o \\
71.0865 & 14.703$\pm$0.006 & ATLAS & o \\
71.1066 & 14.714$\pm$0.006 & ATLAS & o \\
71.1108 & 14.711$\pm$0.007 & ATLAS & o \\
71.1202 & 14.734$\pm$0.009 & ATLAS & o \\
73.0627 & 14.678$\pm$0.007 & ATLAS & o \\
73.0659 & 14.700$\pm$0.007 & ATLAS & o \\
73.0722 & 14.666$\pm$0.006 & ATLAS & o \\
73.0854 & 14.688$\pm$0.006 & ATLAS & o \\
73.5924 & 14.685$\pm$0.008 & ATLAS & o \\
73.5956 & 14.675$\pm$0.007 & ATLAS & o \\
73.6005 & 14.689$\pm$0.010 & ATLAS & o \\
73.6073 & 14.678$\pm$0.008 & ATLAS & o \\
75.0325 & 14.748$\pm$0.010 & ATLAS & o \\
75.0387 & 14.764$\pm$0.009 & ATLAS & o \\
75.0424 & 14.749$\pm$0.009 & ATLAS & o \\
75.0529 & 14.750$\pm$0.009 & ATLAS & o \\
76.4888 & 14.671$\pm$0.053 & ATLAS & o \\
76.4920 & 14.759$\pm$0.015 & ATLAS & o \\
76.4979 & 14.803$\pm$0.013 & ATLAS & o \\
76.5165 & 14.762$\pm$0.009 & ATLAS & o \\
77.5088 & 14.747$\pm$0.013 & ATLAS & o \\
77.5115 & 14.797$\pm$0.012 & ATLAS & o \\
77.5260 & 14.781$\pm$0.012 & ATLAS & o \\
77.5319 & 14.804$\pm$0.011 & ATLAS & o \\
81.6077 & 14.961$\pm$0.007 & ATLAS & o \\
81.6106 & 14.955$\pm$0.007 & ATLAS & o \\
81.6161 & 14.972$\pm$0.007 & ATLAS & o \\
81.6329 & 14.957$\pm$0.008 & ATLAS & o \\
83.8146 & 14.945$\pm$0.007 & ATLAS & o \\
83.8197 & 14.952$\pm$0.007 & ATLAS & o \\
83.8234 & 14.933$\pm$0.007 & ATLAS & o \\
83.8346 & 14.943$\pm$0.007 & ATLAS & o \\
87.0694 & 15.028$\pm$0.008 & ATLAS & o \\
87.0726 & 15.028$\pm$0.008 & ATLAS & o \\
87.0771 & 15.055$\pm$0.008 & ATLAS & o \\
87.0906 & 15.036$\pm$0.008 & ATLAS & o \\
87.8822 & 15.036$\pm$0.007 & ATLAS & o \\
87.8859 & 15.040$\pm$0.007 & ATLAS & o \\
87.8927 & 15.021$\pm$0.007 & ATLAS & o \\
95.1028 & 15.240$\pm$0.009 & ATLAS & o \\
95.1075 & 15.229$\pm$0.009 & ATLAS & o \\
95.1150 & 15.234$\pm$0.010 & ATLAS & o \\
95.1228 & 15.237$\pm$0.010 & ATLAS & o \\
99.7597 & 15.149$\pm$0.012 & ATLAS & o \\
99.7624 & 15.161$\pm$0.012 & ATLAS & o \\
99.7784 & 15.151$\pm$0.010 & ATLAS & o \\
99.7839 & 15.167$\pm$0.009 & ATLAS & o \\
101.0257 & 15.200$\pm$0.009 & ATLAS & o \\
101.0276 & 15.183$\pm$0.009 & ATLAS & o \\
101.0303 & 15.168$\pm$0.009 & ATLAS & o \\
101.0479 & 15.098$\pm$0.008 & ATLAS & o \\
101.5057 & 15.189$\pm$0.009 & ATLAS & o \\
101.5094 & 15.175$\pm$0.009 & ATLAS & o \\
101.5158 & 15.193$\pm$0.009 & ATLAS & o \\
101.5256 & 15.174$\pm$0.009 & ATLAS & o \\
101.7828 & 15.201$\pm$0.014 & ATLAS & o \\
101.7855 & 15.192$\pm$0.011 & ATLAS & o \\
101.8135 & 15.239$\pm$0.027 & ATLAS & o \\
101.8177 & 15.159$\pm$0.016 & ATLAS & o \\
102.6790 & 15.171$\pm$0.014 & ATLAS & o \\
102.6822 & 15.177$\pm$0.014 & ATLAS & o \\
102.6883 & 15.188$\pm$0.013 & ATLAS & o \\
102.7083 & 15.133$\pm$0.023 & ATLAS & o \\
103.0076 & 15.275$\pm$0.049 & ATLAS & o \\
103.0308 & 15.283$\pm$0.044 & ATLAS & o \\
103.0326 & 15.283$\pm$0.042 & ATLAS & o \\
103.0399 & 15.309$\pm$0.061 & ATLAS & o \\
103.7153 & 15.227$\pm$0.043 & ATLAS & o \\
109.0615 & 15.273$\pm$0.009 & ATLAS & o \\
109.0667 & 15.270$\pm$0.010 & ATLAS & o \\
109.1021 & 15.289$\pm$0.010 & ATLAS & o \\
109.1265 & 15.292$\pm$0.009 & ATLAS & o \\
110.9747 & 15.326$\pm$0.010 & ATLAS & o \\
110.9811 & 15.351$\pm$0.011 & ATLAS & o \\
110.9867 & 15.337$\pm$0.011 & ATLAS & o \\
110.9917 & 15.350$\pm$0.010 & ATLAS & o \\
113.0424 & 15.366$\pm$0.011 & ATLAS & o \\
113.0478 & 15.371$\pm$0.010 & ATLAS & o \\
113.0831 & 15.368$\pm$0.009 & ATLAS & o \\
113.0863 & 15.381$\pm$0.009 & ATLAS & o \\
113.5482 & 15.383$\pm$0.009 & ATLAS & o \\
113.5514 & 15.370$\pm$0.009 & ATLAS & o \\
113.5843 & 15.364$\pm$0.009 & ATLAS & o \\
113.5898 & 15.397$\pm$0.011 & ATLAS & o \\
115.0114 & 15.483$\pm$0.012 & ATLAS & o \\
115.0133 & 15.479$\pm$0.012 & ATLAS & o \\
115.0188 & 15.506$\pm$0.012 & ATLAS & o \\
115.0545 & 15.478$\pm$0.011 & ATLAS & o \\
118.9947 & 15.593$\pm$0.011 & ATLAS & o \\
118.9989 & 15.595$\pm$0.011 & ATLAS & o \\
119.0016 & 15.599$\pm$0.012 & ATLAS & o \\
119.0236 & 15.601$\pm$0.011 & ATLAS & o \\
123.0329 & 15.561$\pm$0.011 & ATLAS & o \\
123.0370 & 15.574$\pm$0.011 & ATLAS & o \\
123.0644 & 15.557$\pm$0.012 & ATLAS & o \\
123.0927 & 15.538$\pm$0.012 & ATLAS & o \\
125.4809 & 15.575$\pm$0.010 & ATLAS & o \\
125.4828 & 15.602$\pm$0.010 & ATLAS & o \\
125.4859 & 15.611$\pm$0.010 & ATLAS & o \\
125.5041 & 15.608$\pm$0.011 & ATLAS & o \\
126.9583 & 15.650$\pm$0.011 & ATLAS & o \\
126.9601 & 15.680$\pm$0.011 & ATLAS & o \\
126.9832 & 15.639$\pm$0.013 & ATLAS & o \\
126.9873 & 15.651$\pm$0.012 & ATLAS & o \\
129.4461 & 15.727$\pm$0.012 & ATLAS & o \\
129.4516 & 15.716$\pm$0.013 & ATLAS & o \\
129.4557 & 15.722$\pm$0.013 & ATLAS & o \\
129.4611 & 15.698$\pm$0.013 & ATLAS & o \\
129.6241 & 15.793$\pm$0.021 & ATLAS & o \\
130.8904 & 15.821$\pm$0.020 & ATLAS & o \\
130.8936 & 15.767$\pm$0.020 & ATLAS & o \\
130.9168 & 15.834$\pm$0.021 & ATLAS & o \\
130.9209 & 15.594$\pm$0.107 & ATLAS & o \\
131.5102 & 15.769$\pm$0.019 & ATLAS & o \\
131.5159 & 15.809$\pm$0.021 & ATLAS & o \\
131.5497 & 15.772$\pm$0.019 & ATLAS & o \\
131.5527 & 15.789$\pm$0.021 & ATLAS & o \\
137.0675 & 15.753$\pm$0.016 & ATLAS & o \\
137.0710 & 15.750$\pm$0.016 & ATLAS & o \\
137.0764 & 15.766$\pm$0.015 & ATLAS & o \\
137.0873 & 15.722$\pm$0.014 & ATLAS & o \\
137.4984 & 15.734$\pm$0.015 & ATLAS & o \\
137.5039 & 15.755$\pm$0.017 & ATLAS & o \\
137.5071 & 15.742$\pm$0.018 & ATLAS & o \\
137.5175 & 15.801$\pm$0.017 & ATLAS & o \\
138.9782 & 15.788$\pm$0.012 & ATLAS & o \\
138.9810 & 15.776$\pm$0.013 & ATLAS & o \\
138.9864 & 15.790$\pm$0.012 & ATLAS & o \\
139.0217 & 15.800$\pm$0.013 & ATLAS & o \\
139.7343 & 15.551$\pm$0.178 & ATLAS & o \\
139.7700 & 15.865$\pm$0.140 & ATLAS & o \\
139.7731 & 15.836$\pm$0.116 & ATLAS & o \\
139.7785 & 15.527$\pm$0.151 & ATLAS & o \\
140.9697 & 15.832$\pm$0.013 & ATLAS & o \\
140.9729 & 15.840$\pm$0.013 & ATLAS & o \\
140.9783 & 15.834$\pm$0.014 & ATLAS & o \\
140.9886 & 15.808$\pm$0.011 & ATLAS & o \\
143.6578 & 15.873$\pm$0.013 & ATLAS & o \\
143.6605 & 15.895$\pm$0.013 & ATLAS & o \\
143.6660 & 15.914$\pm$0.012 & ATLAS & o \\
143.6758 & 15.897$\pm$0.013 & ATLAS & o \\
144.9129 & 15.903$\pm$0.014 & ATLAS & o \\
144.9147 & 15.916$\pm$0.013 & ATLAS & o \\
144.9365 & 15.916$\pm$0.014 & ATLAS & o \\
144.9419 & 15.888$\pm$0.015 & ATLAS & o \\
148.9169 & 15.828$\pm$0.014 & ATLAS & o \\
148.9187 & 15.819$\pm$0.012 & ATLAS & o \\
148.9219 & 15.833$\pm$0.013 & ATLAS & o \\
148.9425 & 15.815$\pm$0.014 & ATLAS & o \\
151.6519 & 15.867$\pm$0.011 & ATLAS & o \\
151.6546 & 15.855$\pm$0.012 & ATLAS & o \\
151.6600 & 15.868$\pm$0.015 & ATLAS & o \\
151.6822 & 15.884$\pm$0.015 & ATLAS & o \\
155.7303 & 15.984$\pm$0.014 & ATLAS & o \\
155.7334 & 15.947$\pm$0.015 & ATLAS & o \\
155.7683 & 15.816$\pm$0.014 & ATLAS & o \\
155.7966 & 16.010$\pm$0.015 & ATLAS & o \\
156.3734 & 16.037$\pm$0.095 & ATLAS & o \\
156.3757 & 15.966$\pm$0.077 & ATLAS & o \\
156.3940 & 16.020$\pm$0.036 & ATLAS & o \\
156.3990 & 16.050$\pm$0.036 & ATLAS & o \\
157.3689 & 16.023$\pm$0.020 & ATLAS & o \\
157.3707 & 16.096$\pm$0.021 & ATLAS & o \\
157.3748 & 16.016$\pm$0.017 & ATLAS & o \\
157.3802 & 16.032$\pm$0.018 & ATLAS & o \\
158.6099 & 15.939$\pm$0.021 & ATLAS & o \\
158.6126 & 15.969$\pm$0.021 & ATLAS & o \\
158.6331 & 15.935$\pm$0.018 & ATLAS & o \\
158.6512 & 15.966$\pm$0.021 & ATLAS & o \\
158.9364 & 15.917$\pm$0.015 & ATLAS & o \\
158.9396 & 15.941$\pm$0.016 & ATLAS & o \\
158.9672 & 15.957$\pm$0.018 & ATLAS & o \\
158.9753 & 15.968$\pm$0.021 & ATLAS & o \\
164.9132 & 16.105$\pm$0.024 & ATLAS & o \\
164.9164 & 16.018$\pm$0.018 & ATLAS & o \\
164.9223 & 16.090$\pm$0.018 & ATLAS & o \\
164.9259 & 16.092$\pm$0.022 & ATLAS & o \\
164.9291 & 16.077$\pm$0.019 & ATLAS & o \\
164.9322 & 16.038$\pm$0.020 & ATLAS & o \\
164.9350 & 16.032$\pm$0.065 & ATLAS & o \\
166.9250 & 16.125$\pm$0.022 & ATLAS & o \\
166.9282 & 16.129$\pm$0.022 & ATLAS & o \\
166.9338 & 16.167$\pm$0.021 & ATLAS & o \\
166.9442 & 16.178$\pm$0.063 & ATLAS & o \\
168.9019 & 16.197$\pm$0.018 & ATLAS & o \\
168.9051 & 16.197$\pm$0.017 & ATLAS & o \\
168.9110 & 16.200$\pm$0.018 & ATLAS & o \\
168.9251 & 16.189$\pm$0.017 & ATLAS & o \\
170.8890 & 16.122$\pm$0.013 & ATLAS & o \\
170.8919 & 16.075$\pm$0.015 & ATLAS & o \\
170.8970 & 16.128$\pm$0.013 & ATLAS & o \\
170.9314 & 16.108$\pm$0.016 & ATLAS & o \\
173.3867 & 16.096$\pm$0.018 & ATLAS & o \\
173.3899 & 16.086$\pm$0.017 & ATLAS & o \\
173.3958 & 16.112$\pm$0.016 & ATLAS & o \\
173.4308 & 16.160$\pm$0.044 & ATLAS & o \\
174.9445 & 16.139$\pm$0.014 & ATLAS & o \\
174.9501 & 16.155$\pm$0.015 & ATLAS & o \\
174.9528 & 16.162$\pm$0.015 & ATLAS & o \\
174.9635 & 16.143$\pm$0.015 & ATLAS & o \\
177.3812 & 16.172$\pm$0.017 & ATLAS & o \\
177.3848 & 16.225$\pm$0.015 & ATLAS & o \\
177.3903 & 16.188$\pm$0.016 & ATLAS & o \\
177.4252 & 16.270$\pm$0.033 & ATLAS & o \\
178.8659 & 16.290$\pm$0.019 & ATLAS & o \\
178.8691 & 16.289$\pm$0.019 & ATLAS & o \\
178.8747 & 16.301$\pm$0.018 & ATLAS & o \\
178.8873 & 16.264$\pm$0.019 & ATLAS & o \\
181.2474 & 16.322$\pm$0.024 & ATLAS & o \\
181.2497 & 16.333$\pm$0.023 & ATLAS & o \\
181.2501 & 16.345$\pm$0.019 & ATLAS & o \\
181.2506 & 16.347$\pm$0.019 & ATLAS & o \\
181.2510 & 16.228$\pm$0.020 & ATLAS & o \\
181.2519 & 16.327$\pm$0.021 & ATLAS & o \\
181.2537 & 16.308$\pm$0.019 & ATLAS & o \\
181.2569 & 16.360$\pm$0.018 & ATLAS & o \\
181.2623 & 16.308$\pm$0.024 & ATLAS & o \\
182.8641 & 16.323$\pm$0.019 & ATLAS & o \\
182.8673 & 16.299$\pm$0.018 & ATLAS & o \\
182.8733 & 16.279$\pm$0.018 & ATLAS & o \\
182.8840 & 16.305$\pm$0.016 & ATLAS & o \\
183.6219 & 16.189$\pm$0.021 & ATLAS & o \\
183.6250 & 15.962$\pm$0.020 & ATLAS & o \\
183.6304 & 16.106$\pm$0.020 & ATLAS & o \\
183.6408 & 15.922$\pm$0.019 & ATLAS & o \\
184.8776 & 16.256$\pm$0.018 & ATLAS & o \\
184.8808 & 16.250$\pm$0.020 & ATLAS & o \\
184.8862 & 16.230$\pm$0.020 & ATLAS & o \\
184.8968 & 16.243$\pm$0.018 & ATLAS & o \\
184.9164 & 16.278$\pm$0.018 & ATLAS & o \\
185.3571 & 16.260$\pm$0.023 & ATLAS & o \\
186.8482 & 16.276$\pm$0.022 & ATLAS & o \\
186.8509 & 16.354$\pm$0.025 & ATLAS & o \\
186.8712 & 16.284$\pm$0.023 & ATLAS & o \\
186.8847 & 16.325$\pm$0.030 & ATLAS & o \\
191.6693 & 16.312$\pm$0.072 & ATLAS & o \\
192.9275 & 16.518$\pm$0.033 & ATLAS & o \\
192.9307 & 16.536$\pm$0.035 & ATLAS & o \\
192.9512 & 16.453$\pm$0.032 & ATLAS & o \\
192.9576 & 16.481$\pm$0.039 & ATLAS & o \\
193.4410 & 16.598$\pm$0.044 & ATLAS & o \\
193.4590 & 16.452$\pm$0.039 & ATLAS & o \\
193.4637 & 16.534$\pm$0.036 & ATLAS & o \\
193.4734 & 16.508$\pm$0.040 & ATLAS & o \\
194.8146 & 16.524$\pm$0.021 & ATLAS & o \\
194.8178 & 16.510$\pm$0.026 & ATLAS & o \\
194.8243 & 16.525$\pm$0.025 & ATLAS & o \\
194.8354 & 16.513$\pm$0.026 & ATLAS & o \\
196.9071 & 16.410$\pm$0.024 & ATLAS & o \\
196.9340 & 16.115$\pm$0.017 & ATLAS & o \\
196.9358 & 16.451$\pm$0.029 & ATLAS & o \\
196.9390 & 16.432$\pm$0.025 & ATLAS & o \\
199.6017 & 16.511$\pm$0.019 & ATLAS & o \\
199.6045 & 16.551$\pm$0.019 & ATLAS & o \\
199.6109 & 16.526$\pm$0.021 & ATLAS & o \\
199.6258 & 16.501$\pm$0.016 & ATLAS & o \\
200.8926 & 16.569$\pm$0.024 & ATLAS & o \\
200.9607 & 16.558$\pm$0.026 & ATLAS & o \\
200.9866 & 16.551$\pm$0.035 & ATLAS & o \\
203.5876 & 16.643$\pm$0.020 & ATLAS & o \\
203.5908 & 16.609$\pm$0.023 & ATLAS & o \\
203.5980 & 16.580$\pm$0.020 & ATLAS & o \\
203.6080 & 16.612$\pm$0.023 & ATLAS & o \\
207.5712 & 16.618$\pm$0.024 & ATLAS & o \\
207.5748 & 16.724$\pm$0.030 & ATLAS & o \\
207.5820 & 16.764$\pm$0.045 & ATLAS & o \\
207.5919 & 16.992$\pm$0.401 & ATLAS & o \\
208.8025 & 16.563$\pm$0.023 & ATLAS & o \\
208.8056 & 16.547$\pm$0.025 & ATLAS & o \\
208.8120 & 16.502$\pm$0.020 & ATLAS & o \\
208.8218 & 16.574$\pm$0.022 & ATLAS & o \\
209.6382 & 16.614$\pm$0.025 & ATLAS & o \\
209.6736 & 16.602$\pm$0.024 & ATLAS & o \\
209.6740 & 16.589$\pm$0.023 & ATLAS & o \\
209.6745 & 16.628$\pm$0.023 & ATLAS & o \\
209.6749 & 16.615$\pm$0.023 & ATLAS & o \\
211.5654 & 16.664$\pm$0.028 & ATLAS & o \\
211.5686 & 16.650$\pm$0.028 & ATLAS & o \\
211.5758 & 16.596$\pm$0.033 & ATLAS & o \\
211.5857 & 16.714$\pm$0.026 & ATLAS & o \\
213.2925 & 16.697$\pm$0.031 & ATLAS & o \\
213.2965 & 16.673$\pm$0.032 & ATLAS & o \\
213.3019 & 16.671$\pm$0.032 & ATLAS & o \\
213.3120 & 16.684$\pm$0.026 & ATLAS & o \\
219.5960 & 16.794$\pm$0.044 & ATLAS & o \\
219.5996 & 16.848$\pm$0.048 & ATLAS & o \\
219.6055 & 16.843$\pm$0.054 & ATLAS & o \\
219.6181 & 16.844$\pm$0.046 & ATLAS & o \\
221.3134 & 16.724$\pm$0.044 & ATLAS & o \\
221.3170 & 16.663$\pm$0.044 & ATLAS & o \\
221.3242 & 16.681$\pm$0.045 & ATLAS & o \\
221.3410 & 16.668$\pm$0.040 & ATLAS & o \\
223.5676 & 16.810$\pm$0.109 & ATLAS & o \\
223.5712 & 16.751$\pm$0.035 & ATLAS & o \\
223.5770 & 16.770$\pm$0.029 & ATLAS & o \\
223.5906 & 16.725$\pm$0.133 & ATLAS & o \\
245.2854 & 17.049$\pm$0.137 & ATLAS & o \\
245.2881 & 17.200$\pm$0.117 & ATLAS & o \\
245.2974 & 16.975$\pm$0.055 & ATLAS & o \\
247.5361 & 16.976$\pm$0.146 & ATLAS & o \\
247.5628 & 16.941$\pm$0.061 & ATLAS & o \\
249.3360 & 16.960$\pm$0.056 & ATLAS & o \\
249.3402 & 16.998$\pm$0.059 & ATLAS & o \\
249.3461 & 17.058$\pm$0.082 & ATLAS & o \\
249.3689 & 16.985$\pm$0.076 & ATLAS & o \\
260.7094 & 17.035$\pm$0.041 & ATLAS & o \\
260.7126 & 16.956$\pm$0.037 & ATLAS & o \\
260.7371 & 17.011$\pm$0.030 & ATLAS & o \\
264.7094 & 16.971$\pm$0.051 & ATLAS & o \\
67.9500 & 14.790$\pm$0.038 & P60 & r \\
79.9797 & 15.077$\pm$0.041 & P60 & r \\
86.8618 & 15.146$\pm$0.041 & P60 & r \\
95.9420 & 15.311$\pm$0.043 & P60 & r \\
102.8366 & 15.355$\pm$0.043 & P60 & r \\
107.8148 & 15.420$\pm$0.045 & P60 & r \\
109.8508 & 15.388$\pm$0.044 & P60 & r \\
114.8975 & 15.533$\pm$0.045 & P60 & r \\
119.7803 & 15.714$\pm$0.048 & P60 & r \\
130.7369 & 15.902$\pm$0.052 & P60 & r \\
138.7395 & 15.845$\pm$0.049 & P60 & r \\
143.8109 & 16.049$\pm$0.053 & P60 & r \\
153.8218 & 16.110$\pm$0.053 & P60 & r \\
154.8271 & 16.103$\pm$0.053 & P60 & r \\
157.6710 & 16.096$\pm$0.054 & P60 & r \\
163.6823 & 16.168$\pm$0.055 & P60 & r \\
166.7223 & 16.255$\pm$0.057 & P60 & r \\
173.7022 & 16.224$\pm$0.056 & P60 & r \\
182.8610 & 16.458$\pm$0.060 & P60 & r \\
198.6567 & 16.561$\pm$0.064 & P60 & r \\
210.6018 & 16.710$\pm$0.066 & P60 & r \\
224.6424 & 16.883$\pm$0.071 & P60 & r \\
233.6219 & 16.910$\pm$0.072 & P60 & r \\
257.6957 & 17.360$\pm$0.099 & P60 & r \\
272.6043 & 17.840$\pm$0.104 & P60 & r \\
273.6053 & 18.010$\pm$0.114 & P60 & r \\
283.6109 & 18.520$\pm$0.153 & P60 & r \\
285.6121 & 19.400$\pm$0.321 & P60 & r \\
67.9520 & 14.660$\pm$0.038 & P60 & i \\
79.9817 & 14.964$\pm$0.040 & P60 & i \\
86.8635 & 15.096$\pm$0.041 & P60 & i \\
95.9436 & 15.280$\pm$0.042 & P60 & i \\
102.8386 & 15.322$\pm$0.043 & P60 & i \\
107.8168 & 15.315$\pm$0.043 & P60 & i \\
109.8528 & 15.352$\pm$0.043 & P60 & i \\
114.8995 & 15.264$\pm$0.042 & P60 & i \\
119.7823 & 15.689$\pm$0.048 & P60 & i \\
130.7389 & 15.886$\pm$0.052 & P60 & i \\
138.7412 & 15.847$\pm$0.049 & P60 & i \\
143.8142 & 16.019$\pm$0.052 & P60 & i \\
153.8272 & 16.090$\pm$0.053 & P60 & i \\
154.8327 & 16.062$\pm$0.052 & P60 & i \\
157.6744 & 15.874$\pm$0.051 & P60 & i \\
163.6839 & 16.140$\pm$0.054 & P60 & i \\
166.7240 & 16.194$\pm$0.055 & P60 & i \\
173.7039 & 16.181$\pm$0.055 & P60 & i \\
174.8971 & 16.035$\pm$0.052 & P60 & i \\
182.8626 & 16.231$\pm$0.056 & P60 & i \\
198.6584 & 16.529$\pm$0.062 & P60 & i \\
210.6035 & 16.685$\pm$0.065 & P60 & i \\
224.6441 & 16.682$\pm$0.066 & P60 & i \\
233.6235 & 16.953$\pm$0.072 & P60 & i \\
257.6206 & 17.208$\pm$0.087 & P60 & i \\
272.6097 & 17.936$\pm$0.108 & P60 & i \\
283.6178 & 18.825$\pm$0.164 & P60 & i \\
57.9530 & 15.244$\pm$0.024 & ZTF & g \\
57.9530 & 15.244$\pm$0.024 & ZTF & g \\
57.9540 & 15.220$\pm$0.029 & ZTF & g \\
57.9540 & 15.220$\pm$0.029 & ZTF & g \\
57.9540 & 15.220$\pm$0.029 & ZTF & g \\
63.9591 & 15.260$\pm$0.026 & ZTF & g \\
63.9591 & 15.260$\pm$0.026 & ZTF & g \\
63.9591 & 15.260$\pm$0.026 & ZTF & g \\
65.9251 & 15.320$\pm$0.023 & ZTF & g \\
65.9251 & 15.320$\pm$0.023 & ZTF & g \\
65.9251 & 15.320$\pm$0.023 & ZTF & g \\
66.9374 & 15.304$\pm$0.035 & ZTF & g \\
66.9374 & 15.303$\pm$0.035 & ZTF & g \\
66.9374 & 15.303$\pm$0.035 & ZTF & g \\
69.9215 & 15.315$\pm$0.027 & ZTF & g \\
69.9215 & 15.315$\pm$0.027 & ZTF & g \\
69.9215 & 15.315$\pm$0.027 & ZTF & g \\
70.9085 & 15.267$\pm$0.027 & ZTF & g \\
70.9085 & 15.267$\pm$0.027 & ZTF & g \\
70.9085 & 15.267$\pm$0.027 & ZTF & g \\
71.9589 & 15.304$\pm$0.033 & ZTF & g \\
71.9589 & 15.304$\pm$0.033 & ZTF & g \\
71.9589 & 15.304$\pm$0.033 & ZTF & g \\
80.9217 & 15.490$\pm$0.046 & ZTF & g \\
80.9217 & 15.490$\pm$0.046 & ZTF & g \\
80.9231 & 15.523$\pm$0.023 & ZTF & g \\
80.9231 & 15.523$\pm$0.023 & ZTF & g \\
80.9572 & 15.488$\pm$0.044 & ZTF & g \\
80.9572 & 15.488$\pm$0.044 & ZTF & g \\
80.9606 & 15.531$\pm$0.039 & ZTF & g \\
80.9606 & 15.531$\pm$0.039 & ZTF & g \\
83.9219 & 15.471$\pm$0.029 & ZTF & g \\
83.9219 & 15.471$\pm$0.029 & ZTF & g \\
83.9229 & 15.468$\pm$0.033 & ZTF & g \\
83.9229 & 15.467$\pm$0.033 & ZTF & g \\
86.9602 & 15.550$\pm$0.030 & ZTF & g \\
90.8738 & 15.619$\pm$0.035 & ZTF & g \\
90.8738 & 15.619$\pm$0.035 & ZTF & g \\
93.9448 & 15.704$\pm$0.034 & ZTF & g \\
93.9448 & 15.704$\pm$0.034 & ZTF & g \\
95.9198 & 15.651$\pm$0.041 & ZTF & g \\
95.9198 & 15.651$\pm$0.041 & ZTF & g \\
98.9191 & 15.576$\pm$0.041 & ZTF & g \\
98.9191 & 15.576$\pm$0.041 & ZTF & g \\
101.8991 & 15.655$\pm$0.035 & ZTF & g \\
101.8991 & 15.655$\pm$0.035 & ZTF & g \\
101.9185 & 15.677$\pm$0.049 & ZTF & g \\
101.9185 & 15.677$\pm$0.049 & ZTF & g \\
103.9564 & 15.693$\pm$0.032 & ZTF & g \\
107.9407 & 15.708$\pm$0.049 & ZTF & g \\
110.8770 & 15.632$\pm$0.034 & ZTF & g \\
110.8770 & 15.632$\pm$0.034 & ZTF & g \\
110.9135 & 15.642$\pm$0.043 & ZTF & g \\
110.9135 & 15.642$\pm$0.043 & ZTF & g \\
113.8361 & 15.775$\pm$0.027 & ZTF & g \\
113.8361 & 15.775$\pm$0.027 & ZTF & g \\
115.9198 & 15.827$\pm$0.039 & ZTF & g \\
115.9198 & 15.827$\pm$0.039 & ZTF & g \\
117.9063 & 15.886$\pm$0.039 & ZTF & g \\
117.9063 & 15.886$\pm$0.039 & ZTF & g \\
117.9073 & 15.890$\pm$0.034 & ZTF & g \\
117.9073 & 15.890$\pm$0.034 & ZTF & g \\
119.8792 & 15.900$\pm$0.037 & ZTF & g \\
119.8792 & 15.900$\pm$0.037 & ZTF & g \\
119.8982 & 15.900$\pm$0.031 & ZTF & g \\
119.8982 & 15.900$\pm$0.031 & ZTF & g \\
122.8785 & 15.868$\pm$0.030 & ZTF & g \\
122.8785 & 15.868$\pm$0.030 & ZTF & g \\
122.8991 & 15.865$\pm$0.037 & ZTF & g \\
122.8991 & 15.865$\pm$0.037 & ZTF & g \\
126.8565 & 15.982$\pm$0.031 & ZTF & g \\
126.8565 & 15.982$\pm$0.031 & ZTF & g \\
126.8746 & 15.952$\pm$0.041 & ZTF & g \\
126.8746 & 15.952$\pm$0.041 & ZTF & g \\
129.8977 & 16.054$\pm$0.030 & ZTF & g \\
129.8977 & 16.054$\pm$0.030 & ZTF & g \\
139.8158 & 16.085$\pm$0.040 & ZTF & g \\
139.8158 & 16.085$\pm$0.040 & ZTF & g \\
139.8515 & 16.106$\pm$0.032 & ZTF & g \\
139.8515 & 16.106$\pm$0.032 & ZTF & g \\
139.8579 & 16.065$\pm$0.045 & ZTF & g \\
139.8579 & 16.064$\pm$0.045 & ZTF & g \\
139.8762 & 16.101$\pm$0.031 & ZTF & g \\
139.8762 & 16.101$\pm$0.031 & ZTF & g \\
140.8561 & 16.096$\pm$0.041 & ZTF & g \\
140.8561 & 16.096$\pm$0.041 & ZTF & g \\
140.8750 & 16.129$\pm$0.027 & ZTF & g \\
140.8750 & 16.129$\pm$0.027 & ZTF & g \\
141.8428 & 16.145$\pm$0.027 & ZTF & g \\
141.8428 & 16.145$\pm$0.027 & ZTF & g \\
141.8438 & 16.127$\pm$0.027 & ZTF & g \\
141.8438 & 16.127$\pm$0.027 & ZTF & g \\
141.8592 & 16.111$\pm$0.040 & ZTF & g \\
141.8592 & 16.111$\pm$0.040 & ZTF & g \\
141.8883 & 16.133$\pm$0.030 & ZTF & g \\
141.8883 & 16.133$\pm$0.030 & ZTF & g \\
143.8162 & 16.152$\pm$0.048 & ZTF & g \\
143.8162 & 16.152$\pm$0.048 & ZTF & g \\
143.8362 & 16.165$\pm$0.027 & ZTF & g \\
143.8362 & 16.165$\pm$0.027 & ZTF & g \\
146.8712 & 16.106$\pm$0.029 & ZTF & g \\
146.8712 & 16.106$\pm$0.029 & ZTF & g \\
148.8578 & 16.053$\pm$0.025 & ZTF & g \\
148.8578 & 16.053$\pm$0.025 & ZTF & g \\
149.7839 & 16.084$\pm$0.034 & ZTF & g \\
149.7839 & 16.084$\pm$0.034 & ZTF & g \\
150.8781 & 16.111$\pm$0.032 & ZTF & g \\
150.8781 & 16.111$\pm$0.032 & ZTF & g \\
151.7730 & 16.118$\pm$0.035 & ZTF & g \\
151.7730 & 16.118$\pm$0.035 & ZTF & g \\
152.8507 & 16.161$\pm$0.034 & ZTF & g \\
152.8507 & 16.161$\pm$0.034 & ZTF & g \\
155.8257 & 16.222$\pm$0.030 & ZTF & g \\
155.8257 & 16.222$\pm$0.030 & ZTF & g \\
156.7829 & 16.233$\pm$0.036 & ZTF & g \\
156.7829 & 16.233$\pm$0.036 & ZTF & g \\
157.8038 & 16.174$\pm$0.029 & ZTF & g \\
157.8038 & 16.174$\pm$0.029 & ZTF & g \\
158.8899 & 16.123$\pm$0.056 & ZTF & g \\
158.8899 & 16.123$\pm$0.056 & ZTF & g \\
159.8987 & 16.113$\pm$0.033 & ZTF & g \\
159.8987 & 16.113$\pm$0.033 & ZTF & g \\
163.8286 & 16.181$\pm$0.033 & ZTF & g \\
163.8286 & 16.181$\pm$0.033 & ZTF & g \\
164.8828 & 16.241$\pm$0.039 & ZTF & g \\
164.8828 & 16.241$\pm$0.039 & ZTF & g \\
166.7666 & 16.270$\pm$0.029 & ZTF & g \\
166.7666 & 16.270$\pm$0.029 & ZTF & g \\
167.8072 & 16.369$\pm$0.025 & ZTF & g \\
167.8072 & 16.369$\pm$0.025 & ZTF & g \\
171.7308 & 16.240$\pm$0.028 & ZTF & g \\
171.7308 & 16.240$\pm$0.028 & ZTF & g \\
172.8085 & 16.222$\pm$0.021 & ZTF & g \\
172.8085 & 16.221$\pm$0.021 & ZTF & g \\
173.7597 & 16.259$\pm$0.039 & ZTF & g \\
173.7597 & 16.259$\pm$0.039 & ZTF & g \\
174.7098 & 16.271$\pm$0.030 & ZTF & g \\
174.7098 & 16.271$\pm$0.030 & ZTF & g \\
176.7896 & 16.352$\pm$0.035 & ZTF & g \\
176.7896 & 16.352$\pm$0.035 & ZTF & g \\
178.7102 & 16.386$\pm$0.039 & ZTF & g \\
178.7102 & 16.386$\pm$0.039 & ZTF & g \\
179.8309 & 16.456$\pm$0.035 & ZTF & g \\
179.8309 & 16.456$\pm$0.035 & ZTF & g \\
180.7330 & 16.435$\pm$0.041 & ZTF & g \\
180.7330 & 16.435$\pm$0.041 & ZTF & g \\
181.8517 & 16.469$\pm$0.032 & ZTF & g \\
181.8517 & 16.469$\pm$0.032 & ZTF & g \\
182.7285 & 16.414$\pm$0.039 & ZTF & g \\
182.7285 & 16.414$\pm$0.039 & ZTF & g \\
183.7504 & 16.394$\pm$0.027 & ZTF & g \\
183.7504 & 16.394$\pm$0.027 & ZTF & g \\
185.7539 & 16.387$\pm$0.039 & ZTF & g \\
185.7539 & 16.387$\pm$0.039 & ZTF & g \\
194.7172 & 16.582$\pm$0.044 & ZTF & g \\
194.7172 & 16.582$\pm$0.044 & ZTF & g \\
194.8413 & 16.596$\pm$0.052 & ZTF & g \\
194.8413 & 16.596$\pm$0.052 & ZTF & g \\
196.7155 & 16.517$\pm$0.047 & ZTF & g \\
196.7155 & 16.517$\pm$0.047 & ZTF & g \\
196.7343 & 16.555$\pm$0.031 & ZTF & g \\
196.7343 & 16.555$\pm$0.031 & ZTF & g \\
197.6492 & 16.510$\pm$0.051 & ZTF & g \\
197.6492 & 16.510$\pm$0.051 & ZTF & g \\
197.6506 & 16.544$\pm$0.029 & ZTF & g \\
197.6506 & 16.544$\pm$0.029 & ZTF & g \\
199.6487 & 16.597$\pm$0.029 & ZTF & g \\
199.6487 & 16.597$\pm$0.029 & ZTF & g \\
199.7446 & 16.605$\pm$0.034 & ZTF & g \\
199.7446 & 16.605$\pm$0.034 & ZTF & g \\
201.7133 & 16.641$\pm$0.043 & ZTF & g \\
201.7133 & 16.641$\pm$0.043 & ZTF & g \\
204.6698 & 16.749$\pm$0.028 & ZTF & g \\
204.6698 & 16.748$\pm$0.028 & ZTF & g \\
205.6907 & 16.778$\pm$0.049 & ZTF & g \\
205.6907 & 16.778$\pm$0.049 & ZTF & g \\
206.6894 & 16.776$\pm$0.041 & ZTF & g \\
206.6894 & 16.776$\pm$0.041 & ZTF & g \\
207.6295 & 16.719$\pm$0.034 & ZTF & g \\
207.6295 & 16.719$\pm$0.034 & ZTF & g \\
210.7117 & 16.662$\pm$0.035 & ZTF & g \\
210.7117 & 16.662$\pm$0.035 & ZTF & g \\
222.6523 & 16.788$\pm$0.036 & ZTF & g \\
222.6523 & 16.788$\pm$0.036 & ZTF & g \\
222.6528 & 16.810$\pm$0.042 & ZTF & g \\
222.6528 & 16.810$\pm$0.042 & ZTF & g \\
228.6348 & 16.964$\pm$0.036 & ZTF & g \\
228.6348 & 16.964$\pm$0.036 & ZTF & g \\
228.6357 & 16.981$\pm$0.045 & ZTF & g \\
228.6357 & 16.981$\pm$0.045 & ZTF & g \\
230.6901 & 17.044$\pm$0.047 & ZTF & g \\
230.6901 & 17.044$\pm$0.047 & ZTF & g \\
230.7122 & 17.043$\pm$0.039 & ZTF & g \\
230.7122 & 17.043$\pm$0.039 & ZTF & g \\
233.6909 & 16.935$\pm$0.047 & ZTF & g \\
233.6909 & 16.935$\pm$0.047 & ZTF & g \\
234.6827 & 16.901$\pm$0.038 & ZTF & g \\
235.6876 & 16.905$\pm$0.036 & ZTF & g \\
235.6876 & 16.905$\pm$0.036 & ZTF & g \\
251.6305 & 17.140$\pm$0.052 & ZTF & g \\
251.6305 & 17.140$\pm$0.052 & ZTF & g \\
258.6200 & 17.065$\pm$0.055 & ZTF & g \\
258.6200 & 17.065$\pm$0.055 & ZTF & g \\
58.9425 & 14.681$\pm$0.037 & ZTF & r \\
58.9425 & 14.681$\pm$0.037 & ZTF & r \\
58.9425 & 14.681$\pm$0.037 & ZTF & r \\
60.9463 & 14.596$\pm$0.029 & ZTF & r \\
60.9463 & 14.596$\pm$0.029 & ZTF & r \\
60.9463 & 14.596$\pm$0.029 & ZTF & r \\
63.9338 & 14.658$\pm$0.031 & ZTF & r \\
63.9338 & 14.658$\pm$0.031 & ZTF & r \\
63.9338 & 14.658$\pm$0.031 & ZTF & r \\
65.9534 & 14.733$\pm$0.026 & ZTF & r \\
65.9534 & 14.733$\pm$0.026 & ZTF & r \\
65.9534 & 14.733$\pm$0.026 & ZTF & r \\
72.9207 & 14.797$\pm$0.027 & ZTF & r \\
72.9207 & 14.797$\pm$0.027 & ZTF & r \\
72.9207 & 14.797$\pm$0.027 & ZTF & r \\
74.9258 & 14.854$\pm$0.025 & ZTF & r \\
74.9258 & 14.854$\pm$0.025 & ZTF & r \\
74.9258 & 14.854$\pm$0.025 & ZTF & r \\
74.9267 & 14.870$\pm$0.024 & ZTF & r \\
74.9267 & 14.870$\pm$0.024 & ZTF & r \\
74.9267 & 14.870$\pm$0.024 & ZTF & r \\
74.9580 & 14.880$\pm$0.029 & ZTF & r \\
74.9580 & 14.880$\pm$0.029 & ZTF & r \\
74.9580 & 14.880$\pm$0.029 & ZTF & r \\
76.9149 & 14.909$\pm$0.025 & ZTF & r \\
76.9149 & 14.909$\pm$0.025 & ZTF & r \\
76.9465 & 14.928$\pm$0.041 & ZTF & r \\
76.9465 & 14.928$\pm$0.041 & ZTF & r \\
83.9692 & 15.117$\pm$0.031 & ZTF & r \\
83.9692 & 15.117$\pm$0.031 & ZTF & r \\
83.9697 & 15.070$\pm$0.027 & ZTF & r \\
83.9697 & 15.070$\pm$0.027 & ZTF & r \\
95.9405 & 15.301$\pm$0.044 & ZTF & r \\
95.9405 & 15.301$\pm$0.044 & ZTF & r \\
95.9415 & 15.280$\pm$0.044 & ZTF & r \\
95.9415 & 15.280$\pm$0.044 & ZTF & r \\
98.9410 & 15.295$\pm$0.028 & ZTF & r \\
98.9410 & 15.295$\pm$0.028 & ZTF & r \\
98.9414 & 15.288$\pm$0.021 & ZTF & r \\
98.9414 & 15.288$\pm$0.021 & ZTF & r \\
103.8781 & 15.407$\pm$0.024 & ZTF & r \\
103.8997 & 15.420$\pm$0.041 & ZTF & r \\
107.8668 & 15.451$\pm$0.033 & ZTF & r \\
108.9355 & 15.394$\pm$0.032 & ZTF & r \\
110.9397 & 15.428$\pm$0.027 & ZTF & r \\
110.9397 & 15.428$\pm$0.027 & ZTF & r \\
113.9200 & 15.525$\pm$0.023 & ZTF & r \\
113.9200 & 15.525$\pm$0.023 & ZTF & r \\
115.9627 & 15.593$\pm$0.025 & ZTF & r \\
115.9627 & 15.593$\pm$0.025 & ZTF & r \\
117.8792 & 15.668$\pm$0.028 & ZTF & r \\
117.8792 & 15.668$\pm$0.028 & ZTF & r \\
117.8802 & 15.668$\pm$0.039 & ZTF & r \\
117.8802 & 15.668$\pm$0.039 & ZTF & r \\
122.9737 & 15.685$\pm$0.021 & ZTF & r \\
122.9737 & 15.685$\pm$0.021 & ZTF & r \\
124.8942 & 15.688$\pm$0.028 & ZTF & r \\
124.8942 & 15.688$\pm$0.028 & ZTF & r \\
129.9194 & 15.870$\pm$0.023 & ZTF & r \\
129.9194 & 15.870$\pm$0.023 & ZTF & r \\
143.7963 & 16.063$\pm$0.036 & ZTF & r \\
143.7963 & 16.063$\pm$0.036 & ZTF & r \\
146.8996 & 15.975$\pm$0.027 & ZTF & r \\
146.8996 & 15.975$\pm$0.027 & ZTF & r \\
148.8370 & 16.005$\pm$0.025 & ZTF & r \\
148.8370 & 16.005$\pm$0.025 & ZTF & r \\
149.8166 & 15.994$\pm$0.036 & ZTF & r \\
149.8166 & 15.994$\pm$0.036 & ZTF & r \\
150.8154 & 16.051$\pm$0.029 & ZTF & r \\
150.8154 & 16.051$\pm$0.029 & ZTF & r \\
151.7951 & 16.044$\pm$0.037 & ZTF & r \\
151.7951 & 16.044$\pm$0.037 & ZTF & r \\
152.8157 & 16.061$\pm$0.030 & ZTF & r \\
152.8157 & 16.061$\pm$0.030 & ZTF & r \\
155.8825 & 16.148$\pm$0.035 & ZTF & r \\
155.8825 & 16.148$\pm$0.035 & ZTF & r \\
157.8926 & 16.129$\pm$0.034 & ZTF & r \\
157.8926 & 16.129$\pm$0.034 & ZTF & r \\
158.8164 & 16.056$\pm$0.035 & ZTF & r \\
158.8164 & 16.056$\pm$0.035 & ZTF & r \\
159.8257 & 16.103$\pm$0.042 & ZTF & r \\
159.8257 & 16.103$\pm$0.042 & ZTF & r \\
162.7945 & 16.153$\pm$0.019 & ZTF & r \\
162.7945 & 16.153$\pm$0.019 & ZTF & r \\
164.7663 & 16.193$\pm$0.021 & ZTF & r \\
164.7663 & 16.193$\pm$0.021 & ZTF & r \\
165.8283 & 16.220$\pm$0.031 & ZTF & r \\
165.8283 & 16.220$\pm$0.031 & ZTF & r \\
165.8408 & 16.427$\pm$0.034 & ZTF & r \\
165.8408 & 16.427$\pm$0.034 & ZTF & r \\
166.8406 & 16.208$\pm$0.016 & ZTF & r \\
166.8406 & 16.208$\pm$0.016 & ZTF & r \\
167.8216 & 16.278$\pm$0.025 & ZTF & r \\
167.8216 & 16.278$\pm$0.025 & ZTF & r \\
170.7948 & 16.249$\pm$0.024 & ZTF & r \\
170.7948 & 16.249$\pm$0.024 & ZTF & r \\
171.7905 & 16.231$\pm$0.028 & ZTF & r \\
171.7905 & 16.230$\pm$0.028 & ZTF & r \\
172.8583 & 16.261$\pm$0.028 & ZTF & r \\
172.8583 & 16.261$\pm$0.028 & ZTF & r \\
174.7726 & 16.322$\pm$0.032 & ZTF & r \\
174.7726 & 16.322$\pm$0.032 & ZTF & r \\
177.8372 & 16.348$\pm$0.036 & ZTF & r \\
177.8372 & 16.348$\pm$0.036 & ZTF & r \\
178.7341 & 16.377$\pm$0.022 & ZTF & r \\
178.7341 & 16.377$\pm$0.022 & ZTF & r \\
179.7732 & 16.409$\pm$0.034 & ZTF & r \\
179.7732 & 16.408$\pm$0.034 & ZTF & r \\
181.7730 & 16.452$\pm$0.045 & ZTF & r \\
181.7730 & 16.452$\pm$0.045 & ZTF & r \\
182.7332 & 16.412$\pm$0.032 & ZTF & r \\
182.7332 & 16.412$\pm$0.032 & ZTF & r \\
183.7943 & 16.373$\pm$0.027 & ZTF & r \\
183.7943 & 16.373$\pm$0.027 & ZTF & r \\
185.7322 & 16.399$\pm$0.029 & ZTF & r \\
185.7322 & 16.399$\pm$0.029 & ZTF & r \\
194.7554 & 16.657$\pm$0.036 & ZTF & r \\
194.7554 & 16.657$\pm$0.036 & ZTF & r \\
194.7737 & 16.651$\pm$0.041 & ZTF & r \\
194.7737 & 16.651$\pm$0.041 & ZTF & r \\
196.7705 & 16.540$\pm$0.031 & ZTF & r \\
196.7705 & 16.540$\pm$0.031 & ZTF & r \\
196.7858 & 16.570$\pm$0.031 & ZTF & r \\
196.7858 & 16.570$\pm$0.031 & ZTF & r \\
199.6735 & 16.621$\pm$0.041 & ZTF & r \\
199.6735 & 16.621$\pm$0.041 & ZTF & r \\
199.6745 & 16.663$\pm$0.032 & ZTF & r \\
199.6745 & 16.663$\pm$0.032 & ZTF & r \\
200.7326 & 16.673$\pm$0.040 & ZTF & r \\
200.7326 & 16.673$\pm$0.040 & ZTF & r \\
201.6711 & 16.700$\pm$0.049 & ZTF & r \\
201.6711 & 16.700$\pm$0.049 & ZTF & r \\
202.6907 & 16.711$\pm$0.033 & ZTF & r \\
202.6907 & 16.711$\pm$0.033 & ZTF & r \\
203.6925 & 16.719$\pm$0.034 & ZTF & r \\
203.6925 & 16.719$\pm$0.034 & ZTF & r \\
204.6902 & 16.783$\pm$0.036 & ZTF & r \\
204.6902 & 16.783$\pm$0.036 & ZTF & r \\
206.7320 & 16.811$\pm$0.033 & ZTF & r \\
206.7320 & 16.811$\pm$0.033 & ZTF & r \\
207.6699 & 16.756$\pm$0.040 & ZTF & r \\
207.6699 & 16.756$\pm$0.040 & ZTF & r \\
208.6680 & 16.723$\pm$0.032 & ZTF & r \\
208.6680 & 16.723$\pm$0.032 & ZTF & r \\
209.6748 & 16.725$\pm$0.031 & ZTF & r \\
209.6748 & 16.725$\pm$0.031 & ZTF & r \\
210.6717 & 16.791$\pm$0.036 & ZTF & r \\
210.6717 & 16.791$\pm$0.036 & ZTF & r \\
211.6855 & 16.845$\pm$0.054 & ZTF & r \\
211.6855 & 16.845$\pm$0.054 & ZTF & r \\
213.6681 & 16.827$\pm$0.033 & ZTF & r \\
213.6681 & 16.827$\pm$0.033 & ZTF & r \\
222.6873 & 16.872$\pm$0.041 & ZTF & r \\
222.6873 & 16.872$\pm$0.041 & ZTF & r \\
222.6878 & 16.877$\pm$0.036 & ZTF & r \\
222.6878 & 16.877$\pm$0.036 & ZTF & r \\
228.6492 & 17.040$\pm$0.035 & ZTF & r \\
228.6492 & 17.039$\pm$0.035 & ZTF & r \\
228.6539 & 17.023$\pm$0.033 & ZTF & r \\
228.6539 & 17.023$\pm$0.033 & ZTF & r \\
230.6063 & 17.044$\pm$0.040 & ZTF & r \\
230.6063 & 17.044$\pm$0.040 & ZTF & r \\
230.6073 & 17.080$\pm$0.049 & ZTF & r \\
230.6073 & 17.080$\pm$0.049 & ZTF & r \\
236.6284 & 17.003$\pm$0.054 & ZTF & r \\
236.6284 & 17.003$\pm$0.054 & ZTF & r \\
237.6746 & 17.049$\pm$0.047 & ZTF & r \\
237.6746 & 17.049$\pm$0.047 & ZTF & r \\
251.6594 & 17.172$\pm$0.035 & ZTF & r \\
251.6594 & 17.172$\pm$0.035 & ZTF & r \\
251.6599 & 17.266$\pm$0.053 & ZTF & r \\
251.6599 & 17.266$\pm$0.053 & ZTF & r \\
256.6299 & 17.308$\pm$0.042 & ZTF & r \\
256.6299 & 17.308$\pm$0.042 & ZTF & r \\
257.6634 & 17.327$\pm$0.071 & ZTF & r \\
257.6634 & 17.327$\pm$0.071 & ZTF & r \\
258.6332 & 17.139$\pm$0.040 & ZTF & r \\
258.6332 & 17.139$\pm$0.040 & ZTF & r \\
267.6225 & 17.399$\pm$0.065 & ZTF & r \\
267.6225 & 17.399$\pm$0.065 & ZTF & r \\
268.6552 & 17.509$\pm$0.063 & ZTF & r \\
94.9198 & 14.946$\pm$0.028 & ZTF & i \\
94.9198 & 14.946$\pm$0.028 & ZTF & i \\
94.9340 & 14.943$\pm$0.035 & ZTF & i \\
109.9395 & 14.984$\pm$0.049 & ZTF & i \\
124.9426 & 15.368$\pm$0.042 & ZTF & i \\
124.9426 & 15.368$\pm$0.042 & ZTF & i \\
127.8977 & 15.350$\pm$0.029 & ZTF & i \\
127.8977 & 15.350$\pm$0.029 & ZTF & i \\
142.8349 & 15.568$\pm$0.029 & ZTF & i \\
142.8349 & 15.568$\pm$0.029 & ZTF & i \\
157.8189 & 15.677$\pm$0.036 & ZTF & i \\
157.8189 & 15.677$\pm$0.036 & ZTF & i \\
172.7626 & 15.732$\pm$0.041 & ZTF & i \\
172.7626 & 15.732$\pm$0.041 & ZTF & i \\
180.7730 & 15.965$\pm$0.030 & ZTF & i \\
180.7730 & 15.965$\pm$0.030 & ZTF & i \\
180.7740 & 15.936$\pm$0.035 & ZTF & i \\
180.7740 & 15.936$\pm$0.035 & ZTF & i \\
183.7524 & 15.881$\pm$0.040 & ZTF & i \\
183.7524 & 15.881$\pm$0.040 & ZTF & i \\
183.7721 & 15.878$\pm$0.034 & ZTF & i \\
183.7721 & 15.878$\pm$0.034 & ZTF & i \\
187.7106 & 15.954$\pm$0.035 & ZTF & i \\
187.7106 & 15.954$\pm$0.035 & ZTF & i \\
200.6612 & 16.135$\pm$0.026 & ZTF & i \\
200.6612 & 16.135$\pm$0.026 & ZTF & i \\
201.8214 & 16.165$\pm$0.037 & ZTF & i \\
201.8214 & 16.165$\pm$0.037 & ZTF & i \\
203.6064 & 16.202$\pm$0.042 & ZTF & i \\
203.6064 & 16.202$\pm$0.042 & ZTF & i \\
205.6492 & 16.312$\pm$0.045 & ZTF & i \\
205.6492 & 16.312$\pm$0.045 & ZTF & i \\
214.7522 & 16.335$\pm$0.036 & ZTF & i \\
214.7522 & 16.335$\pm$0.036 & ZTF & i \\
233.7132 & 16.417$\pm$0.049 & ZTF & i \\
223.9858 & 18.583$\pm$0.036 & Mephisto & u \\
223.9911 & 18.572$\pm$0.036 & Mephisto & u \\
223.9963 & 18.547$\pm$0.035 & Mephisto & u \\
223.9999 & 18.553$\pm$0.038 & Mephisto & u \\
224.0011 & 18.479$\pm$0.035 & Mephisto & u \\
226.0153 & 18.649$\pm$0.038 & Mephisto & u \\
226.0187 & 18.722$\pm$0.042 & Mephisto & u \\
226.0212 & 18.733$\pm$0.042 & Mephisto & u \\
227.9833 & 19.015$\pm$0.055 & Mephisto & u \\
227.9946 & 18.830$\pm$0.046 & Mephisto & u \\
227.9958 & 18.890$\pm$0.048 & Mephisto & u \\
228.0002 & 18.831$\pm$0.046 & Mephisto & u \\
228.0103 & 18.822$\pm$0.046 & Mephisto & u \\
228.9830 & 18.953$\pm$0.052 & Mephisto & u \\
228.9854 & 18.893$\pm$0.049 & Mephisto & u \\
228.9878 & 18.856$\pm$0.047 & Mephisto & u \\
257.0086 & 19.120$\pm$0.060 & Mephisto & u \\
257.0110 & 19.118$\pm$0.060 & Mephisto & u \\
257.0133 & 19.128$\pm$0.060 & Mephisto & u \\
257.9959 & 18.792$\pm$0.044 & Mephisto & u \\
257.9984 & 18.785$\pm$0.043 & Mephisto & u \\
258.0011 & 18.731$\pm$0.041 & Mephisto & u \\
258.9981 & 18.711$\pm$0.041 & Mephisto & u \\
259.0013 & 18.785$\pm$0.043 & Mephisto & u \\
259.0036 & 18.759$\pm$0.042 & Mephisto & u \\
263.0037 & 18.472$\pm$0.033 & Mephisto & u \\
263.0062 & 18.434$\pm$0.032 & Mephisto & u \\
263.0085 & 18.467$\pm$0.033 & Mephisto & u \\
263.9973 & 18.449$\pm$0.032 & Mephisto & u \\
263.9996 & 18.435$\pm$0.032 & Mephisto & u \\
264.0024 & 18.391$\pm$0.030 & Mephisto & u \\
264.0058 & 18.450$\pm$0.032 & Mephisto & u \\
275.0025 & 19.521$\pm$0.084 & Mephisto & u \\
279.0068 & 19.889$\pm$0.122 & Mephisto & u \\
279.9991 & 20.190$\pm$0.188 & Mephisto & u \\
224.0031 & 17.957$\pm$0.030 & Mephisto & v \\
224.0057 & 17.935$\pm$0.029 & Mephisto & v \\
224.0083 & 17.904$\pm$0.028 & Mephisto & v \\
224.0158 & 17.803$\pm$0.027 & Mephisto & v \\
224.0182 & 17.875$\pm$0.029 & Mephisto & v \\
224.0196 & 17.851$\pm$0.029 & Mephisto & v \\
224.0204 & 17.819$\pm$0.028 & Mephisto & v \\
224.0223 & 17.892$\pm$0.030 & Mephisto & v \\
224.0242 & 17.886$\pm$0.030 & Mephisto & v \\
224.0285 & 17.827$\pm$0.028 & Mephisto & v \\
224.0296 & 17.897$\pm$0.030 & Mephisto & v \\
226.0243 & 17.939$\pm$0.029 & Mephisto & v \\
226.0267 & 17.925$\pm$0.029 & Mephisto & v \\
226.0291 & 17.925$\pm$0.029 & Mephisto & v \\
227.0545 & 17.997$\pm$0.031 & Mephisto & v \\
227.9747 & 17.930$\pm$0.029 & Mephisto & v \\
227.9775 & 18.089$\pm$0.034 & Mephisto & v \\
227.9799 & 18.116$\pm$0.035 & Mephisto & v \\
228.9919 & 18.045$\pm$0.032 & Mephisto & v \\
228.9956 & 18.047$\pm$0.032 & Mephisto & v \\
228.9979 & 18.023$\pm$0.031 & Mephisto & v \\
256.9953 & 18.421$\pm$0.046 & Mephisto & v \\
257.0026 & 18.321$\pm$0.041 & Mephisto & v \\
257.0052 & 18.327$\pm$0.041 & Mephisto & v \\
257.9871 & 18.099$\pm$0.034 & Mephisto & v \\
257.9896 & 18.192$\pm$0.037 & Mephisto & v \\
257.9920 & 18.209$\pm$0.037 & Mephisto & v \\
258.9873 & 18.075$\pm$0.033 & Mephisto & v \\
258.9900 & 18.103$\pm$0.034 & Mephisto & v \\
258.9930 & 18.150$\pm$0.036 & Mephisto & v \\
259.9881 & 18.049$\pm$0.032 & Mephisto & v \\
259.9931 & 18.068$\pm$0.033 & Mephisto & v \\
260.9919 & 18.006$\pm$0.031 & Mephisto & v \\
260.9983 & 18.047$\pm$0.032 & Mephisto & v \\
261.9929 & 18.038$\pm$0.033 & Mephisto & v \\
261.9952 & 18.047$\pm$0.033 & Mephisto & v \\
261.9975 & 18.059$\pm$0.034 & Mephisto & v \\
262.9900 & 17.937$\pm$0.029 & Mephisto & v \\
263.0004 & 17.947$\pm$0.029 & Mephisto & v \\
263.0138 & 17.907$\pm$0.028 & Mephisto & v \\
263.9897 & 17.827$\pm$0.026 & Mephisto & v \\
263.9919 & 17.837$\pm$0.026 & Mephisto & v \\
263.9942 & 17.844$\pm$0.027 & Mephisto & v \\
264.0123 & 17.876$\pm$0.027 & Mephisto & v \\
265.9983 & 18.039$\pm$0.032 & Mephisto & v \\
275.0074 & 18.958$\pm$0.073 & Mephisto & v \\
279.0017 & 19.693$\pm$0.146 & Mephisto & v \\
280.0042 & 19.431$\pm$0.113 & Mephisto & v \\
223.9858 & 16.166$\pm$0.005 & Mephisto & i \\
223.9911 & 16.144$\pm$0.005 & Mephisto & i \\
223.9963 & 16.170$\pm$0.005 & Mephisto & i \\
223.9999 & 16.145$\pm$0.006 & Mephisto & i \\
224.0011 & 16.081$\pm$0.007 & Mephisto & i \\
226.0243 & 16.338$\pm$0.005 & Mephisto & i \\
226.0267 & 16.271$\pm$0.005 & Mephisto & i \\
226.0291 & 16.261$\pm$0.005 & Mephisto & i \\
228.9919 & 16.304$\pm$0.005 & Mephisto & i \\
228.9956 & 16.284$\pm$0.005 & Mephisto & i \\
228.9979 & 16.279$\pm$0.005 & Mephisto & i \\
256.9953 & 16.552$\pm$0.006 & Mephisto & i \\
257.0026 & 16.521$\pm$0.006 & Mephisto & i \\
257.0052 & 16.540$\pm$0.006 & Mephisto & i \\
257.9871 & 16.395$\pm$0.006 & Mephisto & i \\
257.9897 & 16.385$\pm$0.006 & Mephisto & i \\
257.9920 & 16.388$\pm$0.006 & Mephisto & i \\
258.9873 & 16.279$\pm$0.006 & Mephisto & i \\
259.0071 & 16.344$\pm$0.006 & Mephisto & i \\
259.0095 & 16.338$\pm$0.006 & Mephisto & i \\
259.9881 & 16.271$\pm$0.006 & Mephisto & i \\
259.9931 & 16.249$\pm$0.006 & Mephisto & i \\
261.9929 & 16.334$\pm$0.005 & Mephisto & i \\
261.9952 & 16.313$\pm$0.005 & Mephisto & i \\
261.9975 & 16.332$\pm$0.005 & Mephisto & i \\
262.9900 & 16.238$\pm$0.005 & Mephisto & i \\
263.0004 & 16.282$\pm$0.005 & Mephisto & i \\
263.0138 & 16.297$\pm$0.005 & Mephisto & i \\
263.9897 & 16.285$\pm$0.005 & Mephisto & i \\
263.9919 & 16.293$\pm$0.005 & Mephisto & i \\
263.9942 & 16.311$\pm$0.005 & Mephisto & i \\
264.0123 & 16.331$\pm$0.005 & Mephisto & i \\
269.9925 & 16.729$\pm$0.013 & Mephisto & i \\
269.9930 & 16.629$\pm$0.014 & Mephisto & i \\
269.9936 & 16.698$\pm$0.013 & Mephisto & i \\
275.0025 & 17.341$\pm$0.012 & Mephisto & i \\
279.0068 & 17.535$\pm$0.032 & Mephisto & i \\
279.9991 & 17.792$\pm$0.019 & Mephisto & i \\
224.0031 & 16.419$\pm$0.019 & Mephisto & z \\
224.0057 & 16.455$\pm$0.019 & Mephisto & z \\
224.0082 & 16.418$\pm$0.019 & Mephisto & z \\
224.0158 & 16.459$\pm$0.021 & Mephisto & z \\
224.0182 & 16.500$\pm$0.022 & Mephisto & z \\
224.0196 & 16.473$\pm$0.021 & Mephisto & z \\
224.0204 & 16.471$\pm$0.021 & Mephisto & z \\
224.0223 & 16.503$\pm$0.022 & Mephisto & z \\
224.0241 & 16.495$\pm$0.022 & Mephisto & z \\
224.0285 & 16.528$\pm$0.022 & Mephisto & z \\
224.0296 & 16.540$\pm$0.022 & Mephisto & z \\
226.0153 & 16.904$\pm$0.032 & Mephisto & z \\
226.0187 & 16.613$\pm$0.022 & Mephisto & z \\
226.0212 & 16.612$\pm$0.022 & Mephisto & z \\
228.9830 & 16.647$\pm$0.023 & Mephisto & z \\
228.9854 & 16.669$\pm$0.023 & Mephisto & z \\
228.9878 & 16.632$\pm$0.023 & Mephisto & z \\
257.0086 & 17.079$\pm$0.034 & Mephisto & z \\
257.0110 & 17.083$\pm$0.035 & Mephisto & z \\
257.0133 & 17.064$\pm$0.034 & Mephisto & z \\
257.9960 & 16.725$\pm$0.025 & Mephisto & z \\
257.9984 & 16.720$\pm$0.025 & Mephisto & z \\
258.0010 & 16.767$\pm$0.026 & Mephisto & z \\
259.0132 & 16.665$\pm$0.024 & Mephisto & z \\
259.0155 & 16.539$\pm$0.022 & Mephisto & z \\
259.0178 & 16.570$\pm$0.022 & Mephisto & z \\
259.9962 & 16.567$\pm$0.022 & Mephisto & z \\
259.9986 & 16.506$\pm$0.022 & Mephisto & z \\
260.0009 & 16.516$\pm$0.022 & Mephisto & z \\
262.0010 & 16.667$\pm$0.023 & Mephisto & z \\
262.0033 & 16.673$\pm$0.023 & Mephisto & z \\
262.0056 & 16.649$\pm$0.023 & Mephisto & z \\
263.0037 & 16.566$\pm$0.021 & Mephisto & z \\
263.0062 & 16.557$\pm$0.021 & Mephisto & z \\
263.0085 & 16.503$\pm$0.021 & Mephisto & z \\
263.9973 & 16.665$\pm$0.023 & Mephisto & z \\
263.9996 & 16.652$\pm$0.023 & Mephisto & z \\
264.0024 & 16.649$\pm$0.023 & Mephisto & z \\
264.0057 & 16.677$\pm$0.023 & Mephisto & z \\
269.9950 & 17.053$\pm$0.040 & Mephisto & z \\
269.9956 & 17.082$\pm$0.036 & Mephisto & z \\
269.9961 & 17.358$\pm$0.048 & Mephisto & z \\
275.0074 & 18.657$\pm$0.146 & Mephisto & z \\
279.0017 & 18.220$\pm$0.096 & Mephisto & z \\
280.0042 & 18.932$\pm$0.183 & Mephisto & z \\
210.5913 & 18.249$\pm$0.116 & PO & u \\
210.5937 & 18.276$\pm$0.122 & PO & u \\
210.5961 & 18.257$\pm$0.117 & PO & u \\
210.5986 & 18.228$\pm$0.117 & PO & u \\
210.6010 & 18.639$\pm$0.153 & PO & u \\
210.6034 & 18.699$\pm$0.165 & PO & u \\
213.5913 & 18.506$\pm$0.128 & PO & u \\
213.5937 & 18.520$\pm$0.140 & PO & u \\
213.5961 & 18.400$\pm$0.127 & PO & u \\
213.5985 & 18.567$\pm$0.151 & PO & u \\
213.6009 & 18.396$\pm$0.118 & PO & u \\
213.6034 & 18.597$\pm$0.144 & PO & u \\
214.5912 & 18.309$\pm$0.154 & PO & u \\
214.5937 & 17.971$\pm$0.161 & PO & u \\
214.5961 & 18.566$\pm$0.176 & PO & u \\
214.5986 & 18.307$\pm$0.139 & PO & u \\
214.6010 & 18.520$\pm$0.166 & PO & u \\
214.6035 & 18.221$\pm$0.134 & PO & u \\
214.7042 & 18.025$\pm$0.160 & PO & u \\
214.7066 & 17.705$\pm$0.137 & PO & u \\
214.7090 & 17.911$\pm$0.144 & PO & u \\
214.7114 & 17.931$\pm$0.153 & PO & u \\
214.7139 & 17.985$\pm$0.157 & PO & u \\
214.7163 & 18.066$\pm$0.164 & PO & u \\
215.5912 & 18.498$\pm$0.213 & PO & u \\
215.5937 & 18.216$\pm$0.156 & PO & u \\
215.5961 & 18.113$\pm$0.151 & PO & u \\
215.5986 & 18.667$\pm$0.210 & PO & u \\
215.6010 & 18.552$\pm$0.175 & PO & u \\
215.6035 & 18.506$\pm$0.174 & PO & u \\
219.5739 & 18.268$\pm$0.162 & PO & u \\
219.5763 & 18.545$\pm$0.190 & PO & u \\
219.5788 & 18.378$\pm$0.149 & PO & u \\
219.5812 & 18.715$\pm$0.211 & PO & u \\
219.5836 & 18.677$\pm$0.185 & PO & u \\
219.5860 & 18.615$\pm$0.180 & PO & u \\
219.6467 & 18.283$\pm$0.149 & PO & u \\
219.6491 & 18.712$\pm$0.189 & PO & u \\
219.6540 & 18.930$\pm$0.312 & PO & u \\
219.6588 & 18.421$\pm$0.192 & PO & u \\
221.5790 & 18.291$\pm$0.177 & PO & u \\
221.5815 & 18.259$\pm$0.182 & PO & u \\
221.5839 & 18.299$\pm$0.158 & PO & u \\
221.5864 & 18.959$\pm$0.320 & PO & u \\
221.6467 & 18.272$\pm$0.180 & PO & u \\
221.6492 & 18.308$\pm$0.174 & PO & u \\
221.6540 & 18.423$\pm$0.206 & PO & u \\
221.6564 & 17.886$\pm$0.148 & PO & u \\
221.6588 & 18.775$\pm$0.272 & PO & u \\
222.5740 & 18.253$\pm$0.156 & PO & u \\
222.5764 & 18.147$\pm$0.141 & PO & u \\
222.5789 & 18.625$\pm$0.198 & PO & u \\
222.5814 & 18.291$\pm$0.139 & PO & u \\
222.5838 & 18.297$\pm$0.134 & PO & u \\
222.5863 & 18.703$\pm$0.184 & PO & u \\
222.6467 & 18.189$\pm$0.155 & PO & u \\
222.6491 & 18.278$\pm$0.147 & PO & u \\
222.6516 & 18.580$\pm$0.198 & PO & u \\
222.6540 & 18.501$\pm$0.173 & PO & u \\
222.6564 & 18.271$\pm$0.165 & PO & u \\
222.6588 & 18.265$\pm$0.153 & PO & u \\
225.5634 & 18.549$\pm$0.140 & PO & u \\
225.5658 & 18.330$\pm$0.113 & PO & u \\
225.5683 & 18.370$\pm$0.112 & PO & u \\
225.5707 & 18.711$\pm$0.149 & PO & u \\
225.5731 & 18.463$\pm$0.123 & PO & u \\
225.5755 & 18.514$\pm$0.125 & PO & u \\
227.5698 & 18.436$\pm$0.116 & PO & u \\
227.5722 & 18.601$\pm$0.124 & PO & u \\
227.5747 & 18.466$\pm$0.112 & PO & u \\
227.5771 & 18.481$\pm$0.120 & PO & u \\
227.5796 & 18.349$\pm$0.106 & PO & u \\
227.5820 & 18.466$\pm$0.121 & PO & u \\
228.6095 & 18.597$\pm$0.133 & PO & u \\
228.6119 & 18.523$\pm$0.123 & PO & u \\
228.6144 & 18.563$\pm$0.135 & PO & u \\
228.6168 & 18.522$\pm$0.131 & PO & u \\
228.6193 & 18.824$\pm$0.152 & PO & u \\
228.6217 & 18.474$\pm$0.123 & PO & u \\
228.6622 & 18.833$\pm$0.161 & PO & u \\
228.6646 & 19.413$\pm$0.215 & PO & u \\
228.6670 & 19.350$\pm$0.211 & PO & u \\
228.6694 & 19.397$\pm$0.220 & PO & u \\
228.6720 & 18.817$\pm$0.148 & PO & u \\
228.6744 & 19.052$\pm$0.181 & PO & u \\
229.5637 & 18.386$\pm$0.116 & PO & u \\
229.5686 & 18.528$\pm$0.132 & PO & u \\
229.5736 & 18.594$\pm$0.136 & PO & u \\
229.5760 & 18.497$\pm$0.122 & PO & u \\
229.6258 & 18.887$\pm$0.158 & PO & u \\
229.6282 & 19.092$\pm$0.212 & PO & u \\
229.6355 & 18.819$\pm$0.153 & PO & u \\
229.6379 & 18.765$\pm$0.143 & PO & u \\
231.5531 & 18.781$\pm$0.152 & PO & u \\
231.5555 & 18.802$\pm$0.154 & PO & u \\
231.5580 & 18.900$\pm$0.158 & PO & u \\
231.5604 & 18.657$\pm$0.134 & PO & u \\
231.5629 & 18.772$\pm$0.137 & PO & u \\
231.5653 & 18.672$\pm$0.125 & PO & u \\
232.6053 & 18.634$\pm$0.126 & PO & u \\
232.6078 & 18.498$\pm$0.110 & PO & u \\
232.6102 & 18.624$\pm$0.126 & PO & u \\
232.6126 & 18.547$\pm$0.123 & PO & u \\
232.6150 & 18.612$\pm$0.123 & PO & u \\
232.6175 & 18.611$\pm$0.122 & PO & u \\
233.5426 & 18.422$\pm$0.129 & PO & u \\
233.5450 & 18.515$\pm$0.122 & PO & u \\
233.5475 & 18.355$\pm$0.111 & PO & u \\
233.5524 & 18.285$\pm$0.103 & PO & u \\
233.5548 & 18.429$\pm$0.118 & PO & u \\
235.6174 & 18.290$\pm$0.124 & PO & u \\
235.6199 & 18.701$\pm$0.200 & PO & u \\
235.6247 & 18.664$\pm$0.143 & PO & u \\
235.6271 & 18.434$\pm$0.128 & PO & u \\
235.6296 & 18.779$\pm$0.174 & PO & u \\
236.6308 & 18.526$\pm$0.134 & PO & u \\
236.6332 & 18.881$\pm$0.172 & PO & u \\
236.6356 & 18.658$\pm$0.141 & PO & u \\
236.6381 & 18.709$\pm$0.145 & PO & u \\
236.6405 & 18.896$\pm$0.154 & PO & u \\
236.6430 & 18.646$\pm$0.143 & PO & u \\
237.6600 & 18.584$\pm$0.123 & PO & u \\
237.6625 & 18.383$\pm$0.111 & PO & u \\
237.6649 & 18.839$\pm$0.142 & PO & u \\
237.6722 & 18.688$\pm$0.136 & PO & u \\
238.6188 & 18.444$\pm$0.114 & PO & u \\
238.6212 & 18.504$\pm$0.121 & PO & u \\
238.6237 & 18.582$\pm$0.124 & PO & u \\
238.6261 & 18.620$\pm$0.130 & PO & u \\
238.6285 & 18.589$\pm$0.127 & PO & u \\
238.6310 & 18.944$\pm$0.158 & PO & u \\
240.5565 & 18.547$\pm$0.122 & PO & u \\
240.5589 & 18.461$\pm$0.126 & PO & u \\
240.5613 & 18.655$\pm$0.131 & PO & u \\
240.5638 & 18.689$\pm$0.128 & PO & u \\
240.5662 & 18.547$\pm$0.118 & PO & u \\
240.5687 & 18.498$\pm$0.118 & PO & u \\
240.5711 & 18.710$\pm$0.128 & PO & u \\
240.6285 & 18.476$\pm$0.119 & PO & u \\
240.6309 & 18.559$\pm$0.128 & PO & u \\
240.6333 & 18.623$\pm$0.142 & PO & u \\
240.6358 & 18.861$\pm$0.152 & PO & u \\
240.6382 & 18.738$\pm$0.152 & PO & u \\
240.6406 & 18.731$\pm$0.143 & PO & u \\
240.6430 & 18.797$\pm$0.145 & PO & u \\
241.5630 & 18.358$\pm$0.119 & PO & u \\
241.5679 & 18.948$\pm$0.170 & PO & u \\
241.5703 & 18.718$\pm$0.143 & PO & u \\
241.5753 & 18.670$\pm$0.162 & PO & u \\
241.5777 & 18.494$\pm$0.138 & PO & u \\
247.5927 & 18.502$\pm$0.162 & PO & u \\
247.5951 & 18.105$\pm$0.125 & PO & u \\
247.5975 & 18.362$\pm$0.144 & PO & u \\
247.5999 & 18.260$\pm$0.129 & PO & u \\
247.6023 & 18.593$\pm$0.182 & PO & u \\
247.6048 & 18.624$\pm$0.186 & PO & u \\
247.6072 & 18.208$\pm$0.148 & PO & u \\
247.6646 & 18.295$\pm$0.145 & PO & u \\
247.6670 & 18.644$\pm$0.192 & PO & u \\
247.6695 & 18.811$\pm$0.282 & PO & u \\
248.5788 & 18.264$\pm$0.136 & PO & u \\
248.5812 & 18.804$\pm$0.205 & PO & u \\
248.5836 & 18.187$\pm$0.137 & PO & u \\
248.5861 & 18.430$\pm$0.153 & PO & u \\
248.5885 & 18.570$\pm$0.169 & PO & u \\
248.5909 & 18.705$\pm$0.220 & PO & u \\
248.5933 & 18.509$\pm$0.187 & PO & u \\
249.5571 & 18.154$\pm$0.126 & PO & u \\
249.5595 & 18.424$\pm$0.137 & PO & u \\
249.5620 & 18.803$\pm$0.196 & PO & u \\
249.5644 & 18.103$\pm$0.130 & PO & u \\
249.5693 & 18.516$\pm$0.196 & PO & u \\
249.5718 & 18.653$\pm$0.200 & PO & u \\
251.5897 & 18.170$\pm$0.130 & PO & u \\
251.5927 & 18.415$\pm$0.205 & PO & u \\
251.5958 & 18.140$\pm$0.132 & PO & u \\
251.6018 & 18.931$\pm$0.296 & PO & u \\
252.5569 & 18.955$\pm$0.179 & PO & u \\
252.5599 & 18.560$\pm$0.134 & PO & u \\
252.5629 & 18.937$\pm$0.168 & PO & u \\
252.5659 & 18.736$\pm$0.171 & PO & u \\
252.5689 & 19.095$\pm$0.231 & PO & u \\
252.5719 & 19.066$\pm$0.222 & PO & u \\
192.6423 & 16.777$\pm$0.055 & PO & g \\
192.6441 & 16.740$\pm$0.052 & PO & g \\
192.6460 & 16.672$\pm$0.046 & PO & g \\
192.7928 & 16.652$\pm$0.056 & PO & g \\
192.7946 & 16.703$\pm$0.055 & PO & g \\
192.7965 & 16.765$\pm$0.058 & PO & g \\
193.6261 & 16.719$\pm$0.047 & PO & g \\
193.6279 & 16.704$\pm$0.047 & PO & g \\
193.6298 & 16.717$\pm$0.047 & PO & g \\
195.6261 & 16.688$\pm$0.045 & PO & g \\
195.6279 & 16.687$\pm$0.046 & PO & g \\
195.6298 & 16.700$\pm$0.046 & PO & g \\
196.6279 & 16.626$\pm$0.043 & PO & g \\
196.6298 & 16.647$\pm$0.044 & PO & g \\
196.6316 & 16.669$\pm$0.044 & PO & g \\
197.6171 & 16.646$\pm$0.044 & PO & g \\
197.6189 & 16.646$\pm$0.044 & PO & g \\
197.6208 & 16.656$\pm$0.044 & PO & g \\
198.6121 & 16.722$\pm$0.046 & PO & g \\
198.6140 & 16.765$\pm$0.047 & PO & g \\
198.6158 & 16.776$\pm$0.047 & PO & g \\
198.7233 & 16.718$\pm$0.045 & PO & g \\
198.7251 & 16.676$\pm$0.044 & PO & g \\
198.7270 & 16.700$\pm$0.045 & PO & g \\
201.6053 & 16.845$\pm$0.049 & PO & g \\
201.6071 & 16.859$\pm$0.049 & PO & g \\
201.6090 & 16.831$\pm$0.048 & PO & g \\
201.7233 & 16.802$\pm$0.047 & PO & g \\
201.7251 & 16.825$\pm$0.048 & PO & g \\
201.7270 & 16.832$\pm$0.048 & PO & g \\
204.6051 & 16.851$\pm$0.048 & PO & g \\
204.6069 & 16.870$\pm$0.049 & PO & g \\
204.6088 & 16.840$\pm$0.048 & PO & g \\
204.7233 & 16.882$\pm$0.049 & PO & g \\
204.7251 & 16.858$\pm$0.049 & PO & g \\
204.7270 & 16.879$\pm$0.049 & PO & g \\
205.6053 & 16.951$\pm$0.051 & PO & g \\
205.6072 & 16.983$\pm$0.052 & PO & g \\
205.6090 & 16.899$\pm$0.050 & PO & g \\
205.7233 & 16.932$\pm$0.050 & PO & g \\
205.7251 & 16.934$\pm$0.050 & PO & g \\
205.7270 & 16.902$\pm$0.049 & PO & g \\
206.6845 & 16.979$\pm$0.052 & PO & g \\
206.6864 & 16.980$\pm$0.052 & PO & g \\
206.6882 & 16.972$\pm$0.051 & PO & g \\
206.7726 & 17.029$\pm$0.053 & PO & g \\
206.7745 & 17.063$\pm$0.055 & PO & g \\
206.7763 & 17.042$\pm$0.054 & PO & g \\
207.5912 & 16.919$\pm$0.050 & PO & g \\
207.5931 & 16.962$\pm$0.052 & PO & g \\
207.5949 & 16.922$\pm$0.050 & PO & g \\
210.6059 & 16.928$\pm$0.051 & PO & g \\
210.6078 & 16.889$\pm$0.050 & PO & g \\
210.6096 & 16.859$\pm$0.049 & PO & g \\
213.6059 & 17.047$\pm$0.055 & PO & g \\
213.6078 & 17.045$\pm$0.055 & PO & g \\
213.6096 & 17.051$\pm$0.056 & PO & g \\
214.6060 & 16.941$\pm$0.060 & PO & g \\
214.6079 & 16.924$\pm$0.060 & PO & g \\
214.6097 & 17.036$\pm$0.064 & PO & g \\
214.7189 & 17.023$\pm$0.068 & PO & g \\
214.7207 & 17.039$\pm$0.062 & PO & g \\
214.7226 & 17.075$\pm$0.062 & PO & g \\
215.6060 & 16.891$\pm$0.057 & PO & g \\
215.6079 & 16.915$\pm$0.059 & PO & g \\
215.6097 & 16.839$\pm$0.057 & PO & g \\
215.6116 & 17.003$\pm$0.061 & PO & g \\
215.6134 & 16.902$\pm$0.061 & PO & g \\
219.5885 & 16.971$\pm$0.056 & PO & g \\
219.5904 & 16.987$\pm$0.056 & PO & g \\
219.5922 & 17.052$\pm$0.058 & PO & g \\
219.5941 & 17.099$\pm$0.060 & PO & g \\
219.5960 & 17.111$\pm$0.063 & PO & g \\
219.6614 & 17.033$\pm$0.059 & PO & g \\
219.6632 & 17.052$\pm$0.060 & PO & g \\
219.6650 & 17.039$\pm$0.057 & PO & g \\
219.6669 & 17.159$\pm$0.068 & PO & g \\
219.6687 & 17.125$\pm$0.062 & PO & g \\
221.5914 & 16.956$\pm$0.055 & PO & g \\
221.5933 & 16.964$\pm$0.055 & PO & g \\
221.5951 & 16.929$\pm$0.055 & PO & g \\
221.5969 & 16.848$\pm$0.053 & PO & g \\
221.5988 & 16.897$\pm$0.054 & PO & g \\
221.6614 & 17.016$\pm$0.072 & PO & g \\
221.6632 & 16.935$\pm$0.055 & PO & g \\
221.6650 & 16.898$\pm$0.053 & PO & g \\
221.6669 & 16.917$\pm$0.053 & PO & g \\
221.6688 & 16.873$\pm$0.053 & PO & g \\
222.5888 & 16.935$\pm$0.051 & PO & g \\
222.5907 & 16.884$\pm$0.051 & PO & g \\
222.5925 & 16.957$\pm$0.052 & PO & g \\
222.5944 & 17.007$\pm$0.055 & PO & g \\
222.5962 & 16.947$\pm$0.052 & PO & g \\
222.6613 & 16.955$\pm$0.054 & PO & g \\
222.6632 & 17.001$\pm$0.056 & PO & g \\
222.6651 & 16.928$\pm$0.052 & PO & g \\
222.6669 & 16.957$\pm$0.053 & PO & g \\
222.6688 & 17.052$\pm$0.057 & PO & g \\
223.6468 & 16.983$\pm$0.054 & PO & g \\
223.6486 & 16.953$\pm$0.053 & PO & g \\
223.6505 & 16.947$\pm$0.053 & PO & g \\
223.6524 & 16.927$\pm$0.052 & PO & g \\
225.5781 & 17.094$\pm$0.055 & PO & g \\
225.5800 & 17.174$\pm$0.057 & PO & g \\
225.5818 & 17.087$\pm$0.054 & PO & g \\
225.5837 & 17.068$\pm$0.054 & PO & g \\
225.5855 & 17.079$\pm$0.054 & PO & g \\
225.6404 & 17.096$\pm$0.055 & PO & g \\
225.6423 & 17.111$\pm$0.055 & PO & g \\
225.6441 & 17.106$\pm$0.055 & PO & g \\
225.6460 & 17.098$\pm$0.056 & PO & g \\
225.6478 & 17.099$\pm$0.055 & PO & g \\
227.5846 & 17.219$\pm$0.057 & PO & g \\
227.5865 & 17.084$\pm$0.053 & PO & g \\
227.5883 & 17.063$\pm$0.053 & PO & g \\
227.5901 & 17.092$\pm$0.054 & PO & g \\
227.5920 & 17.062$\pm$0.053 & PO & g \\
228.6243 & 17.143$\pm$0.055 & PO & g \\
228.6261 & 17.177$\pm$0.056 & PO & g \\
228.6280 & 17.225$\pm$0.058 & PO & g \\
228.6298 & 17.156$\pm$0.056 & PO & g \\
228.6317 & 17.152$\pm$0.056 & PO & g \\
228.6770 & 17.174$\pm$0.057 & PO & g \\
228.6789 & 17.153$\pm$0.056 & PO & g \\
228.6807 & 17.088$\pm$0.054 & PO & g \\
228.6825 & 17.112$\pm$0.055 & PO & g \\
228.6844 & 17.211$\pm$0.058 & PO & g \\
229.5786 & 17.236$\pm$0.058 & PO & g \\
229.5805 & 17.187$\pm$0.057 & PO & g \\
229.5823 & 17.166$\pm$0.056 & PO & g \\
229.5842 & 17.215$\pm$0.058 & PO & g \\
229.5860 & 17.151$\pm$0.056 & PO & g \\
229.6404 & 17.123$\pm$0.055 & PO & g \\
229.6423 & 17.216$\pm$0.058 & PO & g \\
229.6441 & 17.166$\pm$0.056 & PO & g \\
229.6460 & 17.199$\pm$0.058 & PO & g \\
229.6479 & 17.187$\pm$0.057 & PO & g \\
230.6403 & 17.185$\pm$0.057 & PO & g \\
230.6422 & 17.160$\pm$0.056 & PO & g \\
230.6440 & 17.170$\pm$0.056 & PO & g \\
230.6459 & 17.204$\pm$0.057 & PO & g \\
230.6477 & 17.190$\pm$0.057 & PO & g \\
231.5679 & 17.271$\pm$0.059 & PO & g \\
231.5698 & 17.242$\pm$0.059 & PO & g \\
231.5716 & 17.239$\pm$0.059 & PO & g \\
231.5735 & 17.251$\pm$0.059 & PO & g \\
231.5753 & 17.196$\pm$0.057 & PO & g \\
232.6200 & 17.104$\pm$0.055 & PO & g \\
232.6224 & 17.091$\pm$0.054 & PO & g \\
232.6248 & 17.089$\pm$0.054 & PO & g \\
232.6273 & 17.147$\pm$0.056 & PO & g \\
232.6297 & 17.209$\pm$0.058 & PO & g \\
233.5574 & 17.077$\pm$0.054 & PO & g \\
233.5598 & 17.075$\pm$0.054 & PO & g \\
233.5623 & 17.135$\pm$0.056 & PO & g \\
233.5648 & 17.105$\pm$0.055 & PO & g \\
233.5673 & 17.131$\pm$0.056 & PO & g \\
235.6321 & 17.277$\pm$0.060 & PO & g \\
235.6345 & 17.270$\pm$0.060 & PO & g \\
235.6370 & 17.401$\pm$0.064 & PO & g \\
235.6395 & 17.358$\pm$0.063 & PO & g \\
235.6419 & 17.345$\pm$0.062 & PO & g \\
236.6455 & 17.156$\pm$0.056 & PO & g \\
236.6479 & 17.145$\pm$0.056 & PO & g \\
236.6503 & 17.163$\pm$0.056 & PO & g \\
236.6528 & 17.188$\pm$0.057 & PO & g \\
236.6553 & 17.165$\pm$0.056 & PO & g \\
237.6748 & 17.275$\pm$0.059 & PO & g \\
237.6772 & 17.269$\pm$0.059 & PO & g \\
237.6797 & 17.253$\pm$0.059 & PO & g \\
237.6821 & 17.291$\pm$0.060 & PO & g \\
237.6845 & 17.276$\pm$0.060 & PO & g \\
238.6335 & 17.350$\pm$0.061 & PO & g \\
238.6359 & 17.263$\pm$0.059 & PO & g \\
238.6384 & 17.246$\pm$0.058 & PO & g \\
238.6408 & 17.272$\pm$0.059 & PO & g \\
238.6432 & 17.270$\pm$0.059 & PO & g \\
240.5737 & 17.180$\pm$0.056 & PO & g \\
240.5762 & 17.192$\pm$0.057 & PO & g \\
240.5786 & 17.189$\pm$0.057 & PO & g \\
240.5811 & 17.203$\pm$0.057 & PO & g \\
240.5835 & 17.211$\pm$0.057 & PO & g \\
240.6456 & 17.219$\pm$0.057 & PO & g \\
240.6480 & 17.191$\pm$0.057 & PO & g \\
240.6505 & 17.225$\pm$0.060 & PO & g \\
240.6529 & 17.222$\pm$0.059 & PO & g \\
240.6553 & 17.193$\pm$0.057 & PO & g \\
241.5802 & 17.286$\pm$0.062 & PO & g \\
241.5827 & 17.307$\pm$0.063 & PO & g \\
241.5852 & 17.197$\pm$0.060 & PO & g \\
241.5877 & 17.326$\pm$0.067 & PO & g \\
241.5901 & 17.359$\pm$0.068 & PO & g \\
247.6098 & 17.140$\pm$0.057 & PO & g \\
247.6122 & 17.105$\pm$0.057 & PO & g \\
247.6146 & 17.108$\pm$0.055 & PO & g \\
247.6171 & 17.119$\pm$0.056 & PO & g \\
247.6195 & 17.133$\pm$0.056 & PO & g \\
247.6819 & 17.211$\pm$0.068 & PO & g \\
247.6844 & 17.214$\pm$0.066 & PO & g \\
247.6868 & 17.065$\pm$0.064 & PO & g \\
247.6892 & 17.224$\pm$0.065 & PO & g \\
247.6917 & 17.133$\pm$0.067 & PO & g \\
248.5958 & 17.141$\pm$0.057 & PO & g \\
248.5983 & 17.125$\pm$0.059 & PO & g \\
248.6007 & 17.269$\pm$0.064 & PO & g \\
248.6032 & 17.226$\pm$0.060 & PO & g \\
248.6056 & 17.176$\pm$0.061 & PO & g \\
249.5743 & 17.199$\pm$0.062 & PO & g \\
249.5768 & 17.329$\pm$0.065 & PO & g \\
249.5792 & 17.294$\pm$0.067 & PO & g \\
249.5817 & 17.259$\pm$0.062 & PO & g \\
249.5841 & 17.281$\pm$0.064 & PO & g \\
250.5788 & 17.241$\pm$0.069 & PO & g \\
250.5813 & 17.329$\pm$0.065 & PO & g \\
250.5837 & 17.230$\pm$0.086 & PO & g \\
250.5861 & 17.302$\pm$0.070 & PO & g \\
250.5885 & 17.301$\pm$0.068 & PO & g \\
251.6110 & 17.134$\pm$0.128 & PO & g \\
251.6134 & 17.197$\pm$0.122 & PO & g \\
251.6159 & 17.218$\pm$0.093 & PO & g \\
251.6183 & 17.265$\pm$0.110 & PO & g \\
251.6208 & 17.110$\pm$0.091 & PO & g \\
252.5780 & 17.475$\pm$0.071 & PO & g \\
252.5805 & 17.316$\pm$0.064 & PO & g \\
252.5829 & 17.351$\pm$0.065 & PO & g \\
252.5854 & 17.310$\pm$0.063 & PO & g \\
252.5878 & 17.350$\pm$0.065 & PO & g \\
253.5631 & 17.401$\pm$0.063 & PO & g \\
253.5661 & 17.343$\pm$0.062 & PO & g \\
253.5691 & 17.393$\pm$0.063 & PO & g \\
253.5721 & 17.349$\pm$0.062 & PO & g \\
253.5751 & 17.486$\pm$0.071 & PO & g \\
254.5564 & 17.408$\pm$0.063 & PO & g \\
254.5594 & 17.458$\pm$0.067 & PO & g \\
254.5624 & 17.436$\pm$0.064 & PO & g \\
254.5655 & 17.437$\pm$0.065 & PO & g \\
254.5685 & 17.461$\pm$0.065 & PO & g \\
255.5565 & 17.357$\pm$0.063 & PO & g \\
255.5595 & 17.348$\pm$0.062 & PO & g \\
255.5625 & 17.465$\pm$0.067 & PO & g \\
255.5655 & 17.512$\pm$0.067 & PO & g \\
255.5685 & 17.333$\pm$0.063 & PO & g \\
256.5565 & 17.618$\pm$0.071 & PO & g \\
256.5595 & 17.571$\pm$0.069 & PO & g \\
256.5625 & 17.583$\pm$0.069 & PO & g \\
256.5655 & 17.297$\pm$0.061 & PO & g \\
256.5685 & 17.479$\pm$0.066 & PO & g \\
257.5664 & 17.438$\pm$0.065 & PO & g \\
257.5694 & 17.447$\pm$0.065 & PO & g \\
257.5725 & 17.388$\pm$0.063 & PO & g \\
257.5755 & 17.407$\pm$0.063 & PO & g \\
257.5785 & 17.382$\pm$0.063 & PO & g \\
259.5814 & 17.264$\pm$0.059 & PO & g \\
259.5844 & 17.301$\pm$0.060 & PO & g \\
259.5875 & 17.241$\pm$0.058 & PO & g \\
259.5905 & 17.249$\pm$0.059 & PO & g \\
259.5936 & 17.291$\pm$0.060 & PO & g \\
263.5785 & 17.080$\pm$0.054 & PO & g \\
263.5809 & 17.068$\pm$0.053 & PO & g \\
263.5834 & 17.082$\pm$0.053 & PO & g \\
263.5858 & 17.110$\pm$0.054 & PO & g \\
263.5882 & 17.136$\pm$0.055 & PO & g \\
263.5906 & 17.127$\pm$0.055 & PO & g \\
264.5669 & 17.266$\pm$0.060 & PO & g \\
264.5694 & 17.247$\pm$0.060 & PO & g \\
264.5718 & 17.266$\pm$0.059 & PO & g \\
264.5742 & 17.308$\pm$0.061 & PO & g \\
264.5766 & 17.295$\pm$0.061 & PO & g \\
264.5791 & 17.341$\pm$0.062 & PO & g \\
265.5670 & 17.361$\pm$0.063 & PO & g \\
265.5694 & 17.337$\pm$0.062 & PO & g \\
265.5718 & 17.310$\pm$0.060 & PO & g \\
265.5742 & 17.326$\pm$0.061 & PO & g \\
265.5766 & 17.296$\pm$0.060 & PO & g \\
265.5790 & 17.311$\pm$0.060 & PO & g \\
266.5670 & 17.340$\pm$0.061 & PO & g \\
266.5694 & 17.311$\pm$0.060 & PO & g \\
266.5719 & 17.308$\pm$0.060 & PO & g \\
266.5743 & 17.344$\pm$0.061 & PO & g \\
266.5767 & 17.367$\pm$0.062 & PO & g \\
266.5792 & 17.319$\pm$0.060 & PO & g \\
267.5567 & 17.606$\pm$0.076 & PO & g \\
267.5592 & 17.611$\pm$0.077 & PO & g \\
267.5617 & 17.483$\pm$0.067 & PO & g \\
267.5641 & 17.440$\pm$0.064 & PO & g \\
267.5665 & 17.486$\pm$0.066 & PO & g \\
267.5690 & 17.506$\pm$0.067 & PO & g \\
270.5785 & 17.627$\pm$0.073 & PO & g \\
270.5809 & 17.610$\pm$0.074 & PO & g \\
270.5833 & 17.787$\pm$0.082 & PO & g \\
270.5858 & 17.630$\pm$0.074 & PO & g \\
270.5882 & 17.663$\pm$0.075 & PO & g \\
271.5641 & 17.770$\pm$0.082 & PO & g \\
271.5665 & 17.773$\pm$0.084 & PO & g \\
271.5690 & 17.717$\pm$0.076 & PO & g \\
271.5715 & 17.971$\pm$0.100 & PO & g \\
271.5739 & 17.742$\pm$0.077 & PO & g \\
272.5637 & 18.021$\pm$0.112 & PO & g \\
272.5662 & 17.984$\pm$0.099 & PO & g \\
272.5686 & 17.967$\pm$0.095 & PO & g \\
272.5711 & 17.985$\pm$0.102 & PO & g \\
272.5736 & 17.798$\pm$0.086 & PO & g \\
273.5637 & 17.865$\pm$0.085 & PO & g \\
273.5662 & 17.965$\pm$0.096 & PO & g \\
273.5686 & 18.022$\pm$0.094 & PO & g \\
273.5710 & 18.111$\pm$0.095 & PO & g \\
273.5735 & 18.096$\pm$0.098 & PO & g \\
274.5636 & 18.004$\pm$0.097 & PO & g \\
274.5666 & 18.026$\pm$0.100 & PO & g \\
274.5696 & 17.936$\pm$0.088 & PO & g \\
274.5726 & 18.166$\pm$0.100 & PO & g \\
274.5756 & 18.085$\pm$0.097 & PO & g \\
274.5786 & 18.037$\pm$0.091 & PO & g \\
275.5688 & 18.325$\pm$0.111 & PO & g \\
275.5718 & 18.133$\pm$0.103 & PO & g \\
275.5748 & 18.282$\pm$0.114 & PO & g \\
275.5778 & 18.287$\pm$0.108 & PO & g \\
275.5808 & 18.194$\pm$0.101 & PO & g \\
275.5838 & 18.088$\pm$0.097 & PO & g \\
276.5845 & 18.472$\pm$0.176 & PO & g \\
276.5876 & 18.363$\pm$0.127 & PO & g \\
276.5907 & 18.303$\pm$0.123 & PO & g \\
276.5937 & 18.674$\pm$0.169 & PO & g \\
276.5967 & 18.268$\pm$0.120 & PO & g \\
276.5996 & 18.219$\pm$0.119 & PO & g \\
277.5667 & 18.327$\pm$0.125 & PO & g \\
277.5697 & 18.459$\pm$0.125 & PO & g \\
277.5727 & 18.347$\pm$0.120 & PO & g \\
277.5757 & 18.298$\pm$0.113 & PO & g \\
277.5787 & 18.113$\pm$0.101 & PO & g \\
278.5667 & 18.239$\pm$0.114 & PO & g \\
278.5697 & 18.594$\pm$0.140 & PO & g \\
278.5727 & 18.668$\pm$0.150 & PO & g \\
278.5757 & 18.632$\pm$0.158 & PO & g \\
278.5787 & 18.440$\pm$0.132 & PO & g \\
280.5673 & 18.744$\pm$0.214 & PO & g \\
280.5703 & 18.905$\pm$0.209 & PO & g \\
280.5733 & 18.473$\pm$0.147 & PO & g \\
280.5763 & 18.449$\pm$0.170 & PO & g \\
280.5795 & 19.048$\pm$0.208 & PO & g \\
281.5671 & 19.196$\pm$0.305 & PO & g \\
281.5701 & 18.581$\pm$0.170 & PO & g \\
281.5731 & 18.800$\pm$0.184 & PO & g \\
281.5761 & 19.051$\pm$0.225 & PO & g \\
281.5791 & 18.826$\pm$0.207 & PO & g \\
282.5798 & 19.247$\pm$0.209 & PO & g \\
282.5828 & 19.703$\pm$0.295 & PO & g \\
282.5858 & 19.787$\pm$0.415 & PO & g \\
284.5707 & 19.293$\pm$0.221 & PO & g \\
284.5737 & 19.869$\pm$0.315 & PO & g \\
284.5767 & 19.908$\pm$0.321 & PO & g \\
286.5707 & 20.520$\pm$0.745 & PO & g \\
286.5737 & 20.083$\pm$0.433 & PO & g \\
286.5767 & 19.875$\pm$0.269 & PO & g \\
288.5742 & 20.129$\pm$0.457 & PO & g \\
192.6479 & 16.703$\pm$0.056 & PO & r \\
192.6498 & 16.599$\pm$0.053 & PO & r \\
192.6516 & 16.668$\pm$0.055 & PO & r \\
192.7983 & 16.555$\pm$0.054 & PO & r \\
192.8002 & 16.584$\pm$0.054 & PO & r \\
192.8021 & 16.704$\pm$0.057 & PO & r \\
193.6317 & 16.642$\pm$0.051 & PO & r \\
193.6336 & 16.647$\pm$0.050 & PO & r \\
193.6354 & 16.632$\pm$0.050 & PO & r \\
195.6317 & 16.616$\pm$0.050 & PO & r \\
195.6336 & 16.548$\pm$0.049 & PO & r \\
195.6354 & 16.585$\pm$0.049 & PO & r \\
196.6336 & 16.574$\pm$0.049 & PO & r \\
196.6354 & 16.590$\pm$0.049 & PO & r \\
196.6373 & 16.580$\pm$0.049 & PO & r \\
197.6227 & 16.621$\pm$0.050 & PO & r \\
197.6246 & 16.584$\pm$0.049 & PO & r \\
197.6264 & 16.643$\pm$0.050 & PO & r \\
198.6177 & 16.625$\pm$0.050 & PO & r \\
198.6196 & 16.651$\pm$0.050 & PO & r \\
198.6214 & 16.615$\pm$0.050 & PO & r \\
198.7289 & 16.658$\pm$0.051 & PO & r \\
198.7308 & 16.673$\pm$0.051 & PO & r \\
198.7326 & 16.666$\pm$0.051 & PO & r \\
201.6109 & 16.737$\pm$0.053 & PO & r \\
201.6128 & 16.711$\pm$0.052 & PO & r \\
201.6146 & 16.728$\pm$0.052 & PO & r \\
201.7289 & 16.721$\pm$0.052 & PO & r \\
201.7308 & 16.668$\pm$0.051 & PO & r \\
201.7326 & 16.722$\pm$0.052 & PO & r \\
204.6107 & 16.790$\pm$0.053 & PO & r \\
204.6125 & 16.806$\pm$0.054 & PO & r \\
204.6144 & 16.778$\pm$0.053 & PO & r \\
204.7288 & 16.763$\pm$0.053 & PO & r \\
204.7307 & 16.735$\pm$0.052 & PO & r \\
204.7325 & 16.772$\pm$0.053 & PO & r \\
205.6110 & 16.828$\pm$0.054 & PO & r \\
205.6128 & 16.848$\pm$0.054 & PO & r \\
205.6146 & 16.830$\pm$0.054 & PO & r \\
205.7288 & 16.837$\pm$0.055 & PO & r \\
205.7307 & 16.789$\pm$0.054 & PO & r \\
205.7325 & 16.850$\pm$0.055 & PO & r \\
206.6902 & 16.873$\pm$0.055 & PO & r \\
206.6920 & 16.879$\pm$0.056 & PO & r \\
206.6938 & 16.870$\pm$0.056 & PO & r \\
206.7782 & 16.971$\pm$0.059 & PO & r \\
206.7801 & 16.937$\pm$0.057 & PO & r \\
206.7819 & 16.708$\pm$0.056 & PO & r \\
207.5969 & 16.841$\pm$0.055 & PO & r \\
207.5987 & 16.841$\pm$0.055 & PO & r \\
207.6005 & 16.830$\pm$0.054 & PO & r \\
207.6851 & 16.634$\pm$0.085 & PO & r \\
207.6888 & 16.556$\pm$0.079 & PO & r \\
210.6116 & 16.846$\pm$0.056 & PO & r \\
210.6134 & 16.848$\pm$0.056 & PO & r \\
210.6152 & 16.832$\pm$0.056 & PO & r \\
213.6116 & 16.918$\pm$0.057 & PO & r \\
213.6134 & 16.872$\pm$0.056 & PO & r \\
213.6152 & 16.904$\pm$0.057 & PO & r \\
214.6116 & 16.760$\pm$0.067 & PO & r \\
214.6135 & 16.690$\pm$0.063 & PO & r \\
214.6154 & 16.790$\pm$0.067 & PO & r \\
214.7245 & 16.816$\pm$0.064 & PO & r \\
214.7263 & 16.810$\pm$0.062 & PO & r \\
214.7282 & 16.722$\pm$0.060 & PO & r \\
215.6153 & 16.799$\pm$0.102 & PO & r \\
215.6209 & 16.803$\pm$0.086 & PO & r \\
219.5979 & 16.958$\pm$0.059 & PO & r \\
219.5997 & 16.921$\pm$0.058 & PO & r \\
219.6015 & 16.909$\pm$0.058 & PO & r \\
219.6034 & 16.941$\pm$0.059 & PO & r \\
219.6053 & 16.969$\pm$0.060 & PO & r \\
219.6706 & 17.049$\pm$0.063 & PO & r \\
219.6724 & 16.940$\pm$0.059 & PO & r \\
219.6743 & 17.005$\pm$0.063 & PO & r \\
219.6761 & 17.021$\pm$0.060 & PO & r \\
219.6780 & 16.925$\pm$0.060 & PO & r \\
221.6007 & 16.818$\pm$0.057 & PO & r \\
221.6026 & 16.855$\pm$0.058 & PO & r \\
221.6044 & 16.891$\pm$0.060 & PO & r \\
221.6063 & 16.836$\pm$0.058 & PO & r \\
221.6081 & 16.837$\pm$0.057 & PO & r \\
221.6707 & 16.868$\pm$0.057 & PO & r \\
221.6725 & 16.837$\pm$0.056 & PO & r \\
221.6744 & 16.831$\pm$0.057 & PO & r \\
221.6762 & 16.838$\pm$0.057 & PO & r \\
221.6781 & 16.838$\pm$0.057 & PO & r \\
222.5981 & 16.931$\pm$0.057 & PO & r \\
222.6000 & 16.918$\pm$0.057 & PO & r \\
222.6018 & 16.928$\pm$0.057 & PO & r \\
222.6037 & 16.922$\pm$0.057 & PO & r \\
222.6055 & 16.917$\pm$0.057 & PO & r \\
222.6707 & 16.916$\pm$0.058 & PO & r \\
222.6726 & 16.967$\pm$0.059 & PO & r \\
222.6745 & 16.903$\pm$0.057 & PO & r \\
222.6763 & 16.916$\pm$0.057 & PO & r \\
222.6782 & 16.954$\pm$0.059 & PO & r \\
223.6543 & 16.903$\pm$0.057 & PO & r \\
223.6561 & 16.881$\pm$0.057 & PO & r \\
223.6580 & 16.850$\pm$0.057 & PO & r \\
223.6599 & 16.929$\pm$0.060 & PO & r \\
225.5875 & 16.997$\pm$0.058 & PO & r \\
225.5893 & 17.041$\pm$0.058 & PO & r \\
225.5911 & 16.991$\pm$0.057 & PO & r \\
225.5930 & 16.968$\pm$0.057 & PO & r \\
225.5948 & 16.982$\pm$0.057 & PO & r \\
225.6497 & 17.002$\pm$0.057 & PO & r \\
225.6516 & 17.002$\pm$0.058 & PO & r \\
225.6534 & 17.096$\pm$0.062 & PO & r \\
225.6553 & 17.070$\pm$0.062 & PO & r \\
225.6572 & 17.112$\pm$0.062 & PO & r \\
227.5939 & 17.005$\pm$0.057 & PO & r \\
227.5958 & 16.999$\pm$0.057 & PO & r \\
227.5976 & 17.027$\pm$0.057 & PO & r \\
227.5995 & 17.036$\pm$0.058 & PO & r \\
227.6015 & 17.040$\pm$0.058 & PO & r \\
228.6336 & 17.068$\pm$0.058 & PO & r \\
228.6355 & 17.056$\pm$0.058 & PO & r \\
228.6373 & 17.089$\pm$0.059 & PO & r \\
228.6393 & 17.096$\pm$0.059 & PO & r \\
228.6411 & 17.081$\pm$0.059 & PO & r \\
228.6863 & 17.051$\pm$0.058 & PO & r \\
228.6881 & 17.048$\pm$0.059 & PO & r \\
228.6900 & 17.084$\pm$0.060 & PO & r \\
228.6919 & 17.031$\pm$0.058 & PO & r \\
228.6937 & 17.033$\pm$0.058 & PO & r \\
229.5879 & 17.072$\pm$0.059 & PO & r \\
229.5898 & 17.057$\pm$0.059 & PO & r \\
229.5916 & 17.085$\pm$0.060 & PO & r \\
229.5935 & 17.081$\pm$0.060 & PO & r \\
229.5953 & 17.040$\pm$0.059 & PO & r \\
229.6498 & 17.056$\pm$0.058 & PO & r \\
229.6516 & 17.064$\pm$0.059 & PO & r \\
229.6535 & 17.106$\pm$0.060 & PO & r \\
229.6554 & 17.058$\pm$0.059 & PO & r \\
229.6572 & 17.129$\pm$0.061 & PO & r \\
230.6496 & 17.127$\pm$0.060 & PO & r \\
230.6515 & 17.131$\pm$0.060 & PO & r \\
230.6533 & 17.121$\pm$0.060 & PO & r \\
230.6552 & 17.170$\pm$0.062 & PO & r \\
230.6570 & 17.135$\pm$0.060 & PO & r \\
231.5773 & 17.164$\pm$0.063 & PO & r \\
231.5791 & 17.144$\pm$0.061 & PO & r \\
231.5810 & 17.100$\pm$0.061 & PO & r \\
231.5829 & 17.190$\pm$0.064 & PO & r \\
231.5847 & 17.102$\pm$0.061 & PO & r \\
232.6321 & 17.039$\pm$0.060 & PO & r \\
232.6346 & 17.077$\pm$0.060 & PO & r \\
232.6370 & 17.066$\pm$0.059 & PO & r \\
232.6394 & 17.115$\pm$0.061 & PO & r \\
233.5697 & 16.984$\pm$0.057 & PO & r \\
233.5721 & 17.001$\pm$0.058 & PO & r \\
233.5746 & 17.010$\pm$0.058 & PO & r \\
233.5772 & 17.022$\pm$0.058 & PO & r \\
235.6443 & 17.090$\pm$0.061 & PO & r \\
235.6468 & 17.227$\pm$0.065 & PO & r \\
235.6492 & 17.215$\pm$0.064 & PO & r \\
235.6517 & 17.252$\pm$0.066 & PO & r \\
236.6577 & 17.114$\pm$0.060 & PO & r \\
236.6602 & 17.122$\pm$0.060 & PO & r \\
236.6626 & 17.115$\pm$0.060 & PO & r \\
236.6650 & 17.133$\pm$0.061 & PO & r \\
237.6872 & 17.163$\pm$0.062 & PO & r \\
237.6896 & 17.063$\pm$0.059 & PO & r \\
237.6920 & 17.166$\pm$0.062 & PO & r \\
237.6945 & 17.181$\pm$0.062 & PO & r \\
238.6457 & 17.174$\pm$0.062 & PO & r \\
238.6481 & 17.153$\pm$0.062 & PO & r \\
238.6506 & 17.135$\pm$0.061 & PO & r \\
238.6530 & 17.116$\pm$0.060 & PO & r \\
240.5860 & 17.132$\pm$0.060 & PO & r \\
240.5884 & 17.158$\pm$0.061 & PO & r \\
240.5909 & 17.139$\pm$0.060 & PO & r \\
240.5933 & 17.118$\pm$0.060 & PO & r \\
240.5959 & 17.118$\pm$0.060 & PO & r \\
240.6578 & 17.257$\pm$0.081 & PO & r \\
240.6602 & 17.290$\pm$0.085 & PO & r \\
240.6628 & 17.177$\pm$0.066 & PO & r \\
240.6653 & 17.113$\pm$0.061 & PO & r \\
240.6677 & 17.205$\pm$0.064 & PO & r \\
241.5926 & 17.169$\pm$0.070 & PO & r \\
241.5950 & 17.295$\pm$0.074 & PO & r \\
241.5975 & 17.138$\pm$0.069 & PO & r \\
241.5999 & 17.491$\pm$0.086 & PO & r \\
241.6024 & 17.213$\pm$0.071 & PO & r \\
247.6220 & 17.108$\pm$0.060 & PO & r \\
247.6244 & 17.080$\pm$0.061 & PO & r \\
247.6269 & 17.147$\pm$0.062 & PO & r \\
247.6293 & 17.155$\pm$0.063 & PO & r \\
247.6319 & 17.064$\pm$0.060 & PO & r \\
248.6080 & 17.101$\pm$0.062 & PO & r \\
248.6105 & 17.126$\pm$0.062 & PO & r \\
248.6131 & 17.109$\pm$0.062 & PO & r \\
248.6155 & 17.080$\pm$0.061 & PO & r \\
248.6180 & 17.140$\pm$0.063 & PO & r \\
249.5890 & 17.221$\pm$0.068 & PO & r \\
249.5914 & 17.220$\pm$0.066 & PO & r \\
249.5938 & 17.136$\pm$0.062 & PO & r \\
249.5965 & 17.202$\pm$0.064 & PO & r \\
250.5911 & 17.176$\pm$0.067 & PO & r \\
250.5935 & 17.237$\pm$0.069 & PO & r \\
250.5960 & 17.203$\pm$0.068 & PO & r \\
250.5984 & 17.211$\pm$0.066 & PO & r \\
250.6008 & 17.223$\pm$0.068 & PO & r \\
251.6234 & 17.426$\pm$0.111 & PO & r \\
251.6259 & 16.976$\pm$0.117 & PO & r \\
251.6283 & 17.077$\pm$0.106 & PO & r \\
251.6308 & 17.171$\pm$0.097 & PO & r \\
251.6332 & 17.433$\pm$0.100 & PO & r \\
252.5902 & 17.215$\pm$0.065 & PO & r \\
252.5927 & 17.209$\pm$0.064 & PO & r \\
252.5953 & 17.278$\pm$0.066 & PO & r \\
252.5977 & 17.230$\pm$0.065 & PO & r \\
252.6002 & 17.280$\pm$0.066 & PO & r \\
253.5781 & 17.224$\pm$0.064 & PO & r \\
253.5806 & 17.313$\pm$0.068 & PO & r \\
253.5830 & 17.310$\pm$0.068 & PO & r \\
253.5854 & 17.301$\pm$0.066 & PO & r \\
253.5878 & 17.309$\pm$0.068 & PO & r \\
254.5715 & 17.395$\pm$0.070 & PO & r \\
254.5739 & 17.290$\pm$0.067 & PO & r \\
254.5764 & 17.292$\pm$0.066 & PO & r \\
254.5788 & 17.349$\pm$0.067 & PO & r \\
254.5812 & 17.343$\pm$0.067 & PO & r \\
255.5715 & 17.205$\pm$0.071 & PO & r \\
255.5739 & 17.318$\pm$0.082 & PO & r \\
255.5764 & 17.501$\pm$0.117 & PO & r \\
255.5788 & 17.412$\pm$0.105 & PO & r \\
255.5812 & 17.361$\pm$0.084 & PO & r \\
256.5716 & 17.379$\pm$0.069 & PO & r \\
256.5740 & 17.381$\pm$0.069 & PO & r \\
256.5764 & 17.322$\pm$0.067 & PO & r \\
256.5789 & 17.330$\pm$0.067 & PO & r \\
256.5813 & 17.341$\pm$0.067 & PO & r \\
257.5815 & 17.323$\pm$0.067 & PO & r \\
257.5840 & 17.278$\pm$0.065 & PO & r \\
257.5864 & 17.301$\pm$0.066 & PO & r \\
257.5888 & 17.312$\pm$0.066 & PO & r \\
257.5912 & 17.299$\pm$0.065 & PO & r \\
259.5966 & 17.229$\pm$0.064 & PO & r \\
259.5990 & 17.243$\pm$0.064 & PO & r \\
259.6015 & 17.178$\pm$0.063 & PO & r \\
259.6039 & 17.264$\pm$0.065 & PO & r \\
259.6063 & 17.133$\pm$0.062 & PO & r \\
263.5931 & 17.136$\pm$0.061 & PO & r \\
263.5955 & 17.170$\pm$0.062 & PO & r \\
263.5980 & 17.072$\pm$0.059 & PO & r \\
263.6004 & 17.130$\pm$0.060 & PO & r \\
263.6029 & 17.086$\pm$0.059 & PO & r \\
263.6053 & 17.114$\pm$0.060 & PO & r \\
264.5816 & 17.194$\pm$0.064 & PO & r \\
264.5840 & 17.198$\pm$0.066 & PO & r \\
264.5864 & 17.242$\pm$0.068 & PO & r \\
264.5888 & 17.253$\pm$0.067 & PO & r \\
264.5913 & 17.315$\pm$0.068 & PO & r \\
264.5937 & 17.229$\pm$0.065 & PO & r \\
265.5815 & 17.258$\pm$0.065 & PO & r \\
265.5839 & 17.330$\pm$0.067 & PO & r \\
265.5864 & 17.280$\pm$0.065 & PO & r \\
265.5888 & 17.279$\pm$0.066 & PO & r \\
265.5912 & 17.276$\pm$0.065 & PO & r \\
265.5937 & 17.202$\pm$0.063 & PO & r \\
266.5816 & 17.302$\pm$0.065 & PO & r \\
266.5840 & 17.361$\pm$0.067 & PO & r \\
266.5865 & 17.399$\pm$0.069 & PO & r \\
266.5889 & 17.318$\pm$0.066 & PO & r \\
266.5914 & 17.318$\pm$0.065 & PO & r \\
266.5940 & 17.371$\pm$0.067 & PO & r \\
267.5715 & 17.441$\pm$0.071 & PO & r \\
267.5739 & 17.438$\pm$0.070 & PO & r \\
267.5763 & 17.420$\pm$0.073 & PO & r \\
267.5787 & 17.455$\pm$0.071 & PO & r \\
267.5814 & 17.427$\pm$0.070 & PO & r \\
267.5838 & 17.449$\pm$0.071 & PO & r \\
270.5907 & 17.596$\pm$0.078 & PO & r \\
270.5932 & 17.671$\pm$0.080 & PO & r \\
270.5956 & 17.627$\pm$0.077 & PO & r \\
270.5980 & 17.643$\pm$0.080 & PO & r \\
270.6006 & 17.589$\pm$0.076 & PO & r \\
271.5763 & 17.614$\pm$0.081 & PO & r \\
271.5788 & 17.677$\pm$0.084 & PO & r \\
271.5812 & 17.699$\pm$0.087 & PO & r \\
271.5837 & 17.534$\pm$0.077 & PO & r \\
271.5861 & 17.688$\pm$0.086 & PO & r \\
272.5760 & 17.710$\pm$0.091 & PO & r \\
272.5784 & 17.927$\pm$0.104 & PO & r \\
272.5809 & 17.558$\pm$0.087 & PO & r \\
272.5833 & 17.675$\pm$0.096 & PO & r \\
272.5857 & 18.197$\pm$0.130 & PO & r \\
273.5759 & 17.846$\pm$0.087 & PO & r \\
273.5784 & 17.976$\pm$0.098 & PO & r \\
273.5810 & 18.040$\pm$0.100 & PO & r \\
273.5834 & 17.929$\pm$0.095 & PO & r \\
273.5859 & 17.929$\pm$0.094 & PO & r \\
274.5840 & 17.988$\pm$0.097 & PO & r \\
274.5870 & 18.136$\pm$0.100 & PO & r \\
274.5902 & 17.991$\pm$0.094 & PO & r \\
274.5932 & 18.053$\pm$0.098 & PO & r \\
274.5962 & 18.005$\pm$0.095 & PO & r \\
274.5993 & 17.923$\pm$0.093 & PO & r \\
275.5871 & 18.059$\pm$0.100 & PO & r \\
275.5901 & 18.004$\pm$0.093 & PO & r \\
275.5931 & 18.028$\pm$0.100 & PO & r \\
275.5961 & 18.452$\pm$0.131 & PO & r \\
275.5991 & 18.235$\pm$0.112 & PO & r \\
275.6021 & 17.861$\pm$0.098 & PO & r \\
276.5664 & 18.212$\pm$0.114 & PO & r \\
276.5694 & 18.084$\pm$0.136 & PO & r \\
276.5724 & 18.083$\pm$0.115 & PO & r \\
276.5754 & 18.232$\pm$0.116 & PO & r \\
276.5784 & 18.669$\pm$0.172 & PO & r \\
276.5814 & 18.409$\pm$0.156 & PO & r \\
282.5708 & 18.916$\pm$0.208 & PO & r \\
282.5737 & 18.985$\pm$0.228 & PO & r \\
282.5767 & 18.843$\pm$0.185 & PO & r \\
290.5743 & 20.178$\pm$0.698 & PO & r \\
290.5773 & 20.331$\pm$0.616 & PO & r \\
290.5803 & 19.757$\pm$0.362 & PO & r \\
193.6374 & 16.394$\pm$0.041 & PO & i \\
193.6392 & 16.387$\pm$0.040 & PO & i \\
193.6411 & 16.324$\pm$0.039 & PO & i \\
195.6374 & 16.283$\pm$0.039 & PO & i \\
195.6392 & 16.282$\pm$0.038 & PO & i \\
195.6411 & 16.264$\pm$0.038 & PO & i \\
196.6392 & 16.292$\pm$0.038 & PO & i \\
196.6411 & 16.281$\pm$0.038 & PO & i \\
196.6429 & 16.259$\pm$0.038 & PO & i \\
197.6284 & 16.287$\pm$0.039 & PO & i \\
197.6302 & 16.290$\pm$0.039 & PO & i \\
197.6321 & 16.306$\pm$0.040 & PO & i \\
198.6234 & 16.388$\pm$0.040 & PO & i \\
198.6252 & 16.371$\pm$0.040 & PO & i \\
198.6273 & 16.390$\pm$0.041 & PO & i \\
201.6166 & 16.412$\pm$0.042 & PO & i \\
201.6184 & 16.428$\pm$0.042 & PO & i \\
201.6203 & 16.398$\pm$0.041 & PO & i \\
204.6163 & 16.483$\pm$0.042 & PO & i \\
204.6181 & 16.457$\pm$0.041 & PO & i \\
204.6200 & 16.473$\pm$0.042 & PO & i \\
204.7344 & 16.492$\pm$0.042 & PO & i \\
204.7362 & 16.518$\pm$0.043 & PO & i \\
204.7381 & 16.519$\pm$0.043 & PO & i \\
205.6165 & 16.626$\pm$0.045 & PO & i \\
205.6184 & 16.555$\pm$0.044 & PO & i \\
205.6203 & 16.635$\pm$0.046 & PO & i \\
205.7344 & 16.551$\pm$0.045 & PO & i \\
205.7363 & 16.519$\pm$0.045 & PO & i \\
205.7381 & 16.566$\pm$0.045 & PO & i \\
206.6958 & 16.587$\pm$0.045 & PO & i \\
206.6976 & 16.571$\pm$0.045 & PO & i \\
206.6995 & 16.658$\pm$0.047 & PO & i \\
206.7838 & 16.916$\pm$0.071 & PO & i \\
206.7857 & 16.992$\pm$0.066 & PO & i \\
206.7875 & 16.732$\pm$0.059 & PO & i \\
207.6025 & 16.598$\pm$0.046 & PO & i \\
207.6043 & 16.589$\pm$0.045 & PO & i \\
207.6062 & 16.580$\pm$0.045 & PO & i \\
207.6908 & 16.482$\pm$0.103 & PO & i \\
207.6926 & 16.251$\pm$0.063 & PO & i \\
210.6171 & 16.443$\pm$0.044 & PO & i \\
210.6190 & 16.478$\pm$0.045 & PO & i \\
210.6209 & 16.474$\pm$0.044 & PO & i \\
213.6171 & 16.591$\pm$0.046 & PO & i \\
213.6190 & 16.594$\pm$0.047 & PO & i \\
213.6209 & 16.602$\pm$0.047 & PO & i \\
214.6173 & 16.811$\pm$0.104 & PO & i \\
214.6191 & 16.598$\pm$0.071 & PO & i \\
214.6210 & 16.505$\pm$0.062 & PO & i \\
214.7301 & 16.384$\pm$0.064 & PO & i \\
214.7320 & 16.591$\pm$0.073 & PO & i \\
214.7338 & 16.369$\pm$0.061 & PO & i \\
215.6248 & 16.797$\pm$0.068 & PO & i \\
215.6266 & 16.708$\pm$0.064 & PO & i \\
215.6285 & 16.761$\pm$0.069 & PO & i \\
215.6304 & 16.774$\pm$0.072 & PO & i \\
215.6322 & 16.810$\pm$0.077 & PO & i \\
221.6100 & 16.595$\pm$0.046 & PO & i \\
221.6121 & 16.558$\pm$0.046 & PO & i \\
221.6139 & 16.615$\pm$0.048 & PO & i \\
221.6158 & 16.563$\pm$0.045 & PO & i \\
221.6177 & 16.590$\pm$0.046 & PO & i \\
221.6799 & 16.567$\pm$0.046 & PO & i \\
221.6818 & 16.492$\pm$0.045 & PO & i \\
221.6837 & 16.545$\pm$0.045 & PO & i \\
221.6855 & 16.583$\pm$0.046 & PO & i \\
221.6876 & 16.517$\pm$0.044 & PO & i \\
222.6075 & 16.580$\pm$0.045 & PO & i \\
222.6095 & 16.568$\pm$0.044 & PO & i \\
222.6113 & 16.567$\pm$0.044 & PO & i \\
222.6132 & 16.574$\pm$0.044 & PO & i \\
222.6151 & 16.596$\pm$0.045 & PO & i \\
222.6801 & 16.659$\pm$0.048 & PO & i \\
222.6820 & 16.602$\pm$0.046 & PO & i \\
222.6838 & 16.609$\pm$0.047 & PO & i \\
222.6859 & 16.595$\pm$0.047 & PO & i \\
222.6877 & 16.571$\pm$0.046 & PO & i \\
223.6617 & 16.630$\pm$0.050 & PO & i \\
223.6636 & 16.622$\pm$0.054 & PO & i \\
223.6655 & 16.642$\pm$0.059 & PO & i \\
223.6673 & 16.619$\pm$0.052 & PO & i \\
225.5968 & 16.711$\pm$0.049 & PO & i \\
225.5986 & 16.717$\pm$0.047 & PO & i \\
225.6005 & 16.767$\pm$0.049 & PO & i \\
225.6023 & 16.778$\pm$0.049 & PO & i \\
225.6043 & 16.719$\pm$0.048 & PO & i \\
225.6590 & 16.797$\pm$0.049 & PO & i \\
225.6609 & 16.712$\pm$0.049 & PO & i \\
225.6628 & 16.691$\pm$0.048 & PO & i \\
225.6646 & 16.730$\pm$0.048 & PO & i \\
225.6666 & 16.746$\pm$0.049 & PO & i \\
227.6033 & 16.821$\pm$0.050 & PO & i \\
227.6052 & 16.788$\pm$0.048 & PO & i \\
227.6071 & 16.740$\pm$0.047 & PO & i \\
227.6089 & 16.770$\pm$0.048 & PO & i \\
227.6108 & 16.738$\pm$0.048 & PO & i \\
228.6430 & 16.802$\pm$0.049 & PO & i \\
228.6449 & 16.768$\pm$0.048 & PO & i \\
228.6468 & 16.835$\pm$0.049 & PO & i \\
228.6486 & 16.869$\pm$0.050 & PO & i \\
228.6505 & 16.785$\pm$0.048 & PO & i \\
228.6956 & 16.796$\pm$0.049 & PO & i \\
228.6975 & 16.843$\pm$0.050 & PO & i \\
228.6994 & 16.800$\pm$0.049 & PO & i \\
228.7012 & 16.817$\pm$0.049 & PO & i \\
228.7031 & 16.786$\pm$0.049 & PO & i \\
229.5973 & 16.843$\pm$0.051 & PO & i \\
229.5991 & 16.912$\pm$0.052 & PO & i \\
229.6010 & 16.855$\pm$0.051 & PO & i \\
229.6029 & 16.900$\pm$0.052 & PO & i \\
229.6048 & 16.767$\pm$0.048 & PO & i \\
229.6592 & 16.838$\pm$0.051 & PO & i \\
229.6610 & 16.834$\pm$0.051 & PO & i \\
229.6630 & 16.778$\pm$0.049 & PO & i \\
229.6648 & 16.740$\pm$0.048 & PO & i \\
229.6667 & 16.765$\pm$0.048 & PO & i \\
230.6590 & 16.831$\pm$0.049 & PO & i \\
230.6608 & 16.875$\pm$0.051 & PO & i \\
230.6627 & 16.846$\pm$0.050 & PO & i \\
230.6645 & 16.807$\pm$0.048 & PO & i \\
230.6664 & 16.821$\pm$0.049 & PO & i \\
231.5868 & 16.868$\pm$0.051 & PO & i \\
231.5886 & 16.868$\pm$0.053 & PO & i \\
231.5905 & 16.838$\pm$0.052 & PO & i \\
231.5923 & 16.868$\pm$0.053 & PO & i \\
231.5942 & 16.847$\pm$0.051 & PO & i \\
232.6419 & 16.792$\pm$0.049 & PO & i \\
232.6444 & 16.806$\pm$0.050 & PO & i \\
232.6470 & 16.786$\pm$0.050 & PO & i \\
232.6494 & 16.763$\pm$0.049 & PO & i \\
233.5796 & 16.682$\pm$0.046 & PO & i \\
233.5821 & 16.585$\pm$0.044 & PO & i \\
233.5845 & 16.587$\pm$0.044 & PO & i \\
233.5869 & 16.699$\pm$0.047 & PO & i \\
235.6541 & 16.805$\pm$0.051 & PO & i \\
235.6567 & 16.803$\pm$0.050 & PO & i \\
235.6591 & 16.757$\pm$0.049 & PO & i \\
235.6616 & 16.771$\pm$0.049 & PO & i \\
236.6677 & 16.790$\pm$0.048 & PO & i \\
236.6701 & 16.751$\pm$0.047 & PO & i \\
236.6725 & 16.721$\pm$0.047 & PO & i \\
236.6750 & 16.743$\pm$0.049 & PO & i \\
237.6969 & 16.772$\pm$0.049 & PO & i \\
237.6993 & 16.794$\pm$0.050 & PO & i \\
237.7018 & 16.869$\pm$0.053 & PO & i \\
237.7042 & 16.843$\pm$0.052 & PO & i \\
238.6556 & 16.794$\pm$0.049 & PO & i \\
238.6581 & 16.605$\pm$0.046 & PO & i \\
238.6605 & 16.829$\pm$0.050 & PO & i \\
238.6630 & 16.831$\pm$0.051 & PO & i \\
240.5984 & 16.836$\pm$0.050 & PO & i \\
240.6009 & 16.839$\pm$0.050 & PO & i \\
240.6033 & 16.844$\pm$0.049 & PO & i \\
240.6058 & 16.808$\pm$0.049 & PO & i \\
240.6082 & 16.839$\pm$0.049 & PO & i \\
240.6107 & 16.882$\pm$0.050 & PO & i \\
240.6702 & 16.779$\pm$0.050 & PO & i \\
240.6726 & 16.871$\pm$0.052 & PO & i \\
240.6750 & 16.939$\pm$0.053 & PO & i \\
240.6775 & 16.866$\pm$0.052 & PO & i \\
240.6799 & 16.905$\pm$0.054 & PO & i \\
240.6823 & 16.878$\pm$0.052 & PO & i \\
241.6048 & 16.834$\pm$0.066 & PO & i \\
241.6073 & 16.775$\pm$0.077 & PO & i \\
241.6097 & 16.915$\pm$0.096 & PO & i \\
241.6121 & 16.395$\pm$0.084 & PO & i \\
241.6148 & 16.351$\pm$0.097 & PO & i \\
241.6172 & 16.455$\pm$0.143 & PO & i \\
247.6344 & 16.784$\pm$0.051 & PO & i \\
247.6368 & 16.729$\pm$0.049 & PO & i \\
247.6393 & 16.753$\pm$0.050 & PO & i \\
247.6417 & 16.862$\pm$0.054 & PO & i \\
247.6441 & 16.783$\pm$0.050 & PO & i \\
247.6466 & 16.845$\pm$0.051 & PO & i \\
248.6205 & 16.609$\pm$0.047 & PO & i \\
248.6229 & 16.879$\pm$0.053 & PO & i \\
248.6254 & 16.754$\pm$0.049 & PO & i \\
248.6278 & 16.749$\pm$0.050 & PO & i \\
248.6302 & 16.786$\pm$0.051 & PO & i \\
248.6326 & 16.797$\pm$0.052 & PO & i \\
249.5989 & 16.819$\pm$0.051 & PO & i \\
249.6014 & 16.859$\pm$0.052 & PO & i \\
249.6038 & 16.714$\pm$0.050 & PO & i \\
249.6062 & 16.777$\pm$0.049 & PO & i \\
249.6087 & 16.747$\pm$0.050 & PO & i \\
249.6111 & 16.781$\pm$0.050 & PO & i \\
250.6033 & 16.887$\pm$0.055 & PO & i \\
250.6057 & 16.907$\pm$0.054 & PO & i \\
250.6082 & 16.838$\pm$0.055 & PO & i \\
250.6106 & 16.903$\pm$0.054 & PO & i \\
250.6130 & 16.915$\pm$0.060 & PO & i \\
250.6154 & 16.874$\pm$0.056 & PO & i \\
251.6357 & 17.056$\pm$0.116 & PO & i \\
251.6381 & 17.002$\pm$0.093 & PO & i \\
251.6405 & 17.122$\pm$0.085 & PO & i \\
251.6430 & 16.889$\pm$0.068 & PO & i \\
251.6456 & 16.906$\pm$0.066 & PO & i \\
251.6480 & 16.727$\pm$0.062 & PO & i \\
252.6027 & 16.940$\pm$0.053 & PO & i \\
252.6051 & 16.914$\pm$0.053 & PO & i \\
252.6075 & 17.016$\pm$0.055 & PO & i \\
252.6099 & 16.996$\pm$0.055 & PO & i \\
252.6124 & 16.956$\pm$0.054 & PO & i \\
252.6148 & 16.934$\pm$0.054 & PO & i \\
253.5904 & 17.041$\pm$0.059 & PO & i \\
253.5928 & 17.025$\pm$0.057 & PO & i \\
253.5952 & 16.954$\pm$0.054 & PO & i \\
253.5977 & 17.041$\pm$0.057 & PO & i \\
253.6003 & 16.890$\pm$0.054 & PO & i \\
253.6027 & 16.905$\pm$0.054 & PO & i \\
254.5837 & 17.059$\pm$0.057 & PO & i \\
254.5862 & 17.016$\pm$0.057 & PO & i \\
254.5888 & 16.954$\pm$0.054 & PO & i \\
254.5912 & 16.973$\pm$0.054 & PO & i \\
254.5936 & 16.974$\pm$0.055 & PO & i \\
254.5960 & 16.935$\pm$0.053 & PO & i \\
255.5837 & 17.169$\pm$0.127 & PO & i \\
255.5862 & 17.315$\pm$0.156 & PO & i \\
255.5886 & 17.275$\pm$0.146 & PO & i \\
255.5912 & 16.765$\pm$0.078 & PO & i \\
255.5936 & 16.980$\pm$0.083 & PO & i \\
255.5960 & 16.963$\pm$0.083 & PO & i \\
256.5838 & 17.034$\pm$0.057 & PO & i \\
256.5862 & 17.057$\pm$0.057 & PO & i \\
256.5886 & 17.059$\pm$0.061 & PO & i \\
256.5911 & 17.070$\pm$0.060 & PO & i \\
256.5935 & 17.128$\pm$0.060 & PO & i \\
256.5959 & 17.061$\pm$0.060 & PO & i \\
257.5937 & 16.995$\pm$0.055 & PO & i \\
257.5962 & 17.044$\pm$0.056 & PO & i \\
257.5988 & 16.989$\pm$0.054 & PO & i \\
257.6012 & 16.988$\pm$0.054 & PO & i \\
257.6036 & 16.948$\pm$0.054 & PO & i \\
257.6061 & 16.952$\pm$0.053 & PO & i \\
259.6088 & 16.815$\pm$0.050 & PO & i \\
259.6114 & 16.764$\pm$0.049 & PO & i \\
259.6139 & 16.820$\pm$0.051 & PO & i \\
259.6163 & 16.818$\pm$0.051 & PO & i \\
259.6187 & 16.821$\pm$0.051 & PO & i \\
259.6211 & 16.880$\pm$0.058 & PO & i \\
263.6080 & 16.540$\pm$0.043 & PO & i \\
263.6104 & 16.558$\pm$0.044 & PO & i \\
263.6128 & 16.655$\pm$0.046 & PO & i \\
263.6153 & 16.702$\pm$0.047 & PO & i \\
263.6177 & 16.656$\pm$0.046 & PO & i \\
263.6201 & 16.684$\pm$0.047 & PO & i \\
264.5962 & 16.851$\pm$0.053 & PO & i \\
264.5988 & 16.675$\pm$0.049 & PO & i \\
264.6012 & 16.844$\pm$0.058 & PO & i \\
264.6036 & 16.781$\pm$0.052 & PO & i \\
264.6061 & 16.779$\pm$0.052 & PO & i \\
264.6086 & 16.864$\pm$0.054 & PO & i \\
265.5963 & 16.851$\pm$0.054 & PO & i \\
265.5987 & 16.929$\pm$0.056 & PO & i \\
265.6012 & 16.927$\pm$0.055 & PO & i \\
265.6036 & 16.905$\pm$0.059 & PO & i \\
265.6060 & 16.947$\pm$0.055 & PO & i \\
265.6084 & 16.929$\pm$0.054 & PO & i \\
266.5964 & 16.950$\pm$0.053 & PO & i \\
266.5989 & 16.960$\pm$0.053 & PO & i \\
266.6013 & 17.008$\pm$0.056 & PO & i \\
266.6037 & 17.025$\pm$0.056 & PO & i \\
266.6061 & 17.081$\pm$0.058 & PO & i \\
266.6086 & 17.123$\pm$0.065 & PO & i \\
267.5862 & 17.088$\pm$0.061 & PO & i \\
267.5887 & 17.131$\pm$0.059 & PO & i \\
267.5911 & 17.129$\pm$0.059 & PO & i \\
267.5935 & 17.175$\pm$0.063 & PO & i \\
267.5960 & 17.174$\pm$0.062 & PO & i \\
267.5984 & 17.198$\pm$0.065 & PO & i \\
270.6031 & 17.390$\pm$0.070 & PO & i \\
270.6055 & 17.455$\pm$0.074 & PO & i \\
270.6080 & 17.503$\pm$0.077 & PO & i \\
271.5887 & 17.612$\pm$0.082 & PO & i \\
271.5912 & 17.700$\pm$0.087 & PO & i \\
271.5936 & 17.692$\pm$0.088 & PO & i \\
271.5960 & 17.816$\pm$0.103 & PO & i \\
271.5984 & 17.686$\pm$0.087 & PO & i \\
272.5884 & 17.676$\pm$0.101 & PO & i \\
272.5908 & 17.732$\pm$0.109 & PO & i \\
272.5932 & 18.177$\pm$0.177 & PO & i \\
272.5957 & 18.087$\pm$0.148 & PO & i \\
272.5981 & 18.059$\pm$0.148 & PO & i \\
273.5883 & 17.730$\pm$0.088 & PO & i \\
273.5908 & 17.618$\pm$0.086 & PO & i \\
273.5932 & 17.724$\pm$0.089 & PO & i \\
273.5958 & 17.560$\pm$0.080 & PO & i \\
273.5982 & 17.477$\pm$0.081 & PO & i \\
193.6429 & 15.863$\pm$0.062 & PO & z \\
193.6448 & 15.809$\pm$0.060 & PO & z \\
193.6467 & 15.883$\pm$0.062 & PO & z \\
195.6430 & 15.765$\pm$0.062 & PO & z \\
195.6448 & 15.749$\pm$0.062 & PO & z \\
195.6467 & 15.745$\pm$0.063 & PO & z \\
196.6448 & 15.772$\pm$0.060 & PO & z \\
196.6467 & 15.770$\pm$0.061 & PO & z \\
196.6486 & 15.816$\pm$0.061 & PO & z \\
197.6340 & 15.764$\pm$0.061 & PO & z \\
197.6358 & 15.789$\pm$0.061 & PO & z \\
197.6377 & 15.762$\pm$0.061 & PO & z \\
198.6291 & 15.746$\pm$0.061 & PO & z \\
198.6310 & 15.752$\pm$0.061 & PO & z \\
198.6329 & 15.730$\pm$0.061 & PO & z \\
201.6221 & 15.804$\pm$0.064 & PO & z \\
201.6240 & 15.863$\pm$0.064 & PO & z \\
201.6259 & 15.844$\pm$0.063 & PO & z \\
204.6219 & 15.921$\pm$0.063 & PO & z \\
204.6237 & 15.930$\pm$0.062 & PO & z \\
204.6256 & 15.949$\pm$0.062 & PO & z \\
204.7400 & 15.961$\pm$0.064 & PO & z \\
204.7419 & 15.947$\pm$0.063 & PO & z \\
204.7437 & 15.925$\pm$0.062 & PO & z \\
205.6221 & 15.984$\pm$0.064 & PO & z \\
205.6240 & 16.013$\pm$0.064 & PO & z \\
205.6258 & 15.980$\pm$0.063 & PO & z \\
205.7400 & 15.920$\pm$0.062 & PO & z \\
205.7419 & 15.922$\pm$0.063 & PO & z \\
205.7437 & 15.926$\pm$0.064 & PO & z \\
206.7013 & 15.974$\pm$0.067 & PO & z \\
206.7050 & 15.964$\pm$0.066 & PO & z \\
206.7894 & 15.836$\pm$0.067 & PO & z \\
206.7914 & 16.009$\pm$0.071 & PO & z \\
206.7933 & 15.951$\pm$0.071 & PO & z \\
207.6080 & 15.931$\pm$0.064 & PO & z \\
207.6099 & 15.944$\pm$0.065 & PO & z \\
207.6118 & 15.932$\pm$0.064 & PO & z \\
207.6963 & 15.563$\pm$0.095 & PO & z \\
210.6229 & 15.874$\pm$0.071 & PO & z \\
210.6248 & 15.820$\pm$0.068 & PO & z \\
210.6266 & 15.872$\pm$0.070 & PO & z \\
213.6228 & 15.942$\pm$0.064 & PO & z \\
213.6248 & 15.909$\pm$0.064 & PO & z \\
213.6266 & 15.904$\pm$0.064 & PO & z \\
214.6228 & 16.049$\pm$0.081 & PO & z \\
214.7357 & 16.060$\pm$0.080 & PO & z \\
214.7378 & 16.082$\pm$0.086 & PO & z \\
214.7396 & 16.039$\pm$0.097 & PO & z \\
215.6341 & 16.227$\pm$0.086 & PO & z \\
215.6359 & 16.041$\pm$0.072 & PO & z \\
215.6378 & 16.185$\pm$0.077 & PO & z \\
215.6397 & 16.235$\pm$0.077 & PO & z \\
215.6415 & 16.372$\pm$0.083 & PO & z \\
215.6955 & 16.217$\pm$0.081 & PO & z \\
215.6973 & 16.054$\pm$0.076 & PO & z \\
215.6992 & 16.069$\pm$0.080 & PO & z \\
215.7010 & 16.054$\pm$0.077 & PO & z \\
215.7029 & 16.130$\pm$0.080 & PO & z \\
221.6196 & 15.989$\pm$0.063 & PO & z \\
221.6214 & 15.936$\pm$0.065 & PO & z \\
221.6233 & 15.961$\pm$0.065 & PO & z \\
221.6251 & 15.923$\pm$0.064 & PO & z \\
221.6270 & 15.948$\pm$0.065 & PO & z \\
221.6894 & 15.966$\pm$0.064 & PO & z \\
221.6913 & 15.965$\pm$0.065 & PO & z \\
221.6931 & 15.938$\pm$0.064 & PO & z \\
221.6950 & 15.984$\pm$0.064 & PO & z \\
221.6969 & 15.912$\pm$0.062 & PO & z \\
222.6170 & 15.999$\pm$0.064 & PO & z \\
222.6188 & 15.951$\pm$0.063 & PO & z \\
222.6206 & 15.975$\pm$0.064 & PO & z \\
222.6225 & 15.955$\pm$0.063 & PO & z \\
222.6244 & 15.974$\pm$0.063 & PO & z \\
222.6896 & 15.976$\pm$0.066 & PO & z \\
222.6915 & 15.995$\pm$0.066 & PO & z \\
222.6933 & 15.999$\pm$0.065 & PO & z \\
222.6952 & 15.955$\pm$0.067 & PO & z \\
222.6970 & 15.989$\pm$0.067 & PO & z \\
223.6693 & 15.921$\pm$0.069 & PO & z \\
223.6711 & 16.045$\pm$0.074 & PO & z \\
223.6729 & 15.952$\pm$0.067 & PO & z \\
223.6749 & 15.970$\pm$0.067 & PO & z \\
225.6061 & 16.061$\pm$0.076 & PO & z \\
225.6080 & 16.027$\pm$0.067 & PO & z \\
225.6099 & 15.993$\pm$0.069 & PO & z \\
225.6117 & 16.047$\pm$0.069 & PO & z \\
225.6136 & 16.050$\pm$0.070 & PO & z \\
225.6685 & 16.245$\pm$0.069 & PO & z \\
225.6704 & 16.145$\pm$0.067 & PO & z \\
225.6722 & 16.164$\pm$0.069 & PO & z \\
225.6740 & 16.158$\pm$0.069 & PO & z \\
225.6759 & 16.126$\pm$0.068 & PO & z \\
227.6127 & 16.121$\pm$0.064 & PO & z \\
227.6145 & 16.019$\pm$0.064 & PO & z \\
227.6164 & 16.025$\pm$0.065 & PO & z \\
227.6183 & 16.064$\pm$0.065 & PO & z \\
227.6202 & 16.095$\pm$0.067 & PO & z \\
228.6524 & 16.131$\pm$0.064 & PO & z \\
228.6543 & 16.122$\pm$0.064 & PO & z \\
228.6562 & 16.140$\pm$0.064 & PO & z \\
228.6580 & 16.235$\pm$0.064 & PO & z \\
228.6599 & 16.206$\pm$0.064 & PO & z \\
228.7050 & 16.180$\pm$0.064 & PO & z \\
228.7069 & 16.139$\pm$0.065 & PO & z \\
228.7088 & 16.136$\pm$0.065 & PO & z \\
228.7106 & 16.125$\pm$0.065 & PO & z \\
228.7125 & 16.140$\pm$0.065 & PO & z \\
229.6067 & 16.135$\pm$0.065 & PO & z \\
229.6086 & 16.137$\pm$0.066 & PO & z \\
229.6104 & 16.110$\pm$0.064 & PO & z \\
229.6122 & 16.102$\pm$0.065 & PO & z \\
229.6141 & 16.089$\pm$0.064 & PO & z \\
229.6686 & 16.099$\pm$0.065 & PO & z \\
229.6705 & 16.131$\pm$0.065 & PO & z \\
229.6724 & 16.118$\pm$0.065 & PO & z \\
229.6742 & 16.042$\pm$0.065 & PO & z \\
229.6761 & 16.065$\pm$0.065 & PO & z \\
230.6682 & 16.200$\pm$0.065 & PO & z \\
230.6701 & 16.128$\pm$0.066 & PO & z \\
230.6720 & 16.138$\pm$0.065 & PO & z \\
230.6738 & 16.174$\pm$0.065 & PO & z \\
230.6757 & 16.144$\pm$0.065 & PO & z \\
231.5961 & 16.249$\pm$0.067 & PO & z \\
231.5980 & 16.235$\pm$0.070 & PO & z \\
231.5998 & 16.135$\pm$0.071 & PO & z \\
231.6016 & 16.286$\pm$0.080 & PO & z \\
231.6035 & 16.203$\pm$0.072 & PO & z \\
232.6519 & 16.146$\pm$0.067 & PO & z \\
232.6543 & 16.099$\pm$0.065 & PO & z \\
232.6568 & 16.067$\pm$0.065 & PO & z \\
232.6592 & 16.057$\pm$0.064 & PO & z \\
233.5894 & 15.995$\pm$0.066 & PO & z \\
233.5919 & 15.994$\pm$0.067 & PO & z \\
233.5943 & 16.010$\pm$0.064 & PO & z \\
233.5968 & 15.940$\pm$0.065 & PO & z \\
235.6640 & 15.992$\pm$0.064 & PO & z \\
235.6665 & 16.151$\pm$0.068 & PO & z \\
235.6689 & 16.042$\pm$0.064 & PO & z \\
235.6713 & 16.053$\pm$0.066 & PO & z \\
236.6774 & 16.047$\pm$0.064 & PO & z \\
236.6799 & 16.019$\pm$0.065 & PO & z \\
236.6823 & 16.012$\pm$0.064 & PO & z \\
236.6847 & 16.105$\pm$0.065 & PO & z \\
237.7068 & 16.116$\pm$0.074 & PO & z \\
237.7093 & 15.935$\pm$0.069 & PO & z \\
237.7117 & 16.111$\pm$0.071 & PO & z \\
237.7142 & 15.838$\pm$0.067 & PO & z \\
238.6654 & 16.063$\pm$0.067 & PO & z \\
238.6679 & 16.024$\pm$0.069 & PO & z \\
238.6703 & 16.147$\pm$0.067 & PO & z \\
238.6728 & 16.119$\pm$0.068 & PO & z \\
240.6131 & 16.147$\pm$0.064 & PO & z \\
240.6156 & 16.162$\pm$0.064 & PO & z \\
240.6180 & 16.200$\pm$0.065 & PO & z \\
240.6204 & 16.269$\pm$0.065 & PO & z \\
240.6229 & 16.205$\pm$0.064 & PO & z \\
240.6253 & 16.180$\pm$0.064 & PO & z \\
240.6848 & 16.192$\pm$0.068 & PO & z \\
240.6872 & 16.140$\pm$0.066 & PO & z \\
240.6898 & 16.086$\pm$0.067 & PO & z \\
240.6923 & 16.040$\pm$0.065 & PO & z \\
240.6947 & 16.057$\pm$0.067 & PO & z \\
240.6971 & 16.128$\pm$0.066 & PO & z \\
247.6491 & 16.066$\pm$0.065 & PO & z \\
247.6515 & 16.060$\pm$0.067 & PO & z \\
247.6540 & 16.126$\pm$0.067 & PO & z \\
247.6564 & 16.023$\pm$0.065 & PO & z \\
247.6588 & 16.180$\pm$0.065 & PO & z \\
247.6615 & 16.066$\pm$0.069 & PO & z \\
248.6351 & 16.078$\pm$0.065 & PO & z \\
248.6375 & 16.083$\pm$0.066 & PO & z \\
248.6400 & 16.097$\pm$0.066 & PO & z \\
248.6424 & 16.103$\pm$0.066 & PO & z \\
248.6451 & 16.083$\pm$0.073 & PO & z \\
248.6475 & 15.952$\pm$0.071 & PO & z \\
249.6136 & 16.112$\pm$0.066 & PO & z \\
249.6160 & 16.110$\pm$0.067 & PO & z \\
249.6184 & 16.156$\pm$0.067 & PO & z \\
249.6209 & 16.190$\pm$0.068 & PO & z \\
249.6234 & 16.031$\pm$0.066 & PO & z \\
249.6258 & 16.157$\pm$0.066 & PO & z \\
250.6181 & 16.293$\pm$0.073 & PO & z \\
250.6205 & 16.261$\pm$0.075 & PO & z \\
251.6505 & 16.124$\pm$0.080 & PO & z \\
251.6530 & 16.142$\pm$0.085 & PO & z \\
251.6554 & 16.131$\pm$0.086 & PO & z \\
251.6578 & 16.188$\pm$0.090 & PO & z \\
251.6602 & 16.005$\pm$0.077 & PO & z \\
251.6627 & 15.957$\pm$0.078 & PO & z \\
252.6173 & 16.229$\pm$0.065 & PO & z \\
252.6197 & 16.233$\pm$0.065 & PO & z \\
252.6221 & 16.191$\pm$0.065 & PO & z \\
252.6246 & 16.244$\pm$0.066 & PO & z \\
252.6272 & 16.263$\pm$0.069 & PO & z \\
252.6296 & 16.193$\pm$0.068 & PO & z \\
253.6052 & 16.221$\pm$0.072 & PO & z \\
253.6076 & 16.143$\pm$0.071 & PO & z \\
253.6100 & 16.220$\pm$0.070 & PO & z \\
253.6125 & 16.193$\pm$0.067 & PO & z \\
253.6149 & 16.237$\pm$0.071 & PO & z \\
253.6173 & 16.120$\pm$0.071 & PO & z \\
254.5985 & 16.206$\pm$0.069 & PO & z \\
254.6009 & 16.264$\pm$0.070 & PO & z \\
254.6034 & 16.202$\pm$0.067 & PO & z \\
254.6058 & 16.184$\pm$0.069 & PO & z \\
254.6082 & 16.217$\pm$0.067 & PO & z \\
254.6107 & 16.280$\pm$0.067 & PO & z \\
255.5986 & 16.126$\pm$0.122 & PO & z \\
255.6010 & 16.099$\pm$0.096 & PO & z \\
255.6034 & 16.162$\pm$0.105 & PO & z \\
255.6058 & 16.227$\pm$0.101 & PO & z \\
255.6083 & 16.151$\pm$0.083 & PO & z \\
255.6107 & 16.240$\pm$0.080 & PO & z \\
256.5986 & 16.541$\pm$0.094 & PO & z \\
256.6010 & 16.613$\pm$0.110 & PO & z \\
256.6035 & 16.487$\pm$0.092 & PO & z \\
256.6060 & 16.402$\pm$0.087 & PO & z \\
256.6084 & 16.354$\pm$0.086 & PO & z \\
256.6108 & 16.302$\pm$0.087 & PO & z \\
257.6086 & 16.202$\pm$0.068 & PO & z \\
257.6110 & 16.199$\pm$0.069 & PO & z \\
257.6134 & 16.266$\pm$0.069 & PO & z \\
257.6159 & 16.193$\pm$0.067 & PO & z \\
257.6183 & 16.285$\pm$0.068 & PO & z \\
257.6207 & 16.259$\pm$0.068 & PO & z \\
259.6236 & 16.094$\pm$0.068 & PO & z \\
259.6260 & 15.916$\pm$0.070 & PO & z \\
259.6285 & 16.032$\pm$0.072 & PO & z \\
259.6309 & 16.019$\pm$0.070 & PO & z \\
259.6333 & 15.744$\pm$0.064 & PO & z \\
259.6357 & 16.054$\pm$0.072 & PO & z \\
263.6226 & 16.037$\pm$0.064 & PO & z \\
263.6250 & 16.048$\pm$0.064 & PO & z \\
263.6274 & 16.093$\pm$0.066 & PO & z \\
263.6299 & 16.065$\pm$0.065 & PO & z \\
263.6325 & 16.085$\pm$0.070 & PO & z \\
263.6349 & 15.974$\pm$0.066 & PO & z \\
264.6110 & 16.231$\pm$0.076 & PO & z \\
264.6135 & 16.163$\pm$0.073 & PO & z \\
264.6159 & 16.227$\pm$0.074 & PO & z \\
264.6185 & 16.244$\pm$0.083 & PO & z \\
264.6210 & 16.043$\pm$0.076 & PO & z \\
264.6234 & 16.068$\pm$0.074 & PO & z \\
265.6109 & 16.193$\pm$0.067 & PO & z \\
265.6134 & 16.253$\pm$0.069 & PO & z \\
265.6160 & 16.206$\pm$0.087 & PO & z \\
265.6184 & 16.032$\pm$0.084 & PO & z \\
265.6208 & 16.156$\pm$0.084 & PO & z \\
265.6232 & 16.084$\pm$0.086 & PO & z \\
266.6110 & 16.320$\pm$0.068 & PO & z \\
266.6134 & 16.262$\pm$0.069 & PO & z \\
266.6161 & 16.130$\pm$0.083 & PO & z \\
266.6185 & 16.131$\pm$0.080 & PO & z \\
266.6209 & 16.178$\pm$0.080 & PO & z \\
266.6234 & 16.186$\pm$0.074 & PO & z \\
\enddata
\label{tab:phot_mephisto}
\end{deluxetable}


==> tables/sn2022jli_phot_data.tex <==
\begin{table}
\begin{tabular}{cccc}
epoch & mag & source & filter \\
8.9154 & 15.366$\pm$0.053 & ASAS-SN & g \\
12.6611 & 15.386$\pm$0.053 & ASAS-SN & g \\
14.6775 & 15.602$\pm$0.171 & ASAS-SN & g \\
16.6692 & 15.737$\pm$0.120 & ASAS-SN & g \\
22.8739 & 15.477$\pm$0.060 & ASAS-SN & g \\
25.6585 & 14.786$\pm$0.007 & ATLAS & o \\
25.6657 & 14.775$\pm$0.007 & ATLAS & o \\
25.6826 & 14.796$\pm$0.012 & ATLAS & o \\
27.6503 & 16.140$\pm$0.113 & ASAS-SN & g \\
31.6665 & 16.245$\pm$0.078 & ASAS-SN & g \\
33.0868 & 15.751$\pm$0.013 & ATLAS & c \\
33.0953 & 15.696$\pm$0.011 & ATLAS & c \\
33.1092 & 15.707$\pm$0.013 & ATLAS & c \\
33.1134 & 15.718$\pm$0.017 & ATLAS & c \\
33.6136 & 16.092$\pm$0.063 & ASAS-SN & g \\
34.6683 & 16.324$\pm$0.125 & ASAS-SN & g \\
35.6096 & 16.005$\pm$0.082 & ASAS-SN & g \\
37.0850 & 15.568$\pm$0.011 & ATLAS & c \\
37.1016 & 15.540$\pm$0.011 & ATLAS & c \\
37.1042 & 15.920$\pm$0.072 & ASAS-SN & g \\
37.1044 & 15.529$\pm$0.010 & ATLAS & c \\
37.1150 & 15.579$\pm$0.018 & ATLAS & c \\
37.6023 & 15.944$\pm$0.066 & ASAS-SN & g \\
37.6553 & 14.867$\pm$0.007 & ATLAS & o \\
37.6739 & 14.861$\pm$0.008 & ATLAS & o \\
37.6854 & 14.882$\pm$0.015 & ATLAS & o \\
38.8515 & 15.774$\pm$0.051 & ASAS-SN & g \\
41.5805 & 15.720$\pm$0.053 & ASAS-SN & g \\
42.9147 & 15.482$\pm$0.039 & ASAS-SN & g \\
45.0839 & 14.578$\pm$0.009 & ATLAS & o \\
45.0959 & 14.517$\pm$0.009 & ATLAS & o \\
45.1065 & 14.563$\pm$0.008 & ATLAS & o \\
45.1101 & 14.538$\pm$0.008 & ATLAS & o \\
47.0924 & 14.489$\pm$0.009 & ATLAS & o \\
47.0965 & 14.520$\pm$0.009 & ATLAS & o \\
47.1034 & 14.494$\pm$0.008 & ATLAS & o \\
47.1159 & 14.496$\pm$0.019 & ATLAS & o \\
47.8300 & 15.275$\pm$0.047 & ASAS-SN & g \\
49.8793 & 15.202$\pm$0.049 & ASAS-SN & g \\
54.0836 & 14.482$\pm$0.005 & ATLAS & o \\
54.0868 & 14.464$\pm$0.006 & ATLAS & o \\
54.0966 & 14.463$\pm$0.005 & ATLAS & o \\
54.1023 & 14.454$\pm$0.005 & ATLAS & o \\
55.0878 & 14.434$\pm$0.006 & ATLAS & o \\
55.0925 & 14.483$\pm$0.006 & ATLAS & o \\
55.1004 & 14.475$\pm$0.006 & ATLAS & o \\
55.1018 & 14.464$\pm$0.006 & ATLAS & o \\
55.1105 & 14.455$\pm$0.006 & ATLAS & o \\
55.1119 & 14.427$\pm$0.006 & ATLAS & o \\
55.1183 & 14.481$\pm$0.009 & ATLAS & o \\
55.1197 & 14.467$\pm$0.011 & ATLAS & o \\
57.9530 & 15.244$\pm$0.024 & ZTF & g \\
57.9530 & 15.244$\pm$0.024 & ZTF & g \\
57.9540 & 15.220$\pm$0.029 & ZTF & g \\
57.9540 & 15.220$\pm$0.029 & ZTF & g \\
57.9540 & 15.220$\pm$0.029 & ZTF & g \\
58.9335 & 15.217$\pm$0.035 & ASAS-SN & g \\
58.9425 & 14.681$\pm$0.037 & ZTF & r \\
58.9425 & 14.681$\pm$0.037 & ZTF & r \\
58.9425 & 14.681$\pm$0.037 & ZTF & r \\
60.9463 & 14.596$\pm$0.029 & ZTF & r \\
60.9463 & 14.596$\pm$0.029 & ZTF & r \\
60.9463 & 14.596$\pm$0.029 & ZTF & r \\
61.5420 & 15.384$\pm$0.038 & ASAS-SN & g \\
63.9338 & 14.658$\pm$0.031 & ZTF & r \\
63.9338 & 14.658$\pm$0.031 & ZTF & r \\
63.9338 & 14.658$\pm$0.031 & ZTF & r \\
63.9554 & 15.147$\pm$0.055 & ASAS-SN & g \\
63.9591 & 15.260$\pm$0.026 & ZTF & g \\
63.9591 & 15.260$\pm$0.026 & ZTF & g \\
63.9591 & 15.260$\pm$0.026 & ZTF & g \\
65.9251 & 15.320$\pm$0.023 & ZTF & g \\
65.9251 & 15.320$\pm$0.023 & ZTF & g \\
65.9251 & 15.320$\pm$0.023 & ZTF & g \\
65.9534 & 14.733$\pm$0.026 & ZTF & r \\
65.9534 & 14.733$\pm$0.026 & ZTF & r \\
65.9534 & 14.733$\pm$0.026 & ZTF & r \\
66.9374 & 15.304$\pm$0.035 & ZTF & g \\
66.9374 & 15.303$\pm$0.035 & ZTF & g \\
66.9374 & 15.303$\pm$0.035 & ZTF & g \\
67.0909 & 14.630$\pm$0.006 & ATLAS & o \\
67.1128 & 14.646$\pm$0.008 & ATLAS & o \\
67.1160 & 14.631$\pm$0.010 & ATLAS & o \\
67.1203 & 14.640$\pm$0.011 & ATLAS & o \\
67.7761 & 15.290$\pm$0.041 & ASAS-SN & g \\
67.9500 & 14.790$\pm$0.038 & P60 & r \\
67.9520 & 14.660$\pm$0.038 & P60 & i \\
69.0885 & 15.091$\pm$0.007 & ATLAS & c \\
69.1067 & 15.087$\pm$0.008 & ATLAS & c \\
69.1158 & 15.089$\pm$0.010 & ATLAS & c \\
69.6153 & 14.702$\pm$0.006 & ATLAS & o \\
69.6255 & 14.684$\pm$0.007 & ATLAS & o \\
69.6403 & 14.707$\pm$0.006 & ATLAS & o \\
69.6452 & 14.698$\pm$0.007 & ATLAS & o \\
69.9215 & 15.315$\pm$0.027 & ZTF & g \\
69.9215 & 15.315$\pm$0.027 & ZTF & g \\
69.9215 & 15.315$\pm$0.027 & ZTF & g \\
70.9085 & 15.267$\pm$0.027 & ZTF & g \\
70.9085 & 15.267$\pm$0.027 & ZTF & g \\
70.9085 & 15.267$\pm$0.027 & ZTF & g \\
71.0865 & 14.703$\pm$0.006 & ATLAS & o \\
71.1037 & 15.251$\pm$0.030 & ASAS-SN & g \\
71.1066 & 14.714$\pm$0.006 & ATLAS & o \\
71.1108 & 14.711$\pm$0.007 & ATLAS & o \\
71.1202 & 14.734$\pm$0.009 & ATLAS & o \\
71.9589 & 15.304$\pm$0.033 & ZTF & g \\
71.9589 & 15.304$\pm$0.033 & ZTF & g \\
71.9589 & 15.304$\pm$0.033 & ZTF & g \\
72.9207 & 14.797$\pm$0.027 & ZTF & r \\
72.9207 & 14.797$\pm$0.027 & ZTF & r \\
72.9207 & 14.797$\pm$0.027 & ZTF & r \\
72.9429 & 15.298$\pm$0.040 & ASAS-SN & g \\
73.0627 & 14.678$\pm$0.007 & ATLAS & o \\
73.0659 & 14.700$\pm$0.007 & ATLAS & o \\
73.0722 & 14.666$\pm$0.006 & ATLAS & o \\
73.0854 & 14.688$\pm$0.006 & ATLAS & o \\
73.5924 & 14.685$\pm$0.008 & ATLAS & o \\
73.5956 & 14.675$\pm$0.007 & ATLAS & o \\
73.6005 & 14.689$\pm$0.010 & ATLAS & o \\
73.6073 & 14.678$\pm$0.008 & ATLAS & o \\
73.8081 & 15.232$\pm$0.070 & ASAS-SN & g \\
74.9258 & 14.854$\pm$0.025 & ZTF & r \\
74.9258 & 14.854$\pm$0.025 & ZTF & r \\
74.9258 & 14.854$\pm$0.025 & ZTF & r \\
74.9267 & 14.870$\pm$0.024 & ZTF & r \\
74.9267 & 14.870$\pm$0.024 & ZTF & r \\
74.9267 & 14.870$\pm$0.024 & ZTF & r \\
74.9580 & 14.880$\pm$0.029 & ZTF & r \\
74.9580 & 14.880$\pm$0.029 & ZTF & r \\
74.9580 & 14.880$\pm$0.029 & ZTF & r \\
75.0325 & 14.748$\pm$0.010 & ATLAS & o \\
75.0387 & 14.764$\pm$0.009 & ATLAS & o \\
75.0424 & 14.749$\pm$0.009 & ATLAS & o \\
75.0529 & 14.750$\pm$0.009 & ATLAS & o \\
76.4888 & 14.671$\pm$0.053 & ATLAS & o \\
76.4920 & 14.759$\pm$0.015 & ATLAS & o \\
76.4979 & 14.803$\pm$0.013 & ATLAS & o \\
76.5165 & 14.762$\pm$0.009 & ATLAS & o \\
76.8817 & 15.208$\pm$0.067 & ASAS-SN & g \\
76.9149 & 14.909$\pm$0.025 & ZTF & r \\
76.9149 & 14.909$\pm$0.025 & ZTF & r \\
76.9465 & 14.928$\pm$0.041 & ZTF & r \\
76.9465 & 14.928$\pm$0.041 & ZTF & r \\
77.5088 & 14.747$\pm$0.013 & ATLAS & o \\
77.5115 & 14.797$\pm$0.012 & ATLAS & o \\
77.5260 & 14.781$\pm$0.012 & ATLAS & o \\
77.5319 & 14.804$\pm$0.011 & ATLAS & o \\
79.9797 & 15.077$\pm$0.041 & P60 & r \\
79.9817 & 14.964$\pm$0.040 & P60 & i \\
80.9217 & 15.490$\pm$0.046 & ZTF & g \\
80.9217 & 15.490$\pm$0.046 & ZTF & g \\
80.9231 & 15.523$\pm$0.023 & ZTF & g \\
80.9231 & 15.523$\pm$0.023 & ZTF & g \\
80.9572 & 15.488$\pm$0.044 & ZTF & g \\
80.9572 & 15.488$\pm$0.044 & ZTF & g \\
80.9606 & 15.531$\pm$0.039 & ZTF & g \\
80.9606 & 15.531$\pm$0.039 & ZTF & g \\
81.6077 & 14.961$\pm$0.007 & ATLAS & o \\
81.6106 & 14.955$\pm$0.007 & ATLAS & o \\
81.6161 & 14.972$\pm$0.007 & ATLAS & o \\
81.6329 & 14.957$\pm$0.008 & ATLAS & o \\
83.8146 & 14.945$\pm$0.007 & ATLAS & o \\
83.8197 & 14.952$\pm$0.007 & ATLAS & o \\
83.8234 & 14.933$\pm$0.007 & ATLAS & o \\
83.8346 & 14.943$\pm$0.007 & ATLAS & o \\
83.9219 & 15.471$\pm$0.029 & ZTF & g \\
83.9219 & 15.471$\pm$0.029 & ZTF & g \\
83.9229 & 15.467$\pm$0.033 & ZTF & g \\
83.9229 & 15.468$\pm$0.033 & ZTF & g \\
83.9692 & 15.117$\pm$0.031 & ZTF & r \\
83.9692 & 15.117$\pm$0.031 & ZTF & r \\
83.9697 & 15.070$\pm$0.027 & ZTF & r \\
83.9697 & 15.070$\pm$0.027 & ZTF & r \\
84.9872 & 15.464$\pm$0.040 & ASAS-SN & g \\
85.0699 & 15.314$\pm$0.008 & ATLAS & c \\
85.0731 & 15.314$\pm$0.008 & ATLAS & c \\
85.0785 & 15.292$\pm$0.008 & ATLAS & c \\
85.0971 & 15.300$\pm$0.008 & ATLAS & c \\
85.4616 & 15.573$\pm$0.051 & ASAS-SN & g \\
85.5648 & 15.323$\pm$0.008 & ATLAS & c \\
85.5676 & 15.310$\pm$0.008 & ATLAS & c \\
85.5744 & 15.330$\pm$0.008 & ATLAS & c \\
85.6048 & 15.297$\pm$0.008 & ATLAS & c \\
86.8618 & 15.146$\pm$0.041 & P60 & r \\
86.8635 & 15.096$\pm$0.041 & P60 & i \\
86.9602 & 15.550$\pm$0.030 & ZTF & g \\
86.9723 & 15.413$\pm$0.114 & ASAS-SN & g \\
87.0694 & 15.028$\pm$0.008 & ATLAS & o \\
87.0726 & 15.028$\pm$0.008 & ATLAS & o \\
87.0771 & 15.055$\pm$0.008 & ATLAS & o \\
87.0906 & 15.036$\pm$0.008 & ATLAS & o \\
87.8822 & 15.036$\pm$0.007 & ATLAS & o \\
87.8859 & 15.040$\pm$0.007 & ATLAS & o \\
87.8927 & 15.021$\pm$0.007 & ATLAS & o \\
87.9420 & 15.574$\pm$0.064 & ASAS-SN & g \\
89.0577 & 15.439$\pm$0.009 & ATLAS & c \\
89.0605 & 15.435$\pm$0.009 & ATLAS & c \\
89.0636 & 15.430$\pm$0.009 & ATLAS & c \\
89.0700 & 15.405$\pm$0.009 & ATLAS & c \\
90.8738 & 15.619$\pm$0.035 & ZTF & g \\
90.8738 & 15.619$\pm$0.035 & ZTF & g \\
90.9718 & 15.528$\pm$0.042 & ASAS-SN & g \\
91.8706 & 15.480$\pm$0.010 & ATLAS & c \\
91.8738 & 15.471$\pm$0.009 & ATLAS & c \\
91.9022 & 15.488$\pm$0.009 & ATLAS & c \\
91.9082 & 15.486$\pm$0.009 & ATLAS & c \\
91.9406 & 15.512$\pm$0.014 & ATLAS & c \\
92.4687 & 15.772$\pm$0.054 & ASAS-SN & g \\
93.0941 & 15.563$\pm$0.009 & ATLAS & c \\
93.0969 & 15.531$\pm$0.009 & ATLAS & c \\
93.1204 & 15.509$\pm$0.010 & ATLAS & c \\
93.1248 & 15.533$\pm$0.010 & ATLAS & c \\
93.7074 & 15.795$\pm$0.056 & ASAS-SN & g \\
93.9448 & 15.704$\pm$0.034 & ZTF & g \\
93.9448 & 15.704$\pm$0.034 & ZTF & g \\
94.7136 & 15.651$\pm$0.046 & ASAS-SN & g \\
94.9198 & 14.946$\pm$0.028 & ZTF & i \\
94.9198 & 14.946$\pm$0.028 & ZTF & i \\
94.9340 & 14.943$\pm$0.035 & ZTF & i \\
95.1028 & 15.240$\pm$0.009 & ATLAS & o \\
95.1075 & 15.229$\pm$0.009 & ATLAS & o \\
95.1150 & 15.234$\pm$0.010 & ATLAS & o \\
95.1228 & 15.237$\pm$0.010 & ATLAS & o \\
95.8213 & 15.631$\pm$0.045 & ASAS-SN & g \\
95.9198 & 15.651$\pm$0.041 & ZTF & g \\
95.9198 & 15.651$\pm$0.041 & ZTF & g \\
95.9405 & 15.301$\pm$0.044 & ZTF & r \\
95.9405 & 15.301$\pm$0.044 & ZTF & r \\
95.9415 & 15.280$\pm$0.044 & ZTF & r \\
95.9415 & 15.280$\pm$0.044 & ZTF & r \\
95.9420 & 15.311$\pm$0.043 & P60 & r \\
95.9436 & 15.280$\pm$0.042 & P60 & i \\
96.8122 & 15.546$\pm$0.045 & ASAS-SN & g \\
97.1056 & 15.437$\pm$0.009 & ATLAS & c \\
97.1120 & 15.434$\pm$0.009 & ATLAS & c \\
97.1246 & 15.445$\pm$0.011 & ATLAS & c \\
97.1279 & 15.417$\pm$0.013 & ATLAS & c \\
97.5938 & 15.440$\pm$0.008 & ATLAS & c \\
97.5981 & 15.461$\pm$0.009 & ATLAS & c \\
97.6037 & 15.470$\pm$0.009 & ATLAS & c \\
97.6138 & 15.444$\pm$0.010 & ATLAS & c \\
97.6847 & 15.483$\pm$0.011 & ATLAS & c \\
98.9191 & 15.576$\pm$0.041 & ZTF & g \\
98.9191 & 15.576$\pm$0.041 & ZTF & g \\
98.9410 & 15.295$\pm$0.028 & ZTF & r \\
98.9410 & 15.295$\pm$0.028 & ZTF & r \\
98.9414 & 15.288$\pm$0.021 & ZTF & r \\
98.9414 & 15.288$\pm$0.021 & ZTF & r \\
99.7597 & 15.149$\pm$0.012 & ATLAS & o \\
99.7624 & 15.161$\pm$0.012 & ATLAS & o \\
99.7784 & 15.151$\pm$0.010 & ATLAS & o \\
99.7839 & 15.167$\pm$0.009 & ATLAS & o \\
100.6916 & 15.424$\pm$0.080 & ASAS-SN & g \\
101.0257 & 15.200$\pm$0.009 & ATLAS & o \\
101.0276 & 15.183$\pm$0.009 & ATLAS & o \\
101.0303 & 15.168$\pm$0.009 & ATLAS & o \\
101.0479 & 15.098$\pm$0.008 & ATLAS & o \\
101.5057 & 15.189$\pm$0.009 & ATLAS & o \\
101.5094 & 15.175$\pm$0.009 & ATLAS & o \\
101.5158 & 15.193$\pm$0.009 & ATLAS & o \\
101.5256 & 15.174$\pm$0.009 & ATLAS & o \\
101.7828 & 15.201$\pm$0.014 & ATLAS & o \\
101.7855 & 15.192$\pm$0.011 & ATLAS & o \\
101.8135 & 15.239$\pm$0.027 & ATLAS & o \\
101.8177 & 15.159$\pm$0.016 & ATLAS & o \\
101.8991 & 15.655$\pm$0.035 & ZTF & g \\
101.8991 & 15.655$\pm$0.035 & ZTF & g \\
101.9185 & 15.677$\pm$0.049 & ZTF & g \\
101.9185 & 15.677$\pm$0.049 & ZTF & g \\
102.6790 & 15.171$\pm$0.014 & ATLAS & o \\
102.6822 & 15.177$\pm$0.014 & ATLAS & o \\
102.6883 & 15.188$\pm$0.013 & ATLAS & o \\
102.7083 & 15.133$\pm$0.023 & ATLAS & o \\
102.8366 & 15.355$\pm$0.043 & P60 & r \\
102.8386 & 15.322$\pm$0.043 & P60 & i \\
103.0076 & 15.275$\pm$0.049 & ATLAS & o \\
103.0308 & 15.283$\pm$0.044 & ATLAS & o \\
103.0326 & 15.283$\pm$0.042 & ATLAS & o \\
103.0399 & 15.309$\pm$0.061 & ATLAS & o \\
103.7153 & 15.227$\pm$0.043 & ATLAS & o \\
103.8781 & 15.407$\pm$0.024 & ZTF & r \\
103.8997 & 15.420$\pm$0.041 & ZTF & r \\
103.9564 & 15.693$\pm$0.032 & ZTF & g \\
104.7242 & 15.722$\pm$0.126 & ASAS-SN & g \\
107.8148 & 15.420$\pm$0.045 & P60 & r \\
107.8168 & 15.315$\pm$0.043 & P60 & i \\
107.8668 & 15.451$\pm$0.033 & ZTF & r \\
107.9407 & 15.708$\pm$0.049 & ZTF & g \\
108.9355 & 15.394$\pm$0.032 & ZTF & r \\
108.9435 & 15.668$\pm$0.064 & ASAS-SN & g \\
109.0615 & 15.273$\pm$0.009 & ATLAS & o \\
109.0667 & 15.270$\pm$0.010 & ATLAS & o \\
109.1021 & 15.289$\pm$0.010 & ATLAS & o \\
109.1265 & 15.292$\pm$0.009 & ATLAS & o \\
109.8508 & 15.388$\pm$0.044 & P60 & r \\
109.8528 & 15.352$\pm$0.043 & P60 & i \\
109.9395 & 14.984$\pm$0.049 & ZTF & i \\
110.8770 & 15.632$\pm$0.034 & ZTF & g \\
110.8770 & 15.632$\pm$0.034 & ZTF & g \\
110.9135 & 15.642$\pm$0.043 & ZTF & g \\
110.9135 & 15.642$\pm$0.043 & ZTF & g \\
110.9397 & 15.428$\pm$0.027 & ZTF & r \\
110.9397 & 15.428$\pm$0.027 & ZTF & r \\
110.9747 & 15.326$\pm$0.010 & ATLAS & o \\
110.9811 & 15.351$\pm$0.011 & ATLAS & o \\
110.9867 & 15.337$\pm$0.011 & ATLAS & o \\
110.9917 & 15.350$\pm$0.010 & ATLAS & o \\
113.0424 & 15.366$\pm$0.011 & ATLAS & o \\
113.0478 & 15.371$\pm$0.010 & ATLAS & o \\
113.0831 & 15.368$\pm$0.009 & ATLAS & o \\
113.0863 & 15.381$\pm$0.009 & ATLAS & o \\
113.5482 & 15.383$\pm$0.009 & ATLAS & o \\
113.5514 & 15.370$\pm$0.009 & ATLAS & o \\
113.5843 & 15.364$\pm$0.009 & ATLAS & o \\
113.5898 & 15.397$\pm$0.011 & ATLAS & o \\
113.8361 & 15.775$\pm$0.027 & ZTF & g \\
113.8361 & 15.775$\pm$0.027 & ZTF & g \\
113.9200 & 15.525$\pm$0.023 & ZTF & r \\
113.9200 & 15.525$\pm$0.023 & ZTF & r \\
114.6117 & 15.856$\pm$0.064 & ASAS-SN & g \\
114.8975 & 15.533$\pm$0.045 & P60 & r \\
114.8995 & 15.264$\pm$0.042 & P60 & i \\
115.0114 & 15.483$\pm$0.012 & ATLAS & o \\
115.0133 & 15.479$\pm$0.012 & ATLAS & o \\
115.0188 & 15.506$\pm$0.012 & ATLAS & o \\
115.0545 & 15.478$\pm$0.011 & ATLAS & o \\
115.4898 & 15.957$\pm$0.063 & ASAS-SN & g \\
115.9198 & 15.827$\pm$0.039 & ZTF & g \\
115.9198 & 15.827$\pm$0.039 & ZTF & g \\
115.9627 & 15.593$\pm$0.025 & ZTF & r \\
115.9627 & 15.593$\pm$0.025 & ZTF & r \\
117.8792 & 15.668$\pm$0.028 & ZTF & r \\
117.8792 & 15.668$\pm$0.028 & ZTF & r \\
117.8802 & 15.668$\pm$0.039 & ZTF & r \\
117.8802 & 15.668$\pm$0.039 & ZTF & r \\
117.9063 & 15.886$\pm$0.039 & ZTF & g \\
117.9063 & 15.886$\pm$0.039 & ZTF & g \\
117.9073 & 15.890$\pm$0.034 & ZTF & g \\
117.9073 & 15.890$\pm$0.034 & ZTF & g \\
118.9947 & 15.593$\pm$0.011 & ATLAS & o \\
118.9989 & 15.595$\pm$0.011 & ATLAS & o \\
119.0016 & 15.599$\pm$0.012 & ATLAS & o \\
119.0236 & 15.601$\pm$0.011 & ATLAS & o \\
119.6638 & 15.787$\pm$0.012 & ATLAS & c \\
119.6841 & 15.844$\pm$0.011 & ATLAS & c \\
119.7103 & 15.816$\pm$0.011 & ATLAS & c \\
119.7198 & 15.829$\pm$0.011 & ATLAS & c \\
119.7803 & 15.714$\pm$0.048 & P60 & r \\
119.7823 & 15.689$\pm$0.048 & P60 & i \\
119.8792 & 15.900$\pm$0.037 & ZTF & g \\
119.8792 & 15.900$\pm$0.037 & ZTF & g \\
119.8982 & 15.900$\pm$0.031 & ZTF & g \\
119.8982 & 15.900$\pm$0.031 & ZTF & g \\
121.0059 & 15.760$\pm$0.011 & ATLAS & c \\
121.0091 & 15.794$\pm$0.012 & ATLAS & c \\
121.0192 & 15.800$\pm$0.011 & ATLAS & c \\
121.0446 & 15.764$\pm$0.011 & ATLAS & c \\
122.8785 & 15.868$\pm$0.030 & ZTF & g \\
122.8785 & 15.868$\pm$0.030 & ZTF & g \\
122.8991 & 15.865$\pm$0.037 & ZTF & g \\
122.8991 & 15.865$\pm$0.037 & ZTF & g \\
122.9737 & 15.685$\pm$0.021 & ZTF & r \\
122.9737 & 15.685$\pm$0.021 & ZTF & r \\
123.0329 & 15.561$\pm$0.011 & ATLAS & o \\
123.0370 & 15.574$\pm$0.011 & ATLAS & o \\
123.0644 & 15.557$\pm$0.012 & ATLAS & o \\
123.0927 & 15.538$\pm$0.012 & ATLAS & o \\
123.7967 & 15.765$\pm$0.012 & ATLAS & c \\
123.7999 & 15.775$\pm$0.011 & ATLAS & c \\
123.8265 & 15.797$\pm$0.011 & ATLAS & c \\
123.8296 & 15.888$\pm$0.015 & ATLAS & c \\
123.8328 & 15.777$\pm$0.013 & ATLAS & c \\
123.8332 & 15.847$\pm$0.016 & ATLAS & c \\
124.8942 & 15.688$\pm$0.028 & ZTF & r \\
124.8942 & 15.688$\pm$0.028 & ZTF & r \\
124.9426 & 15.368$\pm$0.042 & ZTF & i \\
124.9426 & 15.368$\pm$0.042 & ZTF & i \\
125.0551 & 15.846$\pm$0.010 & ATLAS & c \\
125.0894 & 15.838$\pm$0.011 & ATLAS & c \\
125.1179 & 15.851$\pm$0.011 & ATLAS & c \\
125.4809 & 15.575$\pm$0.010 & ATLAS & o \\
125.4828 & 15.602$\pm$0.010 & ATLAS & o \\
125.4859 & 15.611$\pm$0.010 & ATLAS & o \\
125.5041 & 15.608$\pm$0.011 & ATLAS & o \\
126.8565 & 15.982$\pm$0.031 & ZTF & g \\
126.8565 & 15.982$\pm$0.031 & ZTF & g \\
126.8746 & 15.952$\pm$0.041 & ZTF & g \\
126.8746 & 15.952$\pm$0.041 & ZTF & g \\
126.9583 & 15.650$\pm$0.011 & ATLAS & o \\
126.9601 & 15.680$\pm$0.011 & ATLAS & o \\
126.9832 & 15.639$\pm$0.013 & ATLAS & o \\
126.9873 & 15.651$\pm$0.012 & ATLAS & o \\
127.8977 & 15.350$\pm$0.029 & ZTF & i \\
127.8977 & 15.350$\pm$0.029 & ZTF & i \\
129.4461 & 15.727$\pm$0.012 & ATLAS & o \\
129.4516 & 15.716$\pm$0.013 & ATLAS & o \\
129.4557 & 15.722$\pm$0.013 & ATLAS & o \\
129.4611 & 15.698$\pm$0.013 & ATLAS & o \\
129.6241 & 15.793$\pm$0.021 & ATLAS & o \\
129.8977 & 16.054$\pm$0.030 & ZTF & g \\
129.8977 & 16.054$\pm$0.030 & ZTF & g \\
129.9194 & 15.870$\pm$0.023 & ZTF & r \\
129.9194 & 15.870$\pm$0.023 & ZTF & r \\
130.7369 & 15.902$\pm$0.052 & P60 & r \\
130.7389 & 15.886$\pm$0.052 & P60 & i \\
130.8904 & 15.821$\pm$0.020 & ATLAS & o \\
130.8936 & 15.767$\pm$0.020 & ATLAS & o \\
130.9168 & 15.834$\pm$0.021 & ATLAS & o \\
130.9209 & 15.594$\pm$0.107 & ATLAS & o \\
131.5102 & 15.769$\pm$0.019 & ATLAS & o \\
131.5159 & 15.809$\pm$0.021 & ATLAS & o \\
131.5497 & 15.772$\pm$0.019 & ATLAS & o \\
131.5527 & 15.789$\pm$0.021 & ATLAS & o \\
137.0675 & 15.753$\pm$0.016 & ATLAS & o \\
137.0710 & 15.750$\pm$0.016 & ATLAS & o \\
137.0764 & 15.766$\pm$0.015 & ATLAS & o \\
137.0873 & 15.722$\pm$0.014 & ATLAS & o \\
137.4984 & 15.734$\pm$0.015 & ATLAS & o \\
137.5039 & 15.755$\pm$0.017 & ATLAS & o \\
137.5071 & 15.742$\pm$0.018 & ATLAS & o \\
137.5175 & 15.801$\pm$0.017 & ATLAS & o \\
138.7395 & 15.845$\pm$0.049 & P60 & r \\
138.7412 & 15.847$\pm$0.049 & P60 & i \\
138.9782 & 15.788$\pm$0.012 & ATLAS & o \\
138.9810 & 15.776$\pm$0.013 & ATLAS & o \\
138.9864 & 15.790$\pm$0.012 & ATLAS & o \\
139.0217 & 15.800$\pm$0.013 & ATLAS & o \\
139.7343 & 15.551$\pm$0.178 & ATLAS & o \\
139.7700 & 15.865$\pm$0.140 & ATLAS & o \\
139.7731 & 15.836$\pm$0.116 & ATLAS & o \\
139.7785 & 15.527$\pm$0.151 & ATLAS & o \\
139.8158 & 16.085$\pm$0.040 & ZTF & g \\
139.8158 & 16.085$\pm$0.040 & ZTF & g \\
139.8515 & 16.106$\pm$0.032 & ZTF & g \\
139.8515 & 16.106$\pm$0.032 & ZTF & g \\
139.8579 & 16.065$\pm$0.045 & ZTF & g \\
139.8579 & 16.064$\pm$0.045 & ZTF & g \\
139.8762 & 16.101$\pm$0.031 & ZTF & g \\
139.8762 & 16.101$\pm$0.031 & ZTF & g \\
140.8561 & 16.096$\pm$0.041 & ZTF & g \\
140.8561 & 16.096$\pm$0.041 & ZTF & g \\
140.8750 & 16.129$\pm$0.027 & ZTF & g \\
140.8750 & 16.129$\pm$0.027 & ZTF & g \\
140.9697 & 15.832$\pm$0.013 & ATLAS & o \\
140.9729 & 15.840$\pm$0.013 & ATLAS & o \\
140.9783 & 15.834$\pm$0.014 & ATLAS & o \\
140.9886 & 15.808$\pm$0.011 & ATLAS & o \\
141.8428 & 16.145$\pm$0.027 & ZTF & g \\
141.8428 & 16.145$\pm$0.027 & ZTF & g \\
141.8438 & 16.127$\pm$0.027 & ZTF & g \\
141.8438 & 16.127$\pm$0.027 & ZTF & g \\
141.8592 & 16.111$\pm$0.040 & ZTF & g \\
141.8592 & 16.111$\pm$0.040 & ZTF & g \\
141.8883 & 16.133$\pm$0.030 & ZTF & g \\
141.8883 & 16.133$\pm$0.030 & ZTF & g \\
142.8349 & 15.568$\pm$0.029 & ZTF & i \\
142.8349 & 15.568$\pm$0.029 & ZTF & i \\
142.9205 & 16.122$\pm$0.016 & ATLAS & c \\
142.9223 & 16.123$\pm$0.017 & ATLAS & c \\
142.9251 & 16.103$\pm$0.015 & ATLAS & c \\
142.9302 & 16.115$\pm$0.015 & ATLAS & c \\
143.6578 & 15.873$\pm$0.013 & ATLAS & o \\
143.6605 & 15.895$\pm$0.013 & ATLAS & o \\
143.6660 & 15.914$\pm$0.012 & ATLAS & o \\
143.6758 & 15.897$\pm$0.013 & ATLAS & o \\
143.7963 & 16.063$\pm$0.036 & ZTF & r \\
143.7963 & 16.063$\pm$0.036 & ZTF & r \\
143.8109 & 16.049$\pm$0.053 & P60 & r \\
143.8142 & 16.019$\pm$0.052 & P60 & i \\
143.8162 & 16.152$\pm$0.048 & ZTF & g \\
143.8162 & 16.152$\pm$0.048 & ZTF & g \\
143.8362 & 16.165$\pm$0.027 & ZTF & g \\
143.8362 & 16.165$\pm$0.027 & ZTF & g \\
144.9129 & 15.903$\pm$0.014 & ATLAS & o \\
144.9147 & 15.916$\pm$0.013 & ATLAS & o \\
144.9365 & 15.916$\pm$0.014 & ATLAS & o \\
144.9419 & 15.888$\pm$0.015 & ATLAS & o \\
146.8712 & 16.106$\pm$0.029 & ZTF & g \\
146.8712 & 16.106$\pm$0.029 & ZTF & g \\
146.8996 & 15.975$\pm$0.027 & ZTF & r \\
146.8996 & 15.975$\pm$0.027 & ZTF & r \\
147.0465 & 16.125$\pm$0.113 & ATLAS & c \\
147.0530 & 15.792$\pm$0.078 & ATLAS & c \\
148.8370 & 16.005$\pm$0.025 & ZTF & r \\
148.8370 & 16.005$\pm$0.025 & ZTF & r \\
148.8578 & 16.053$\pm$0.025 & ZTF & g \\
148.8578 & 16.053$\pm$0.025 & ZTF & g \\
148.9169 & 15.828$\pm$0.014 & ATLAS & o \\
148.9187 & 15.819$\pm$0.012 & ATLAS & o \\
148.9219 & 15.833$\pm$0.013 & ATLAS & o \\
148.9425 & 15.815$\pm$0.014 & ATLAS & o \\
149.5328 & 16.017$\pm$0.014 & ATLAS & c \\
149.5360 & 16.035$\pm$0.012 & ATLAS & c \\
149.5419 & 16.028$\pm$0.012 & ATLAS & c \\
149.5657 & 16.060$\pm$0.013 & ATLAS & c \\
149.7839 & 16.084$\pm$0.034 & ZTF & g \\
149.7839 & 16.084$\pm$0.034 & ZTF & g \\
149.8166 & 15.994$\pm$0.036 & ZTF & r \\
149.8166 & 15.994$\pm$0.036 & ZTF & r \\
150.8154 & 16.051$\pm$0.029 & ZTF & r \\
150.8154 & 16.051$\pm$0.029 & ZTF & r \\
150.8781 & 16.111$\pm$0.032 & ZTF & g \\
150.8781 & 16.111$\pm$0.032 & ZTF & g \\
150.9071 & 16.138$\pm$0.014 & ATLAS & c \\
150.9089 & 16.084$\pm$0.012 & ATLAS & c \\
150.9136 & 16.128$\pm$0.013 & ATLAS & c \\
150.9187 & 16.105$\pm$0.013 & ATLAS & c \\
151.6519 & 15.867$\pm$0.011 & ATLAS & o \\
151.6546 & 15.855$\pm$0.012 & ATLAS & o \\
151.6600 & 15.868$\pm$0.015 & ATLAS & o \\
151.6822 & 15.884$\pm$0.015 & ATLAS & o \\
151.7730 & 16.118$\pm$0.035 & ZTF & g \\
151.7730 & 16.118$\pm$0.035 & ZTF & g \\
151.7951 & 16.044$\pm$0.037 & ZTF & r \\
151.7951 & 16.044$\pm$0.037 & ZTF & r \\
152.8157 & 16.061$\pm$0.030 & ZTF & r \\
152.8157 & 16.061$\pm$0.030 & ZTF & r \\
152.8507 & 16.161$\pm$0.034 & ZTF & g \\
152.8507 & 16.161$\pm$0.034 & ZTF & g \\
153.4085 & 16.130$\pm$0.013 & ATLAS & c \\
153.4103 & 16.105$\pm$0.013 & ATLAS & c \\
153.4121 & 16.095$\pm$0.013 & ATLAS & c \\
153.4135 & 16.057$\pm$0.013 & ATLAS & c \\
153.4230 & 16.135$\pm$0.014 & ATLAS & c \\
153.4326 & 16.153$\pm$0.013 & ATLAS & c \\
153.8218 & 16.110$\pm$0.053 & P60 & r \\
153.8272 & 16.090$\pm$0.053 & P60 & i \\
154.8271 & 16.103$\pm$0.053 & P60 & r \\
154.8327 & 16.062$\pm$0.052 & P60 & i \\
154.9848 & 16.245$\pm$0.014 & ATLAS & c \\
154.9947 & 16.217$\pm$0.015 & ATLAS & c \\
155.0229 & 16.193$\pm$0.014 & ATLAS & c \\
155.0325 & 16.191$\pm$0.015 & ATLAS & c \\
155.7303 & 15.984$\pm$0.014 & ATLAS & o \\
155.7334 & 15.947$\pm$0.015 & ATLAS & o \\
155.7683 & 15.816$\pm$0.014 & ATLAS & o \\
155.7966 & 16.010$\pm$0.015 & ATLAS & o \\
155.8257 & 16.222$\pm$0.030 & ZTF & g \\
155.8257 & 16.222$\pm$0.030 & ZTF & g \\
155.8825 & 16.148$\pm$0.035 & ZTF & r \\
155.8825 & 16.148$\pm$0.035 & ZTF & r \\
156.3734 & 16.037$\pm$0.095 & ATLAS & o \\
156.3757 & 15.966$\pm$0.077 & ATLAS & o \\
156.3940 & 16.020$\pm$0.036 & ATLAS & o \\
156.3990 & 16.050$\pm$0.036 & ATLAS & o \\
156.7829 & 16.233$\pm$0.036 & ZTF & g \\
156.7829 & 16.233$\pm$0.036 & ZTF & g \\
157.3689 & 16.023$\pm$0.020 & ATLAS & o \\
157.3707 & 16.096$\pm$0.021 & ATLAS & o \\
157.3748 & 16.016$\pm$0.017 & ATLAS & o \\
157.3802 & 16.032$\pm$0.018 & ATLAS & o \\
157.6710 & 16.096$\pm$0.054 & P60 & r \\
157.6744 & 15.874$\pm$0.051 & P60 & i \\
157.8038 & 16.174$\pm$0.029 & ZTF & g \\
157.8038 & 16.174$\pm$0.029 & ZTF & g \\
157.8189 & 15.677$\pm$0.036 & ZTF & i \\
157.8189 & 15.677$\pm$0.036 & ZTF & i \\
157.8926 & 16.129$\pm$0.034 & ZTF & r \\
157.8926 & 16.129$\pm$0.034 & ZTF & r \\
158.6099 & 15.939$\pm$0.021 & ATLAS & o \\
158.6126 & 15.969$\pm$0.021 & ATLAS & o \\
158.6331 & 15.935$\pm$0.018 & ATLAS & o \\
158.6512 & 15.966$\pm$0.021 & ATLAS & o \\
158.8164 & 16.056$\pm$0.035 & ZTF & r \\
158.8164 & 16.056$\pm$0.035 & ZTF & r \\
158.8899 & 16.123$\pm$0.056 & ZTF & g \\
158.8899 & 16.123$\pm$0.056 & ZTF & g \\
158.9364 & 15.917$\pm$0.015 & ATLAS & o \\
158.9396 & 15.941$\pm$0.016 & ATLAS & o \\
158.9672 & 15.957$\pm$0.018 & ATLAS & o \\
158.9753 & 15.968$\pm$0.021 & ATLAS & o \\
159.8257 & 16.103$\pm$0.042 & ZTF & r \\
159.8257 & 16.103$\pm$0.042 & ZTF & r \\
159.8987 & 16.113$\pm$0.033 & ZTF & g \\
159.8987 & 16.113$\pm$0.033 & ZTF & g \\
162.7945 & 16.153$\pm$0.019 & ZTF & r \\
162.7945 & 16.153$\pm$0.019 & ZTF & r \\
163.6823 & 16.168$\pm$0.055 & P60 & r \\
163.6839 & 16.140$\pm$0.054 & P60 & i \\
163.8286 & 16.181$\pm$0.033 & ZTF & g \\
163.8286 & 16.181$\pm$0.033 & ZTF & g \\
164.7663 & 16.193$\pm$0.021 & ZTF & r \\
164.7663 & 16.193$\pm$0.021 & ZTF & r \\
164.8828 & 16.241$\pm$0.039 & ZTF & g \\
164.8828 & 16.241$\pm$0.039 & ZTF & g \\
164.9132 & 16.105$\pm$0.024 & ATLAS & o \\
164.9164 & 16.018$\pm$0.018 & ATLAS & o \\
164.9223 & 16.090$\pm$0.018 & ATLAS & o \\
164.9259 & 16.092$\pm$0.022 & ATLAS & o \\
164.9291 & 16.077$\pm$0.019 & ATLAS & o \\
164.9322 & 16.038$\pm$0.020 & ATLAS & o \\
164.9350 & 16.032$\pm$0.065 & ATLAS & o \\
165.8283 & 16.220$\pm$0.031 & ZTF & r \\
165.8283 & 16.220$\pm$0.031 & ZTF & r \\
165.8408 & 16.427$\pm$0.034 & ZTF & r \\
165.8408 & 16.427$\pm$0.034 & ZTF & r \\
166.7223 & 16.255$\pm$0.057 & P60 & r \\
166.7240 & 16.194$\pm$0.055 & P60 & i \\
166.7666 & 16.270$\pm$0.029 & ZTF & g \\
166.7666 & 16.270$\pm$0.029 & ZTF & g \\
166.8406 & 16.208$\pm$0.016 & ZTF & r \\
166.8406 & 16.208$\pm$0.016 & ZTF & r \\
166.9250 & 16.125$\pm$0.022 & ATLAS & o \\
166.9282 & 16.129$\pm$0.022 & ATLAS & o \\
166.9338 & 16.167$\pm$0.021 & ATLAS & o \\
166.9442 & 16.178$\pm$0.063 & ATLAS & o \\
167.8072 & 16.369$\pm$0.025 & ZTF & g \\
167.8072 & 16.369$\pm$0.025 & ZTF & g \\
167.8216 & 16.278$\pm$0.025 & ZTF & r \\
167.8216 & 16.278$\pm$0.025 & ZTF & r \\
168.9019 & 16.197$\pm$0.018 & ATLAS & o \\
168.9051 & 16.197$\pm$0.017 & ATLAS & o \\
168.9110 & 16.200$\pm$0.018 & ATLAS & o \\
168.9251 & 16.189$\pm$0.017 & ATLAS & o \\
170.7948 & 16.249$\pm$0.024 & ZTF & r \\
170.7948 & 16.249$\pm$0.024 & ZTF & r \\
170.8890 & 16.122$\pm$0.013 & ATLAS & o \\
170.8919 & 16.075$\pm$0.015 & ATLAS & o \\
170.8970 & 16.128$\pm$0.013 & ATLAS & o \\
170.9314 & 16.108$\pm$0.016 & ATLAS & o \\
171.6838 & 16.342$\pm$0.018 & ATLAS & c \\
171.6893 & 16.250$\pm$0.016 & ATLAS & c \\
171.7198 & 16.235$\pm$0.015 & ATLAS & c \\
171.7229 & 16.268$\pm$0.017 & ATLAS & c \\
171.7308 & 16.240$\pm$0.028 & ZTF & g \\
171.7308 & 16.240$\pm$0.028 & ZTF & g \\
171.7905 & 16.230$\pm$0.028 & ZTF & r \\
171.7905 & 16.231$\pm$0.028 & ZTF & r \\
172.7626 & 15.732$\pm$0.041 & ZTF & i \\
172.7626 & 15.732$\pm$0.041 & ZTF & i \\
172.8085 & 16.222$\pm$0.021 & ZTF & g \\
172.8085 & 16.221$\pm$0.021 & ZTF & g \\
172.8583 & 16.261$\pm$0.028 & ZTF & r \\
172.8583 & 16.261$\pm$0.028 & ZTF & r \\
172.8815 & 16.281$\pm$0.016 & ATLAS & c \\
172.9161 & 16.255$\pm$0.016 & ATLAS & c \\
172.9193 & 16.243$\pm$0.016 & ATLAS & c \\
172.9293 & 16.280$\pm$0.015 & ATLAS & c \\
173.3867 & 16.096$\pm$0.018 & ATLAS & o \\
173.3899 & 16.086$\pm$0.017 & ATLAS & o \\
173.3958 & 16.112$\pm$0.016 & ATLAS & o \\
173.4308 & 16.160$\pm$0.044 & ATLAS & o \\
173.7022 & 16.224$\pm$0.056 & P60 & r \\
173.7039 & 16.181$\pm$0.055 & P60 & i \\
173.7597 & 16.259$\pm$0.039 & ZTF & g \\
173.7597 & 16.259$\pm$0.039 & ZTF & g \\
174.7098 & 16.271$\pm$0.030 & ZTF & g \\
174.7098 & 16.271$\pm$0.030 & ZTF & g \\
174.7726 & 16.322$\pm$0.032 & ZTF & r \\
174.7726 & 16.322$\pm$0.032 & ZTF & r \\
174.8971 & 16.035$\pm$0.052 & P60 & i \\
174.9445 & 16.139$\pm$0.014 & ATLAS & o \\
174.9501 & 16.155$\pm$0.015 & ATLAS & o \\
174.9528 & 16.162$\pm$0.015 & ATLAS & o \\
174.9635 & 16.143$\pm$0.015 & ATLAS & o \\
175.6624 & 16.313$\pm$0.015 & ATLAS & c \\
175.6665 & 16.324$\pm$0.016 & ATLAS & c \\
175.6918 & 16.320$\pm$0.014 & ATLAS & c \\
175.6973 & 16.320$\pm$0.017 & ATLAS & c \\
176.7896 & 16.352$\pm$0.035 & ZTF & g \\
176.7896 & 16.352$\pm$0.035 & ZTF & g \\
176.8836 & 16.410$\pm$0.017 & ATLAS & c \\
176.8868 & 16.347$\pm$0.016 & ATLAS & c \\
176.8927 & 16.376$\pm$0.016 & ATLAS & c \\
176.9028 & 16.344$\pm$0.018 & ATLAS & c \\
177.3812 & 16.172$\pm$0.017 & ATLAS & o \\
177.3848 & 16.225$\pm$0.015 & ATLAS & o \\
177.3903 & 16.188$\pm$0.016 & ATLAS & o \\
177.4252 & 16.270$\pm$0.033 & ATLAS & o \\
177.8372 & 16.348$\pm$0.036 & ZTF & r \\
177.8372 & 16.348$\pm$0.036 & ZTF & r \\
178.7102 & 16.386$\pm$0.039 & ZTF & g \\
178.7102 & 16.386$\pm$0.039 & ZTF & g \\
178.7341 & 16.377$\pm$0.022 & ZTF & r \\
178.7341 & 16.377$\pm$0.022 & ZTF & r \\
178.8659 & 16.290$\pm$0.019 & ATLAS & o \\
178.8691 & 16.289$\pm$0.019 & ATLAS & o \\
178.8747 & 16.301$\pm$0.018 & ATLAS & o \\
178.8873 & 16.264$\pm$0.019 & ATLAS & o \\
179.6305 & 16.374$\pm$0.017 & ATLAS & c \\
179.6638 & 16.429$\pm$0.017 & ATLAS & c \\
179.6670 & 16.407$\pm$0.016 & ATLAS & c \\
179.6724 & 16.413$\pm$0.016 & ATLAS & c \\
179.7732 & 16.409$\pm$0.034 & ZTF & r \\
179.7732 & 16.408$\pm$0.034 & ZTF & r \\
179.8309 & 16.456$\pm$0.035 & ZTF & g \\
179.8309 & 16.456$\pm$0.035 & ZTF & g \\
180.7330 & 16.435$\pm$0.041 & ZTF & g \\
180.7330 & 16.435$\pm$0.041 & ZTF & g \\
180.7730 & 15.965$\pm$0.030 & ZTF & i \\
180.7730 & 15.965$\pm$0.030 & ZTF & i \\
180.7740 & 15.936$\pm$0.035 & ZTF & i \\
180.7740 & 15.936$\pm$0.035 & ZTF & i \\
180.9260 & 16.408$\pm$0.017 & ATLAS & c \\
180.9296 & 16.453$\pm$0.017 & ATLAS & c \\
180.9359 & 16.448$\pm$0.019 & ATLAS & c \\
180.9605 & 16.494$\pm$0.020 & ATLAS & c \\
181.2474 & 16.322$\pm$0.024 & ATLAS & o \\
181.2497 & 16.333$\pm$0.023 & ATLAS & o \\
181.2501 & 16.345$\pm$0.019 & ATLAS & o \\
181.2506 & 16.347$\pm$0.019 & ATLAS & o \\
181.2510 & 16.228$\pm$0.020 & ATLAS & o \\
181.2519 & 16.327$\pm$0.021 & ATLAS & o \\
181.2537 & 16.308$\pm$0.019 & ATLAS & o \\
181.2569 & 16.360$\pm$0.018 & ATLAS & o \\
181.2623 & 16.308$\pm$0.024 & ATLAS & o \\
181.7730 & 16.452$\pm$0.045 & ZTF & r \\
181.7730 & 16.452$\pm$0.045 & ZTF & r \\
181.8517 & 16.469$\pm$0.032 & ZTF & g \\
181.8517 & 16.469$\pm$0.032 & ZTF & g \\
182.7285 & 16.414$\pm$0.039 & ZTF & g \\
182.7285 & 16.414$\pm$0.039 & ZTF & g \\
182.7332 & 16.412$\pm$0.032 & ZTF & r \\
182.7332 & 16.412$\pm$0.032 & ZTF & r \\
182.8610 & 16.458$\pm$0.060 & P60 & r \\
182.8626 & 16.231$\pm$0.056 & P60 & i \\
182.8641 & 16.323$\pm$0.019 & ATLAS & o \\
182.8673 & 16.299$\pm$0.018 & ATLAS & o \\
182.8733 & 16.279$\pm$0.018 & ATLAS & o \\
182.8840 & 16.305$\pm$0.016 & ATLAS & o \\
183.6219 & 16.189$\pm$0.021 & ATLAS & o \\
183.6250 & 15.962$\pm$0.020 & ATLAS & o \\
183.6304 & 16.106$\pm$0.020 & ATLAS & o \\
183.6408 & 15.922$\pm$0.019 & ATLAS & o \\
183.7504 & 16.394$\pm$0.027 & ZTF & g \\
183.7504 & 16.394$\pm$0.027 & ZTF & g \\
183.7524 & 15.881$\pm$0.040 & ZTF & i \\
183.7524 & 15.881$\pm$0.040 & ZTF & i \\
183.7721 & 15.878$\pm$0.034 & ZTF & i \\
183.7721 & 15.878$\pm$0.034 & ZTF & i \\
183.7943 & 16.373$\pm$0.027 & ZTF & r \\
183.7943 & 16.373$\pm$0.027 & ZTF & r \\
184.8776 & 16.256$\pm$0.018 & ATLAS & o \\
184.8808 & 16.250$\pm$0.020 & ATLAS & o \\
184.8862 & 16.230$\pm$0.020 & ATLAS & o \\
184.8968 & 16.243$\pm$0.018 & ATLAS & o \\
184.9164 & 16.278$\pm$0.018 & ATLAS & o \\
185.3571 & 16.260$\pm$0.023 & ATLAS & o \\
185.7322 & 16.399$\pm$0.029 & ZTF & r \\
185.7322 & 16.399$\pm$0.029 & ZTF & r \\
185.7539 & 16.387$\pm$0.039 & ZTF & g \\
185.7539 & 16.387$\pm$0.039 & ZTF & g \\
186.8482 & 16.276$\pm$0.022 & ATLAS & o \\
186.8509 & 16.354$\pm$0.025 & ATLAS & o \\
186.8712 & 16.284$\pm$0.023 & ATLAS & o \\
186.8847 & 16.325$\pm$0.030 & ATLAS & o \\
187.7106 & 15.954$\pm$0.035 & ZTF & i \\
187.7106 & 15.954$\pm$0.035 & ZTF & i \\
191.6693 & 16.312$\pm$0.072 & ATLAS & o \\
192.6423 & 16.777$\pm$0.055 & PO & g \\
192.6441 & 16.740$\pm$0.052 & PO & g \\
192.6460 & 16.672$\pm$0.046 & PO & g \\
192.6479 & 16.703$\pm$0.056 & PO & r \\
192.6498 & 16.599$\pm$0.053 & PO & r \\
192.6516 & 16.668$\pm$0.055 & PO & r \\
192.7928 & 16.652$\pm$0.056 & PO & g \\
192.7946 & 16.703$\pm$0.055 & PO & g \\
192.7965 & 16.765$\pm$0.058 & PO & g \\
192.7983 & 16.555$\pm$0.054 & PO & r \\
192.8002 & 16.584$\pm$0.054 & PO & r \\
192.8021 & 16.704$\pm$0.057 & PO & r \\
192.9275 & 16.518$\pm$0.033 & ATLAS & o \\
192.9307 & 16.536$\pm$0.035 & ATLAS & o \\
192.9512 & 16.453$\pm$0.032 & ATLAS & o \\
192.9576 & 16.481$\pm$0.039 & ATLAS & o \\
193.4410 & 16.598$\pm$0.044 & ATLAS & o \\
193.4590 & 16.452$\pm$0.039 & ATLAS & o \\
193.4637 & 16.534$\pm$0.036 & ATLAS & o \\
193.4734 & 16.508$\pm$0.040 & ATLAS & o \\
193.6261 & 16.719$\pm$0.047 & PO & g \\
193.6279 & 16.704$\pm$0.047 & PO & g \\
193.6298 & 16.717$\pm$0.047 & PO & g \\
193.6317 & 16.642$\pm$0.051 & PO & r \\
193.6336 & 16.647$\pm$0.050 & PO & r \\
193.6354 & 16.632$\pm$0.050 & PO & r \\
193.6374 & 16.394$\pm$0.041 & PO & i \\
193.6392 & 16.387$\pm$0.040 & PO & i \\
193.6411 & 16.324$\pm$0.039 & PO & i \\
193.6429 & 15.863$\pm$0.062 & PO & z \\
193.6448 & 15.809$\pm$0.060 & PO & z \\
193.6467 & 15.883$\pm$0.062 & PO & z \\
194.7172 & 16.582$\pm$0.044 & ZTF & g \\
194.7172 & 16.582$\pm$0.044 & ZTF & g \\
194.7554 & 16.657$\pm$0.036 & ZTF & r \\
194.7554 & 16.657$\pm$0.036 & ZTF & r \\
194.7737 & 16.651$\pm$0.041 & ZTF & r \\
194.7737 & 16.651$\pm$0.041 & ZTF & r \\
194.8146 & 16.524$\pm$0.021 & ATLAS & o \\
194.8178 & 16.510$\pm$0.026 & ATLAS & o \\
194.8243 & 16.525$\pm$0.025 & ATLAS & o \\
194.8354 & 16.513$\pm$0.026 & ATLAS & o \\
194.8413 & 16.596$\pm$0.052 & ZTF & g \\
194.8413 & 16.596$\pm$0.052 & ZTF & g \\
195.6261 & 16.688$\pm$0.045 & PO & g \\
195.6279 & 16.687$\pm$0.046 & PO & g \\
195.6298 & 16.700$\pm$0.046 & PO & g \\
195.6317 & 16.616$\pm$0.050 & PO & r \\
195.6336 & 16.548$\pm$0.049 & PO & r \\
195.6354 & 16.585$\pm$0.049 & PO & r \\
195.6374 & 16.283$\pm$0.039 & PO & i \\
195.6392 & 16.282$\pm$0.038 & PO & i \\
195.6411 & 16.264$\pm$0.038 & PO & i \\
195.6430 & 15.765$\pm$0.062 & PO & z \\
195.6448 & 15.749$\pm$0.062 & PO & z \\
195.6467 & 15.745$\pm$0.063 & PO & z \\
196.6279 & 16.626$\pm$0.043 & PO & g \\
196.6298 & 16.647$\pm$0.044 & PO & g \\
196.6316 & 16.669$\pm$0.044 & PO & g \\
196.6336 & 16.574$\pm$0.049 & PO & r \\
196.6354 & 16.590$\pm$0.049 & PO & r \\
196.6373 & 16.580$\pm$0.049 & PO & r \\
196.6392 & 16.292$\pm$0.038 & PO & i \\
196.6411 & 16.281$\pm$0.038 & PO & i \\
196.6429 & 16.259$\pm$0.038 & PO & i \\
196.6448 & 15.772$\pm$0.060 & PO & z \\
196.6467 & 15.770$\pm$0.061 & PO & z \\
196.6486 & 15.816$\pm$0.061 & PO & z \\
196.7155 & 16.517$\pm$0.047 & ZTF & g \\
196.7155 & 16.517$\pm$0.047 & ZTF & g \\
196.7343 & 16.555$\pm$0.031 & ZTF & g \\
196.7343 & 16.555$\pm$0.031 & ZTF & g \\
196.7705 & 16.540$\pm$0.031 & ZTF & r \\
196.7705 & 16.540$\pm$0.031 & ZTF & r \\
196.7858 & 16.570$\pm$0.031 & ZTF & r \\
196.7858 & 16.570$\pm$0.031 & ZTF & r \\
196.9071 & 16.410$\pm$0.024 & ATLAS & o \\
196.9340 & 16.115$\pm$0.017 & ATLAS & o \\
196.9358 & 16.451$\pm$0.029 & ATLAS & o \\
196.9390 & 16.432$\pm$0.025 & ATLAS & o \\
197.3426 & 16.554$\pm$0.022 & ATLAS & c \\
197.3453 & 16.589$\pm$0.021 & ATLAS & c \\
197.3512 & 16.558$\pm$0.019 & ATLAS & c \\
197.3611 & 16.567$\pm$0.019 & ATLAS & c \\
197.6171 & 16.646$\pm$0.044 & PO & g \\
197.6189 & 16.646$\pm$0.044 & PO & g \\
197.6208 & 16.656$\pm$0.044 & PO & g \\
197.6227 & 16.621$\pm$0.050 & PO & r \\
197.6246 & 16.584$\pm$0.049 & PO & r \\
197.6264 & 16.643$\pm$0.050 & PO & r \\
197.6284 & 16.287$\pm$0.039 & PO & i \\
197.6302 & 16.290$\pm$0.039 & PO & i \\
197.6321 & 16.306$\pm$0.040 & PO & i \\
197.6340 & 15.764$\pm$0.061 & PO & z \\
197.6358 & 15.789$\pm$0.061 & PO & z \\
197.6377 & 15.762$\pm$0.061 & PO & z \\
197.6492 & 16.510$\pm$0.051 & ZTF & g \\
197.6492 & 16.510$\pm$0.051 & ZTF & g \\
197.6506 & 16.544$\pm$0.029 & ZTF & g \\
197.6506 & 16.544$\pm$0.029 & ZTF & g \\
198.6121 & 16.722$\pm$0.046 & PO & g \\
198.6140 & 16.765$\pm$0.047 & PO & g \\
198.6158 & 16.776$\pm$0.047 & PO & g \\
198.6177 & 16.625$\pm$0.050 & PO & r \\
198.6196 & 16.651$\pm$0.050 & PO & r \\
198.6214 & 16.615$\pm$0.050 & PO & r \\
198.6234 & 16.388$\pm$0.040 & PO & i \\
198.6252 & 16.371$\pm$0.040 & PO & i \\
198.6273 & 16.390$\pm$0.041 & PO & i \\
198.6291 & 15.746$\pm$0.061 & PO & z \\
198.6310 & 15.752$\pm$0.061 & PO & z \\
198.6329 & 15.730$\pm$0.061 & PO & z \\
198.6567 & 16.561$\pm$0.064 & P60 & r \\
198.6584 & 16.529$\pm$0.062 & P60 & i \\
198.7233 & 16.718$\pm$0.045 & PO & g \\
198.7251 & 16.676$\pm$0.044 & PO & g \\
198.7270 & 16.700$\pm$0.045 & PO & g \\
198.7289 & 16.658$\pm$0.051 & PO & r \\
198.7308 & 16.673$\pm$0.051 & PO & r \\
198.7326 & 16.666$\pm$0.051 & PO & r \\
198.8420 & 16.632$\pm$0.020 & ATLAS & c \\
198.8531 & 16.629$\pm$0.019 & ATLAS & c \\
198.8578 & 16.608$\pm$0.020 & ATLAS & c \\
198.8690 & 16.607$\pm$0.020 & ATLAS & c \\
199.6017 & 16.511$\pm$0.019 & ATLAS & o \\
199.6045 & 16.551$\pm$0.019 & ATLAS & o \\
199.6109 & 16.526$\pm$0.021 & ATLAS & o \\
199.6258 & 16.501$\pm$0.016 & ATLAS & o \\
199.6487 & 16.597$\pm$0.029 & ZTF & g \\
199.6487 & 16.597$\pm$0.029 & ZTF & g \\
199.6735 & 16.621$\pm$0.041 & ZTF & r \\
199.6735 & 16.621$\pm$0.041 & ZTF & r \\
199.6745 & 16.663$\pm$0.032 & ZTF & r \\
199.6745 & 16.663$\pm$0.032 & ZTF & r \\
199.7446 & 16.605$\pm$0.034 & ZTF & g \\
199.7446 & 16.605$\pm$0.034 & ZTF & g \\
200.6612 & 16.135$\pm$0.026 & ZTF & i \\
200.6612 & 16.135$\pm$0.026 & ZTF & i \\
200.7326 & 16.673$\pm$0.040 & ZTF & r \\
200.7326 & 16.673$\pm$0.040 & ZTF & r \\
200.8926 & 16.569$\pm$0.024 & ATLAS & o \\
200.9607 & 16.558$\pm$0.026 & ATLAS & o \\
200.9866 & 16.551$\pm$0.035 & ATLAS & o \\
201.3322 & 16.625$\pm$0.021 & ATLAS & c \\
201.3354 & 16.675$\pm$0.025 & ATLAS & c \\
201.3426 & 16.597$\pm$0.026 & ATLAS & c \\
201.3526 & 16.668$\pm$0.026 & ATLAS & c \\
201.6053 & 16.845$\pm$0.049 & PO & g \\
201.6071 & 16.859$\pm$0.049 & PO & g \\
201.6090 & 16.831$\pm$0.048 & PO & g \\
201.6109 & 16.737$\pm$0.053 & PO & r \\
201.6128 & 16.711$\pm$0.052 & PO & r \\
201.6146 & 16.728$\pm$0.052 & PO & r \\
201.6166 & 16.412$\pm$0.042 & PO & i \\
201.6184 & 16.428$\pm$0.042 & PO & i \\
201.6203 & 16.398$\pm$0.041 & PO & i \\
201.6221 & 15.804$\pm$0.064 & PO & z \\
201.6240 & 15.863$\pm$0.064 & PO & z \\
201.6259 & 15.844$\pm$0.063 & PO & z \\
201.6711 & 16.700$\pm$0.049 & ZTF & r \\
201.6711 & 16.700$\pm$0.049 & ZTF & r \\
201.7133 & 16.641$\pm$0.043 & ZTF & g \\
201.7133 & 16.641$\pm$0.043 & ZTF & g \\
201.7233 & 16.802$\pm$0.047 & PO & g \\
201.7251 & 16.825$\pm$0.048 & PO & g \\
201.7270 & 16.832$\pm$0.048 & PO & g \\
201.7289 & 16.721$\pm$0.052 & PO & r \\
201.7308 & 16.668$\pm$0.051 & PO & r \\
201.7326 & 16.722$\pm$0.052 & PO & r \\
201.8214 & 16.165$\pm$0.037 & ZTF & i \\
201.8214 & 16.165$\pm$0.037 & ZTF & i \\
202.6907 & 16.711$\pm$0.033 & ZTF & r \\
202.6907 & 16.711$\pm$0.033 & ZTF & r \\
202.8783 & 16.752$\pm$0.022 & ATLAS & c \\
202.9049 & 16.700$\pm$0.021 & ATLAS & c \\
202.9184 & 16.717$\pm$0.022 & ATLAS & c \\
203.5876 & 16.643$\pm$0.020 & ATLAS & o \\
203.5908 & 16.609$\pm$0.023 & ATLAS & o \\
203.5980 & 16.580$\pm$0.020 & ATLAS & o \\
203.6064 & 16.202$\pm$0.042 & ZTF & i \\
203.6064 & 16.202$\pm$0.042 & ZTF & i \\
203.6080 & 16.612$\pm$0.023 & ATLAS & o \\
203.6925 & 16.719$\pm$0.034 & ZTF & r \\
203.6925 & 16.719$\pm$0.034 & ZTF & r \\
204.6051 & 16.851$\pm$0.048 & PO & g \\
204.6069 & 16.870$\pm$0.049 & PO & g \\
204.6088 & 16.840$\pm$0.048 & PO & g \\
204.6107 & 16.790$\pm$0.053 & PO & r \\
204.6125 & 16.806$\pm$0.054 & PO & r \\
204.6144 & 16.778$\pm$0.053 & PO & r \\
204.6163 & 16.483$\pm$0.042 & PO & i \\
204.6181 & 16.457$\pm$0.041 & PO & i \\
204.6200 & 16.473$\pm$0.042 & PO & i \\
204.6219 & 15.921$\pm$0.063 & PO & z \\
204.6237 & 15.930$\pm$0.062 & PO & z \\
204.6256 & 15.949$\pm$0.062 & PO & z \\
204.6698 & 16.748$\pm$0.028 & ZTF & g \\
204.6698 & 16.749$\pm$0.028 & ZTF & g \\
204.6902 & 16.783$\pm$0.036 & ZTF & r \\
204.6902 & 16.783$\pm$0.036 & ZTF & r \\
204.7233 & 16.882$\pm$0.049 & PO & g \\
204.7251 & 16.858$\pm$0.049 & PO & g \\
204.7270 & 16.879$\pm$0.049 & PO & g \\
204.7288 & 16.763$\pm$0.053 & PO & r \\
204.7307 & 16.735$\pm$0.052 & PO & r \\
204.7325 & 16.772$\pm$0.053 & PO & r \\
204.7344 & 16.492$\pm$0.042 & PO & i \\
204.7362 & 16.518$\pm$0.043 & PO & i \\
204.7381 & 16.519$\pm$0.043 & PO & i \\
204.7400 & 15.961$\pm$0.064 & PO & z \\
204.7419 & 15.947$\pm$0.063 & PO & z \\
204.7437 & 15.925$\pm$0.062 & PO & z \\
205.3154 & 16.787$\pm$0.044 & ATLAS & c \\
205.3195 & 16.873$\pm$0.033 & ATLAS & c \\
205.3263 & 16.786$\pm$0.039 & ATLAS & c \\
205.6053 & 16.951$\pm$0.051 & PO & g \\
205.6072 & 16.983$\pm$0.052 & PO & g \\
205.6090 & 16.899$\pm$0.050 & PO & g \\
205.6110 & 16.828$\pm$0.054 & PO & r \\
205.6128 & 16.848$\pm$0.054 & PO & r \\
205.6146 & 16.830$\pm$0.054 & PO & r \\
205.6165 & 16.626$\pm$0.045 & PO & i \\
205.6184 & 16.555$\pm$0.044 & PO & i \\
205.6203 & 16.635$\pm$0.046 & PO & i \\
205.6221 & 15.984$\pm$0.064 & PO & z \\
205.6240 & 16.013$\pm$0.064 & PO & z \\
205.6258 & 15.980$\pm$0.063 & PO & z \\
205.6492 & 16.312$\pm$0.045 & ZTF & i \\
205.6492 & 16.312$\pm$0.045 & ZTF & i \\
205.6907 & 16.778$\pm$0.049 & ZTF & g \\
205.6907 & 16.778$\pm$0.049 & ZTF & g \\
205.7233 & 16.932$\pm$0.050 & PO & g \\
205.7251 & 16.934$\pm$0.050 & PO & g \\
205.7270 & 16.902$\pm$0.049 & PO & g \\
205.7288 & 16.837$\pm$0.055 & PO & r \\
205.7307 & 16.789$\pm$0.054 & PO & r \\
205.7325 & 16.850$\pm$0.055 & PO & r \\
205.7344 & 16.551$\pm$0.045 & PO & i \\
205.7363 & 16.519$\pm$0.045 & PO & i \\
205.7381 & 16.566$\pm$0.045 & PO & i \\
205.7400 & 15.920$\pm$0.062 & PO & z \\
205.7419 & 15.922$\pm$0.063 & PO & z \\
205.7437 & 15.926$\pm$0.064 & PO & z \\
206.6845 & 16.979$\pm$0.052 & PO & g \\
206.6864 & 16.980$\pm$0.052 & PO & g \\
206.6882 & 16.972$\pm$0.051 & PO & g \\
206.6894 & 16.776$\pm$0.041 & ZTF & g \\
206.6894 & 16.776$\pm$0.041 & ZTF & g \\
206.6902 & 16.873$\pm$0.055 & PO & r \\
206.6920 & 16.879$\pm$0.056 & PO & r \\
206.6938 & 16.870$\pm$0.056 & PO & r \\
206.6958 & 16.587$\pm$0.045 & PO & i \\
206.6976 & 16.571$\pm$0.045 & PO & i \\
206.6995 & 16.658$\pm$0.047 & PO & i \\
206.7013 & 15.974$\pm$0.067 & PO & z \\
206.7050 & 15.964$\pm$0.066 & PO & z \\
206.7320 & 16.811$\pm$0.033 & ZTF & r \\
206.7320 & 16.811$\pm$0.033 & ZTF & r \\
206.7726 & 17.029$\pm$0.053 & PO & g \\
206.7745 & 17.063$\pm$0.055 & PO & g \\
206.7763 & 17.042$\pm$0.054 & PO & g \\
206.7782 & 16.971$\pm$0.059 & PO & r \\
206.7801 & 16.937$\pm$0.057 & PO & r \\
206.7819 & 16.708$\pm$0.056 & PO & r \\
206.7838 & 16.916$\pm$0.071 & PO & i \\
206.7857 & 16.992$\pm$0.066 & PO & i \\
206.7875 & 16.732$\pm$0.059 & PO & i \\
206.7894 & 15.836$\pm$0.067 & PO & z \\
206.7914 & 16.009$\pm$0.071 & PO & z \\
206.7933 & 15.951$\pm$0.071 & PO & z \\
206.8016 & 16.865$\pm$0.023 & ATLAS & c \\
206.8044 & 16.900$\pm$0.023 & ATLAS & c \\
206.8142 & 16.901$\pm$0.021 & ATLAS & c \\
206.8245 & 16.800$\pm$0.022 & ATLAS & c \\
207.5712 & 16.618$\pm$0.024 & ATLAS & o \\
207.5748 & 16.724$\pm$0.030 & ATLAS & o \\
207.5820 & 16.764$\pm$0.045 & ATLAS & o \\
207.5912 & 16.919$\pm$0.050 & PO & g \\
207.5919 & 16.992$\pm$0.401 & ATLAS & o \\
207.5931 & 16.962$\pm$0.052 & PO & g \\
207.5949 & 16.922$\pm$0.050 & PO & g \\
207.5969 & 16.841$\pm$0.055 & PO & r \\
207.5987 & 16.841$\pm$0.055 & PO & r \\
207.6005 & 16.830$\pm$0.054 & PO & r \\
207.6025 & 16.598$\pm$0.046 & PO & i \\
207.6043 & 16.589$\pm$0.045 & PO & i \\
207.6062 & 16.580$\pm$0.045 & PO & i \\
207.6080 & 15.931$\pm$0.064 & PO & z \\
207.6099 & 15.944$\pm$0.065 & PO & z \\
207.6118 & 15.932$\pm$0.064 & PO & z \\
207.6295 & 16.719$\pm$0.034 & ZTF & g \\
207.6295 & 16.719$\pm$0.034 & ZTF & g \\
207.6699 & 16.756$\pm$0.040 & ZTF & r \\
207.6699 & 16.756$\pm$0.040 & ZTF & r \\
207.6851 & 16.634$\pm$0.085 & PO & r \\
207.6888 & 16.556$\pm$0.079 & PO & r \\
207.6908 & 16.482$\pm$0.103 & PO & i \\
207.6926 & 16.251$\pm$0.063 & PO & i \\
207.6963 & 15.563$\pm$0.095 & PO & z \\
208.6680 & 16.723$\pm$0.032 & ZTF & r \\
208.6680 & 16.723$\pm$0.032 & ZTF & r \\
208.8025 & 16.563$\pm$0.023 & ATLAS & o \\
208.8056 & 16.547$\pm$0.025 & ATLAS & o \\
208.8120 & 16.502$\pm$0.020 & ATLAS & o \\
208.8218 & 16.574$\pm$0.022 & ATLAS & o \\
209.6382 & 16.614$\pm$0.025 & ATLAS & o \\
209.6736 & 16.602$\pm$0.024 & ATLAS & o \\
209.6740 & 16.589$\pm$0.023 & ATLAS & o \\
209.6745 & 16.628$\pm$0.023 & ATLAS & o \\
209.6748 & 16.725$\pm$0.031 & ZTF & r \\
209.6748 & 16.725$\pm$0.031 & ZTF & r \\
209.6749 & 16.615$\pm$0.023 & ATLAS & o \\
210.5913 & 18.249$\pm$0.116 & PO & u \\
210.5937 & 18.276$\pm$0.122 & PO & u \\
210.5961 & 18.257$\pm$0.117 & PO & u \\
210.5986 & 18.228$\pm$0.117 & PO & u \\
210.6010 & 18.639$\pm$0.153 & PO & u \\
210.6018 & 16.710$\pm$0.066 & P60 & r \\
210.6034 & 18.699$\pm$0.165 & PO & u \\
210.6035 & 16.685$\pm$0.065 & P60 & i \\
210.6059 & 16.928$\pm$0.051 & PO & g \\
210.6078 & 16.889$\pm$0.050 & PO & g \\
210.6096 & 16.859$\pm$0.049 & PO & g \\
210.6116 & 16.846$\pm$0.056 & PO & r \\
210.6134 & 16.848$\pm$0.056 & PO & r \\
210.6152 & 16.832$\pm$0.056 & PO & r \\
210.6171 & 16.443$\pm$0.044 & PO & i \\
210.6190 & 16.478$\pm$0.045 & PO & i \\
210.6209 & 16.474$\pm$0.044 & PO & i \\
210.6229 & 15.874$\pm$0.071 & PO & z \\
210.6248 & 15.820$\pm$0.068 & PO & z \\
210.6266 & 15.872$\pm$0.070 & PO & z \\
210.6717 & 16.791$\pm$0.036 & ZTF & r \\
210.6717 & 16.791$\pm$0.036 & ZTF & r \\
210.7117 & 16.662$\pm$0.035 & ZTF & g \\
210.7117 & 16.662$\pm$0.035 & ZTF & g \\
211.5654 & 16.664$\pm$0.028 & ATLAS & o \\
211.5686 & 16.650$\pm$0.028 & ATLAS & o \\
211.5758 & 16.596$\pm$0.033 & ATLAS & o \\
211.5857 & 16.714$\pm$0.026 & ATLAS & o \\
211.6855 & 16.845$\pm$0.054 & ZTF & r \\
211.6855 & 16.845$\pm$0.054 & ZTF & r \\
213.2925 & 16.697$\pm$0.031 & ATLAS & o \\
213.2965 & 16.673$\pm$0.032 & ATLAS & o \\
213.3019 & 16.671$\pm$0.032 & ATLAS & o \\
213.3120 & 16.684$\pm$0.026 & ATLAS & o \\
213.5913 & 18.506$\pm$0.128 & PO & u \\
213.5937 & 18.520$\pm$0.140 & PO & u \\
213.5961 & 18.400$\pm$0.127 & PO & u \\
213.5985 & 18.567$\pm$0.151 & PO & u \\
213.6009 & 18.396$\pm$0.118 & PO & u \\
213.6034 & 18.597$\pm$0.144 & PO & u \\
213.6059 & 17.047$\pm$0.055 & PO & g \\
213.6078 & 17.045$\pm$0.055 & PO & g \\
213.6096 & 17.051$\pm$0.056 & PO & g \\
213.6116 & 16.918$\pm$0.057 & PO & r \\
213.6134 & 16.872$\pm$0.056 & PO & r \\
213.6152 & 16.904$\pm$0.057 & PO & r \\
213.6171 & 16.591$\pm$0.046 & PO & i \\
213.6190 & 16.594$\pm$0.047 & PO & i \\
213.6209 & 16.602$\pm$0.047 & PO & i \\
213.6228 & 15.942$\pm$0.064 & PO & z \\
213.6248 & 15.909$\pm$0.064 & PO & z \\
213.6266 & 15.904$\pm$0.064 & PO & z \\
213.6681 & 16.827$\pm$0.033 & ZTF & r \\
213.6681 & 16.827$\pm$0.033 & ZTF & r \\
214.5912 & 18.309$\pm$0.154 & PO & u \\
214.5937 & 17.971$\pm$0.161 & PO & u \\
214.5961 & 18.566$\pm$0.176 & PO & u \\
214.5986 & 18.307$\pm$0.139 & PO & u \\
214.6010 & 18.520$\pm$0.166 & PO & u \\
214.6035 & 18.221$\pm$0.134 & PO & u \\
214.6060 & 16.941$\pm$0.060 & PO & g \\
214.6079 & 16.924$\pm$0.060 & PO & g \\
214.6097 & 17.036$\pm$0.064 & PO & g \\
214.6116 & 16.760$\pm$0.067 & PO & r \\
214.6135 & 16.690$\pm$0.063 & PO & r \\
214.6154 & 16.790$\pm$0.067 & PO & r \\
214.6173 & 16.811$\pm$0.104 & PO & i \\
214.6191 & 16.598$\pm$0.071 & PO & i \\
214.6210 & 16.505$\pm$0.062 & PO & i \\
214.6228 & 16.049$\pm$0.081 & PO & z \\
214.7042 & 18.025$\pm$0.160 & PO & u \\
214.7066 & 17.705$\pm$0.137 & PO & u \\
214.7090 & 17.911$\pm$0.144 & PO & u \\
214.7114 & 17.931$\pm$0.153 & PO & u \\
214.7139 & 17.985$\pm$0.157 & PO & u \\
214.7163 & 18.066$\pm$0.164 & PO & u \\
214.7189 & 17.023$\pm$0.068 & PO & g \\
214.7207 & 17.039$\pm$0.062 & PO & g \\
214.7226 & 17.075$\pm$0.062 & PO & g \\
214.7245 & 16.816$\pm$0.064 & PO & r \\
214.7263 & 16.810$\pm$0.062 & PO & r \\
214.7282 & 16.722$\pm$0.060 & PO & r \\
214.7301 & 16.384$\pm$0.064 & PO & i \\
214.7320 & 16.591$\pm$0.073 & PO & i \\
214.7338 & 16.369$\pm$0.061 & PO & i \\
214.7357 & 16.060$\pm$0.080 & PO & z \\
214.7378 & 16.082$\pm$0.086 & PO & z \\
214.7396 & 16.039$\pm$0.097 & PO & z \\
214.7522 & 16.335$\pm$0.036 & ZTF & i \\
214.7522 & 16.335$\pm$0.036 & ZTF & i \\
215.5912 & 18.498$\pm$0.213 & PO & u \\
215.5937 & 18.216$\pm$0.156 & PO & u \\
215.5961 & 18.113$\pm$0.151 & PO & u \\
215.5986 & 18.667$\pm$0.210 & PO & u \\
215.6010 & 18.552$\pm$0.175 & PO & u \\
215.6035 & 18.506$\pm$0.174 & PO & u \\
215.6060 & 16.891$\pm$0.057 & PO & g \\
215.6079 & 16.915$\pm$0.059 & PO & g \\
215.6097 & 16.839$\pm$0.057 & PO & g \\
215.6116 & 17.003$\pm$0.061 & PO & g \\
215.6134 & 16.902$\pm$0.061 & PO & g \\
215.6153 & 16.799$\pm$0.102 & PO & r \\
215.6209 & 16.803$\pm$0.086 & PO & r \\
215.6248 & 16.797$\pm$0.068 & PO & i \\
215.6266 & 16.708$\pm$0.064 & PO & i \\
215.6285 & 16.761$\pm$0.069 & PO & i \\
215.6304 & 16.774$\pm$0.072 & PO & i \\
215.6322 & 16.810$\pm$0.077 & PO & i \\
215.6341 & 16.227$\pm$0.086 & PO & z \\
215.6359 & 16.041$\pm$0.072 & PO & z \\
215.6378 & 16.185$\pm$0.077 & PO & z \\
215.6397 & 16.235$\pm$0.077 & PO & z \\
215.6415 & 16.372$\pm$0.083 & PO & z \\
215.6955 & 16.217$\pm$0.081 & PO & z \\
215.6973 & 16.054$\pm$0.076 & PO & z \\
215.6992 & 16.069$\pm$0.080 & PO & z \\
215.7010 & 16.054$\pm$0.077 & PO & z \\
215.7029 & 16.130$\pm$0.080 & PO & z \\
219.5739 & 18.268$\pm$0.162 & PO & u \\
219.5763 & 18.545$\pm$0.190 & PO & u \\
219.5788 & 18.378$\pm$0.149 & PO & u \\
219.5812 & 18.715$\pm$0.211 & PO & u \\
219.5836 & 18.677$\pm$0.185 & PO & u \\
219.5860 & 18.615$\pm$0.180 & PO & u \\
219.5885 & 16.971$\pm$0.056 & PO & g \\
219.5904 & 16.987$\pm$0.056 & PO & g \\
219.5922 & 17.052$\pm$0.058 & PO & g \\
219.5941 & 17.099$\pm$0.060 & PO & g \\
219.5960 & 16.794$\pm$0.044 & ATLAS & o \\
219.5960 & 17.111$\pm$0.063 & PO & g \\
219.5979 & 16.958$\pm$0.059 & PO & r \\
219.5996 & 16.848$\pm$0.048 & ATLAS & o \\
219.5997 & 16.921$\pm$0.058 & PO & r \\
219.6015 & 16.909$\pm$0.058 & PO & r \\
219.6034 & 16.941$\pm$0.059 & PO & r \\
219.6053 & 16.969$\pm$0.060 & PO & r \\
219.6055 & 16.843$\pm$0.054 & ATLAS & o \\
219.6181 & 16.844$\pm$0.046 & ATLAS & o \\
219.6467 & 18.283$\pm$0.149 & PO & u \\
219.6491 & 18.712$\pm$0.189 & PO & u \\
219.6540 & 18.930$\pm$0.312 & PO & u \\
219.6588 & 18.421$\pm$0.192 & PO & u \\
219.6614 & 17.033$\pm$0.059 & PO & g \\
219.6632 & 17.052$\pm$0.060 & PO & g \\
219.6650 & 17.039$\pm$0.057 & PO & g \\
219.6669 & 17.159$\pm$0.068 & PO & g \\
219.6687 & 17.125$\pm$0.062 & PO & g \\
219.6706 & 17.049$\pm$0.063 & PO & r \\
219.6724 & 16.940$\pm$0.059 & PO & r \\
219.6743 & 17.005$\pm$0.063 & PO & r \\
219.6761 & 17.021$\pm$0.060 & PO & r \\
219.6780 & 16.925$\pm$0.060 & PO & r \\
221.3134 & 16.724$\pm$0.044 & ATLAS & o \\
221.3170 & 16.663$\pm$0.044 & ATLAS & o \\
221.3242 & 16.681$\pm$0.045 & ATLAS & o \\
221.3410 & 16.668$\pm$0.040 & ATLAS & o \\
221.5790 & 18.291$\pm$0.177 & PO & u \\
221.5815 & 18.259$\pm$0.182 & PO & u \\
221.5839 & 18.299$\pm$0.158 & PO & u \\
221.5864 & 18.959$\pm$0.320 & PO & u \\
221.5914 & 16.956$\pm$0.055 & PO & g \\
221.5933 & 16.964$\pm$0.055 & PO & g \\
221.5951 & 16.929$\pm$0.055 & PO & g \\
221.5969 & 16.848$\pm$0.053 & PO & g \\
221.5988 & 16.897$\pm$0.054 & PO & g \\
221.6007 & 16.818$\pm$0.057 & PO & r \\
221.6026 & 16.855$\pm$0.058 & PO & r \\
221.6044 & 16.891$\pm$0.060 & PO & r \\
221.6063 & 16.836$\pm$0.058 & PO & r \\
221.6081 & 16.837$\pm$0.057 & PO & r \\
221.6100 & 16.595$\pm$0.046 & PO & i \\
221.6121 & 16.558$\pm$0.046 & PO & i \\
221.6139 & 16.615$\pm$0.048 & PO & i \\
221.6158 & 16.563$\pm$0.045 & PO & i \\
221.6177 & 16.590$\pm$0.046 & PO & i \\
221.6196 & 15.989$\pm$0.063 & PO & z \\
221.6214 & 15.936$\pm$0.065 & PO & z \\
221.6233 & 15.961$\pm$0.065 & PO & z \\
221.6251 & 15.923$\pm$0.064 & PO & z \\
221.6270 & 15.948$\pm$0.065 & PO & z \\
221.6467 & 18.272$\pm$0.180 & PO & u \\
221.6492 & 18.308$\pm$0.174 & PO & u \\
221.6540 & 18.423$\pm$0.206 & PO & u \\
221.6564 & 17.886$\pm$0.148 & PO & u \\
221.6588 & 18.775$\pm$0.272 & PO & u \\
221.6614 & 17.016$\pm$0.072 & PO & g \\
221.6632 & 16.935$\pm$0.055 & PO & g \\
221.6650 & 16.898$\pm$0.053 & PO & g \\
221.6669 & 16.917$\pm$0.053 & PO & g \\
221.6688 & 16.873$\pm$0.053 & PO & g \\
221.6707 & 16.868$\pm$0.057 & PO & r \\
221.6725 & 16.837$\pm$0.056 & PO & r \\
221.6744 & 16.831$\pm$0.057 & PO & r \\
221.6762 & 16.838$\pm$0.057 & PO & r \\
221.6781 & 16.838$\pm$0.057 & PO & r \\
221.6799 & 16.567$\pm$0.046 & PO & i \\
221.6818 & 16.492$\pm$0.045 & PO & i \\
221.6837 & 16.545$\pm$0.045 & PO & i \\
221.6855 & 16.583$\pm$0.046 & PO & i \\
221.6876 & 16.517$\pm$0.044 & PO & i \\
221.6894 & 15.966$\pm$0.064 & PO & z \\
221.6913 & 15.965$\pm$0.065 & PO & z \\
221.6931 & 15.938$\pm$0.064 & PO & z \\
221.6950 & 15.984$\pm$0.064 & PO & z \\
221.6969 & 15.912$\pm$0.062 & PO & z \\
222.5740 & 18.253$\pm$0.156 & PO & u \\
222.5764 & 18.147$\pm$0.141 & PO & u \\
222.5789 & 18.625$\pm$0.198 & PO & u \\
222.5814 & 18.291$\pm$0.139 & PO & u \\
222.5838 & 18.297$\pm$0.134 & PO & u \\
222.5863 & 18.703$\pm$0.184 & PO & u \\
222.5888 & 16.935$\pm$0.051 & PO & g \\
222.5907 & 16.884$\pm$0.051 & PO & g \\
222.5925 & 16.957$\pm$0.052 & PO & g \\
222.5944 & 17.007$\pm$0.055 & PO & g \\
222.5962 & 16.947$\pm$0.052 & PO & g \\
222.5981 & 16.931$\pm$0.057 & PO & r \\
222.6000 & 16.918$\pm$0.057 & PO & r \\
222.6018 & 16.928$\pm$0.057 & PO & r \\
222.6037 & 16.922$\pm$0.057 & PO & r \\
222.6055 & 16.917$\pm$0.057 & PO & r \\
222.6075 & 16.580$\pm$0.045 & PO & i \\
222.6095 & 16.568$\pm$0.044 & PO & i \\
222.6113 & 16.567$\pm$0.044 & PO & i \\
222.6132 & 16.574$\pm$0.044 & PO & i \\
222.6151 & 16.596$\pm$0.045 & PO & i \\
222.6170 & 15.999$\pm$0.064 & PO & z \\
222.6188 & 15.951$\pm$0.063 & PO & z \\
222.6206 & 15.975$\pm$0.064 & PO & z \\
222.6225 & 15.955$\pm$0.063 & PO & z \\
222.6244 & 15.974$\pm$0.063 & PO & z \\
222.6467 & 18.189$\pm$0.155 & PO & u \\
222.6491 & 18.278$\pm$0.147 & PO & u \\
222.6516 & 18.580$\pm$0.198 & PO & u \\
222.6523 & 16.788$\pm$0.036 & ZTF & g \\
222.6523 & 16.788$\pm$0.036 & ZTF & g \\
222.6528 & 16.810$\pm$0.042 & ZTF & g \\
222.6528 & 16.810$\pm$0.042 & ZTF & g \\
222.6540 & 18.501$\pm$0.173 & PO & u \\
222.6564 & 18.271$\pm$0.165 & PO & u \\
222.6588 & 18.265$\pm$0.153 & PO & u \\
222.6613 & 16.955$\pm$0.054 & PO & g \\
222.6632 & 17.001$\pm$0.056 & PO & g \\
222.6651 & 16.928$\pm$0.052 & PO & g \\
222.6669 & 16.957$\pm$0.053 & PO & g \\
222.6688 & 17.052$\pm$0.057 & PO & g \\
222.6707 & 16.916$\pm$0.058 & PO & r \\
222.6726 & 16.967$\pm$0.059 & PO & r \\
222.6745 & 16.903$\pm$0.057 & PO & r \\
222.6763 & 16.916$\pm$0.057 & PO & r \\
222.6782 & 16.954$\pm$0.059 & PO & r \\
222.6801 & 16.659$\pm$0.048 & PO & i \\
222.6820 & 16.602$\pm$0.046 & PO & i \\
222.6838 & 16.609$\pm$0.047 & PO & i \\
222.6859 & 16.595$\pm$0.047 & PO & i \\
222.6873 & 16.872$\pm$0.041 & ZTF & r \\
222.6873 & 16.872$\pm$0.041 & ZTF & r \\
222.6877 & 16.571$\pm$0.046 & PO & i \\
222.6878 & 16.877$\pm$0.036 & ZTF & r \\
222.6878 & 16.877$\pm$0.036 & ZTF & r \\
222.6896 & 15.976$\pm$0.066 & PO & z \\
222.6915 & 15.995$\pm$0.066 & PO & z \\
222.6933 & 15.999$\pm$0.065 & PO & z \\
222.6952 & 15.955$\pm$0.067 & PO & z \\
222.6970 & 15.989$\pm$0.067 & PO & z \\
223.5676 & 16.810$\pm$0.109 & ATLAS & o \\
223.5712 & 16.751$\pm$0.035 & ATLAS & o \\
223.5770 & 16.770$\pm$0.029 & ATLAS & o \\
223.5906 & 16.725$\pm$0.133 & ATLAS & o \\
223.6468 & 16.983$\pm$0.054 & PO & g \\
223.6486 & 16.953$\pm$0.053 & PO & g \\
223.6505 & 16.947$\pm$0.053 & PO & g \\
223.6524 & 16.927$\pm$0.052 & PO & g \\
223.6543 & 16.903$\pm$0.057 & PO & r \\
223.6561 & 16.881$\pm$0.057 & PO & r \\
223.6580 & 16.850$\pm$0.057 & PO & r \\
223.6599 & 16.929$\pm$0.060 & PO & r \\
223.6617 & 16.630$\pm$0.050 & PO & i \\
223.6636 & 16.622$\pm$0.054 & PO & i \\
223.6655 & 16.642$\pm$0.059 & PO & i \\
223.6673 & 16.619$\pm$0.052 & PO & i \\
223.6693 & 15.921$\pm$0.069 & PO & z \\
223.6711 & 16.045$\pm$0.074 & PO & z \\
223.6729 & 15.952$\pm$0.067 & PO & z \\
223.6749 & 15.970$\pm$0.067 & PO & z \\
223.9858 & 16.166$\pm$0.005 & Mephisto & i \\
223.9858 & 18.583$\pm$0.036 & Mephisto & u \\
223.9911 & 16.144$\pm$0.005 & Mephisto & i \\
223.9911 & 18.572$\pm$0.036 & Mephisto & u \\
223.9963 & 18.547$\pm$0.035 & Mephisto & u \\
223.9963 & 16.170$\pm$0.005 & Mephisto & i \\
223.9999 & 16.145$\pm$0.006 & Mephisto & i \\
223.9999 & 18.553$\pm$0.038 & Mephisto & u \\
224.0011 & 16.081$\pm$0.007 & Mephisto & i \\
224.0011 & 18.479$\pm$0.035 & Mephisto & u \\
224.0031 & 17.957$\pm$0.030 & Mephisto & v \\
224.0031 & 16.419$\pm$0.019 & Mephisto & z \\
224.0057 & 16.455$\pm$0.019 & Mephisto & z \\
224.0057 & 17.935$\pm$0.029 & Mephisto & v \\
224.0082 & 16.418$\pm$0.019 & Mephisto & z \\
224.0083 & 17.904$\pm$0.028 & Mephisto & v \\
224.0158 & 16.459$\pm$0.021 & Mephisto & z \\
224.0158 & 17.803$\pm$0.027 & Mephisto & v \\
224.0182 & 16.500$\pm$0.022 & Mephisto & z \\
224.0182 & 17.875$\pm$0.029 & Mephisto & v \\
224.0196 & 16.473$\pm$0.021 & Mephisto & z \\
224.0196 & 17.851$\pm$0.029 & Mephisto & v \\
224.0204 & 16.471$\pm$0.021 & Mephisto & z \\
224.0204 & 17.819$\pm$0.028 & Mephisto & v \\
224.0223 & 16.503$\pm$0.022 & Mephisto & z \\
224.0223 & 17.892$\pm$0.030 & Mephisto & v \\
224.0241 & 16.495$\pm$0.022 & Mephisto & z \\
224.0242 & 17.886$\pm$0.030 & Mephisto & v \\
224.0285 & 17.827$\pm$0.028 & Mephisto & v \\
224.0285 & 16.528$\pm$0.022 & Mephisto & z \\
224.0296 & 17.897$\pm$0.030 & Mephisto & v \\
224.0296 & 16.540$\pm$0.022 & Mephisto & z \\
224.6424 & 16.883$\pm$0.071 & P60 & r \\
224.6441 & 16.682$\pm$0.066 & P60 & i \\
225.5634 & 18.549$\pm$0.140 & PO & u \\
225.5658 & 18.330$\pm$0.113 & PO & u \\
225.5683 & 18.370$\pm$0.112 & PO & u \\
225.5707 & 18.711$\pm$0.149 & PO & u \\
225.5731 & 18.463$\pm$0.123 & PO & u \\
225.5755 & 18.514$\pm$0.125 & PO & u \\
225.5781 & 17.094$\pm$0.055 & PO & g \\
225.5800 & 17.174$\pm$0.057 & PO & g \\
225.5818 & 17.087$\pm$0.054 & PO & g \\
225.5837 & 17.068$\pm$0.054 & PO & g \\
225.5855 & 17.079$\pm$0.054 & PO & g \\
225.5875 & 16.997$\pm$0.058 & PO & r \\
225.5893 & 17.041$\pm$0.058 & PO & r \\
225.5911 & 16.991$\pm$0.057 & PO & r \\
225.5930 & 16.968$\pm$0.057 & PO & r \\
225.5948 & 16.982$\pm$0.057 & PO & r \\
225.5968 & 16.711$\pm$0.049 & PO & i \\
225.5986 & 16.717$\pm$0.047 & PO & i \\
225.6005 & 16.767$\pm$0.049 & PO & i \\
225.6023 & 16.778$\pm$0.049 & PO & i \\
225.6043 & 16.719$\pm$0.048 & PO & i \\
225.6061 & 16.061$\pm$0.076 & PO & z \\
225.6080 & 16.027$\pm$0.067 & PO & z \\
225.6099 & 15.993$\pm$0.069 & PO & z \\
225.6117 & 16.047$\pm$0.069 & PO & z \\
225.6136 & 16.050$\pm$0.070 & PO & z \\
225.6404 & 17.096$\pm$0.055 & PO & g \\
225.6423 & 17.111$\pm$0.055 & PO & g \\
225.6441 & 17.106$\pm$0.055 & PO & g \\
225.6460 & 17.098$\pm$0.056 & PO & g \\
225.6478 & 17.099$\pm$0.055 & PO & g \\
225.6497 & 17.002$\pm$0.057 & PO & r \\
225.6516 & 17.002$\pm$0.058 & PO & r \\
225.6534 & 17.096$\pm$0.062 & PO & r \\
225.6553 & 17.070$\pm$0.062 & PO & r \\
225.6572 & 17.112$\pm$0.062 & PO & r \\
225.6590 & 16.797$\pm$0.049 & PO & i \\
225.6609 & 16.712$\pm$0.049 & PO & i \\
225.6628 & 16.691$\pm$0.048 & PO & i \\
225.6646 & 16.730$\pm$0.048 & PO & i \\
225.6666 & 16.746$\pm$0.049 & PO & i \\
225.6685 & 16.245$\pm$0.069 & PO & z \\
225.6704 & 16.145$\pm$0.067 & PO & z \\
225.6722 & 16.164$\pm$0.069 & PO & z \\
225.6740 & 16.158$\pm$0.069 & PO & z \\
225.6759 & 16.126$\pm$0.068 & PO & z \\
226.0153 & 18.649$\pm$0.038 & Mephisto & u \\
226.0153 & 16.904$\pm$0.032 & Mephisto & z \\
226.0187 & 18.722$\pm$0.042 & Mephisto & u \\
226.0187 & 16.613$\pm$0.022 & Mephisto & z \\
226.0212 & 18.733$\pm$0.042 & Mephisto & u \\
226.0212 & 16.612$\pm$0.022 & Mephisto & z \\
226.0243 & 17.939$\pm$0.029 & Mephisto & v \\
226.0243 & 16.338$\pm$0.005 & Mephisto & i \\
226.0267 & 17.925$\pm$0.029 & Mephisto & v \\
226.0267 & 16.271$\pm$0.005 & Mephisto & i \\
226.0291 & 17.925$\pm$0.029 & Mephisto & v \\
226.0291 & 16.261$\pm$0.005 & Mephisto & i \\
227.0545 & 17.997$\pm$0.031 & Mephisto & v \\
227.5653 & 16.989$\pm$0.025 & ATLAS & c \\
227.5689 & 17.031$\pm$0.028 & ATLAS & c \\
227.5698 & 18.436$\pm$0.116 & PO & u \\
227.5722 & 18.601$\pm$0.124 & PO & u \\
227.5740 & 17.037$\pm$0.029 & ATLAS & c \\
227.5747 & 18.466$\pm$0.112 & PO & u \\
227.5771 & 18.481$\pm$0.120 & PO & u \\
227.5796 & 18.349$\pm$0.106 & PO & u \\
227.5820 & 18.466$\pm$0.121 & PO & u \\
227.5846 & 17.219$\pm$0.057 & PO & g \\
227.5860 & 16.977$\pm$0.139 & ATLAS & c \\
227.5865 & 17.084$\pm$0.053 & PO & g \\
227.5883 & 17.063$\pm$0.053 & PO & g \\
227.5901 & 17.092$\pm$0.054 & PO & g \\
227.5920 & 17.062$\pm$0.053 & PO & g \\
227.5939 & 17.005$\pm$0.057 & PO & r \\
227.5958 & 16.999$\pm$0.057 & PO & r \\
227.5976 & 17.027$\pm$0.057 & PO & r \\
227.5995 & 17.036$\pm$0.058 & PO & r \\
227.6015 & 17.040$\pm$0.058 & PO & r \\
227.6033 & 16.821$\pm$0.050 & PO & i \\
227.6052 & 16.788$\pm$0.048 & PO & i \\
227.6071 & 16.740$\pm$0.047 & PO & i \\
227.6089 & 16.770$\pm$0.048 & PO & i \\
227.6108 & 16.738$\pm$0.048 & PO & i \\
227.6127 & 16.121$\pm$0.064 & PO & z \\
227.6145 & 16.019$\pm$0.064 & PO & z \\
227.6164 & 16.025$\pm$0.065 & PO & z \\
227.6183 & 16.064$\pm$0.065 & PO & z \\
227.6202 & 16.095$\pm$0.067 & PO & z \\
227.9747 & 17.930$\pm$0.029 & Mephisto & v \\
227.9775 & 18.089$\pm$0.034 & Mephisto & v \\
227.9799 & 18.116$\pm$0.035 & Mephisto & v \\
227.9833 & 19.015$\pm$0.055 & Mephisto & u \\
227.9946 & 18.830$\pm$0.046 & Mephisto & u \\
227.9958 & 18.890$\pm$0.048 & Mephisto & u \\
228.0002 & 18.831$\pm$0.046 & Mephisto & u \\
228.0103 & 18.822$\pm$0.046 & Mephisto & u \\
228.6095 & 18.597$\pm$0.133 & PO & u \\
228.6119 & 18.523$\pm$0.123 & PO & u \\
228.6144 & 18.563$\pm$0.135 & PO & u \\
228.6168 & 18.522$\pm$0.131 & PO & u \\
228.6193 & 18.824$\pm$0.152 & PO & u \\
228.6217 & 18.474$\pm$0.123 & PO & u \\
228.6243 & 17.143$\pm$0.055 & PO & g \\
228.6261 & 17.177$\pm$0.056 & PO & g \\
228.6280 & 17.225$\pm$0.058 & PO & g \\
228.6298 & 17.156$\pm$0.056 & PO & g \\
228.6317 & 17.152$\pm$0.056 & PO & g \\
228.6336 & 17.068$\pm$0.058 & PO & r \\
228.6348 & 16.964$\pm$0.036 & ZTF & g \\
228.6348 & 16.964$\pm$0.036 & ZTF & g \\
228.6355 & 17.056$\pm$0.058 & PO & r \\
228.6357 & 16.981$\pm$0.045 & ZTF & g \\
228.6357 & 16.981$\pm$0.045 & ZTF & g \\
228.6373 & 17.089$\pm$0.059 & PO & r \\
228.6393 & 17.096$\pm$0.059 & PO & r \\
228.6411 & 17.081$\pm$0.059 & PO & r \\
228.6430 & 16.802$\pm$0.049 & PO & i \\
228.6449 & 16.768$\pm$0.048 & PO & i \\
228.6468 & 16.835$\pm$0.049 & PO & i \\
228.6486 & 16.869$\pm$0.050 & PO & i \\
228.6492 & 17.039$\pm$0.035 & ZTF & r \\
228.6492 & 17.040$\pm$0.035 & ZTF & r \\
228.6505 & 16.785$\pm$0.048 & PO & i \\
228.6524 & 16.131$\pm$0.064 & PO & z \\
228.6539 & 17.023$\pm$0.033 & ZTF & r \\
228.6539 & 17.023$\pm$0.033 & ZTF & r \\
228.6543 & 16.122$\pm$0.064 & PO & z \\
228.6562 & 16.140$\pm$0.064 & PO & z \\
228.6580 & 16.235$\pm$0.064 & PO & z \\
228.6599 & 16.206$\pm$0.064 & PO & z \\
228.6622 & 18.833$\pm$0.161 & PO & u \\
228.6646 & 19.413$\pm$0.215 & PO & u \\
228.6670 & 19.350$\pm$0.211 & PO & u \\
228.6694 & 19.397$\pm$0.220 & PO & u \\
228.6720 & 18.817$\pm$0.148 & PO & u \\
228.6744 & 19.052$\pm$0.181 & PO & u \\
228.6770 & 17.174$\pm$0.057 & PO & g \\
228.6789 & 17.153$\pm$0.056 & PO & g \\
228.6807 & 17.088$\pm$0.054 & PO & g \\
228.6825 & 17.112$\pm$0.055 & PO & g \\
228.6844 & 17.211$\pm$0.058 & PO & g \\
228.6863 & 17.051$\pm$0.058 & PO & r \\
228.6881 & 17.048$\pm$0.059 & PO & r \\
228.6900 & 17.084$\pm$0.060 & PO & r \\
228.6919 & 17.031$\pm$0.058 & PO & r \\
228.6937 & 17.033$\pm$0.058 & PO & r \\
228.6956 & 16.796$\pm$0.049 & PO & i \\
228.6975 & 16.843$\pm$0.050 & PO & i \\
228.6994 & 16.800$\pm$0.049 & PO & i \\
228.7012 & 16.817$\pm$0.049 & PO & i \\
228.7031 & 16.786$\pm$0.049 & PO & i \\
228.7050 & 16.180$\pm$0.064 & PO & z \\
228.7069 & 16.139$\pm$0.065 & PO & z \\
228.7088 & 16.136$\pm$0.065 & PO & z \\
228.7106 & 16.125$\pm$0.065 & PO & z \\
228.7125 & 16.140$\pm$0.065 & PO & z \\
228.7701 & 17.016$\pm$0.026 & ATLAS & c \\
228.7742 & 16.991$\pm$0.029 & ATLAS & c \\
228.7875 & 17.047$\pm$0.029 & ATLAS & c \\
228.7947 & 17.058$\pm$0.028 & ATLAS & c \\
228.9830 & 16.647$\pm$0.023 & Mephisto & z \\
228.9830 & 18.953$\pm$0.052 & Mephisto & u \\
228.9854 & 18.893$\pm$0.049 & Mephisto & u \\
228.9854 & 16.669$\pm$0.023 & Mephisto & z \\
228.9878 & 18.856$\pm$0.047 & Mephisto & u \\
228.9878 & 16.632$\pm$0.023 & Mephisto & z \\
228.9919 & 18.045$\pm$0.032 & Mephisto & v \\
228.9919 & 16.304$\pm$0.005 & Mephisto & i \\
228.9956 & 18.047$\pm$0.032 & Mephisto & v \\
228.9956 & 16.284$\pm$0.005 & Mephisto & i \\
228.9979 & 18.023$\pm$0.031 & Mephisto & v \\
228.9979 & 16.279$\pm$0.005 & Mephisto & i \\
229.5637 & 18.386$\pm$0.116 & PO & u \\
229.5686 & 18.528$\pm$0.132 & PO & u \\
229.5736 & 18.594$\pm$0.136 & PO & u \\
229.5760 & 18.497$\pm$0.122 & PO & u \\
229.5786 & 17.236$\pm$0.058 & PO & g \\
229.5805 & 17.187$\pm$0.057 & PO & g \\
229.5823 & 17.166$\pm$0.056 & PO & g \\
229.5842 & 17.215$\pm$0.058 & PO & g \\
229.5860 & 17.151$\pm$0.056 & PO & g \\
229.5879 & 17.072$\pm$0.059 & PO & r \\
229.5898 & 17.057$\pm$0.059 & PO & r \\
229.5916 & 17.085$\pm$0.060 & PO & r \\
229.5935 & 17.081$\pm$0.060 & PO & r \\
229.5953 & 17.040$\pm$0.059 & PO & r \\
229.5973 & 16.843$\pm$0.051 & PO & i \\
229.5991 & 16.912$\pm$0.052 & PO & i \\
229.6010 & 16.855$\pm$0.051 & PO & i \\
229.6029 & 16.900$\pm$0.052 & PO & i \\
229.6048 & 16.767$\pm$0.048 & PO & i \\
229.6067 & 16.135$\pm$0.065 & PO & z \\
229.6086 & 16.137$\pm$0.066 & PO & z \\
229.6104 & 16.110$\pm$0.064 & PO & z \\
229.6122 & 16.102$\pm$0.065 & PO & z \\
229.6141 & 16.089$\pm$0.064 & PO & z \\
229.6258 & 18.887$\pm$0.158 & PO & u \\
229.6282 & 19.092$\pm$0.212 & PO & u \\
229.6355 & 18.819$\pm$0.153 & PO & u \\
229.6379 & 18.765$\pm$0.143 & PO & u \\
229.6404 & 17.123$\pm$0.055 & PO & g \\
229.6423 & 17.216$\pm$0.058 & PO & g \\
229.6441 & 17.166$\pm$0.056 & PO & g \\
229.6460 & 17.199$\pm$0.058 & PO & g \\
229.6479 & 17.187$\pm$0.057 & PO & g \\
229.6498 & 17.056$\pm$0.058 & PO & r \\
229.6516 & 17.064$\pm$0.059 & PO & r \\
229.6535 & 17.106$\pm$0.060 & PO & r \\
229.6554 & 17.058$\pm$0.059 & PO & r \\
229.6572 & 17.129$\pm$0.061 & PO & r \\
229.6592 & 16.838$\pm$0.051 & PO & i \\
229.6610 & 16.834$\pm$0.051 & PO & i \\
229.6630 & 16.778$\pm$0.049 & PO & i \\
229.6648 & 16.740$\pm$0.048 & PO & i \\
229.6667 & 16.765$\pm$0.048 & PO & i \\
229.6686 & 16.099$\pm$0.065 & PO & z \\
229.6705 & 16.131$\pm$0.065 & PO & z \\
229.6724 & 16.118$\pm$0.065 & PO & z \\
229.6742 & 16.042$\pm$0.065 & PO & z \\
229.6761 & 16.065$\pm$0.065 & PO & z \\
230.6063 & 17.044$\pm$0.040 & ZTF & r \\
230.6063 & 17.044$\pm$0.040 & ZTF & r \\
230.6073 & 17.080$\pm$0.049 & ZTF & r \\
230.6073 & 17.080$\pm$0.049 & ZTF & r \\
230.6403 & 17.185$\pm$0.057 & PO & g \\
230.6422 & 17.160$\pm$0.056 & PO & g \\
230.6440 & 17.170$\pm$0.056 & PO & g \\
230.6459 & 17.204$\pm$0.057 & PO & g \\
230.6477 & 17.190$\pm$0.057 & PO & g \\
230.6496 & 17.127$\pm$0.060 & PO & r \\
230.6515 & 17.131$\pm$0.060 & PO & r \\
230.6533 & 17.121$\pm$0.060 & PO & r \\
230.6552 & 17.170$\pm$0.062 & PO & r \\
230.6570 & 17.135$\pm$0.060 & PO & r \\
230.6590 & 16.831$\pm$0.049 & PO & i \\
230.6608 & 16.875$\pm$0.051 & PO & i \\
230.6627 & 16.846$\pm$0.050 & PO & i \\
230.6645 & 16.807$\pm$0.048 & PO & i \\
230.6664 & 16.821$\pm$0.049 & PO & i \\
230.6682 & 16.200$\pm$0.065 & PO & z \\
230.6701 & 16.128$\pm$0.066 & PO & z \\
230.6720 & 16.138$\pm$0.065 & PO & z \\
230.6738 & 16.174$\pm$0.065 & PO & z \\
230.6757 & 16.144$\pm$0.065 & PO & z \\
230.6901 & 17.044$\pm$0.047 & ZTF & g \\
230.6901 & 17.044$\pm$0.047 & ZTF & g \\
230.7122 & 17.043$\pm$0.039 & ZTF & g \\
230.7122 & 17.043$\pm$0.039 & ZTF & g \\
231.5376 & 17.112$\pm$0.039 & ATLAS & c \\
231.5408 & 17.108$\pm$0.038 & ATLAS & c \\
231.5462 & 17.072$\pm$0.037 & ATLAS & c \\
231.5531 & 18.781$\pm$0.152 & PO & u \\
231.5555 & 18.802$\pm$0.154 & PO & u \\
231.5580 & 18.900$\pm$0.158 & PO & u \\
231.5604 & 18.657$\pm$0.134 & PO & u \\
231.5611 & 17.016$\pm$0.027 & ATLAS & c \\
231.5629 & 18.772$\pm$0.137 & PO & u \\
231.5653 & 18.672$\pm$0.125 & PO & u \\
231.5679 & 17.271$\pm$0.059 & PO & g \\
231.5698 & 17.242$\pm$0.059 & PO & g \\
231.5716 & 17.239$\pm$0.059 & PO & g \\
231.5735 & 17.251$\pm$0.059 & PO & g \\
231.5753 & 17.196$\pm$0.057 & PO & g \\
231.5773 & 17.164$\pm$0.063 & PO & r \\
231.5791 & 17.144$\pm$0.061 & PO & r \\
231.5810 & 17.100$\pm$0.061 & PO & r \\
231.5829 & 17.190$\pm$0.064 & PO & r \\
231.5847 & 17.102$\pm$0.061 & PO & r \\
231.5868 & 16.868$\pm$0.051 & PO & i \\
231.5886 & 16.868$\pm$0.053 & PO & i \\
231.5905 & 16.838$\pm$0.052 & PO & i \\
231.5923 & 16.868$\pm$0.053 & PO & i \\
231.5942 & 16.847$\pm$0.051 & PO & i \\
231.5961 & 16.249$\pm$0.067 & PO & z \\
231.5980 & 16.235$\pm$0.070 & PO & z \\
231.5998 & 16.135$\pm$0.071 & PO & z \\
231.6016 & 16.286$\pm$0.080 & PO & z \\
231.6035 & 16.203$\pm$0.072 & PO & z \\
232.6053 & 18.634$\pm$0.126 & PO & u \\
232.6078 & 18.498$\pm$0.110 & PO & u \\
232.6102 & 18.624$\pm$0.126 & PO & u \\
232.6126 & 18.547$\pm$0.123 & PO & u \\
232.6150 & 18.612$\pm$0.123 & PO & u \\
232.6175 & 18.611$\pm$0.122 & PO & u \\
232.6200 & 17.104$\pm$0.055 & PO & g \\
232.6224 & 17.091$\pm$0.054 & PO & g \\
232.6248 & 17.089$\pm$0.054 & PO & g \\
232.6273 & 17.147$\pm$0.056 & PO & g \\
232.6297 & 17.209$\pm$0.058 & PO & g \\
232.6321 & 17.039$\pm$0.060 & PO & r \\
232.6346 & 17.077$\pm$0.060 & PO & r \\
232.6370 & 17.066$\pm$0.059 & PO & r \\
232.6394 & 17.115$\pm$0.061 & PO & r \\
232.6419 & 16.792$\pm$0.049 & PO & i \\
232.6444 & 16.806$\pm$0.050 & PO & i \\
232.6470 & 16.786$\pm$0.050 & PO & i \\
232.6494 & 16.763$\pm$0.049 & PO & i \\
232.6519 & 16.146$\pm$0.067 & PO & z \\
232.6543 & 16.099$\pm$0.065 & PO & z \\
232.6568 & 16.067$\pm$0.065 & PO & z \\
232.6592 & 16.057$\pm$0.064 & PO & z \\
233.5426 & 18.422$\pm$0.129 & PO & u \\
233.5450 & 18.515$\pm$0.122 & PO & u \\
233.5475 & 18.355$\pm$0.111 & PO & u \\
233.5524 & 18.285$\pm$0.103 & PO & u \\
233.5548 & 18.429$\pm$0.118 & PO & u \\
233.5574 & 17.077$\pm$0.054 & PO & g \\
233.5598 & 17.075$\pm$0.054 & PO & g \\
233.5623 & 17.135$\pm$0.056 & PO & g \\
233.5648 & 17.105$\pm$0.055 & PO & g \\
233.5673 & 17.131$\pm$0.056 & PO & g \\
233.5697 & 16.984$\pm$0.057 & PO & r \\
233.5721 & 17.001$\pm$0.058 & PO & r \\
233.5746 & 17.010$\pm$0.058 & PO & r \\
233.5772 & 17.022$\pm$0.058 & PO & r \\
233.5796 & 16.682$\pm$0.046 & PO & i \\
233.5821 & 16.585$\pm$0.044 & PO & i \\
233.5845 & 16.587$\pm$0.044 & PO & i \\
233.5869 & 16.699$\pm$0.047 & PO & i \\
233.5894 & 15.995$\pm$0.066 & PO & z \\
233.5919 & 15.994$\pm$0.067 & PO & z \\
233.5943 & 16.010$\pm$0.064 & PO & z \\
233.5968 & 15.940$\pm$0.065 & PO & z \\
233.6219 & 16.910$\pm$0.072 & P60 & r \\
233.6235 & 16.953$\pm$0.072 & P60 & i \\
233.6909 & 16.935$\pm$0.047 & ZTF & g \\
233.6909 & 16.935$\pm$0.047 & ZTF & g \\
233.7132 & 16.417$\pm$0.049 & ZTF & i \\
234.6827 & 16.901$\pm$0.038 & ZTF & g \\
235.6174 & 18.290$\pm$0.124 & PO & u \\
235.6199 & 18.701$\pm$0.200 & PO & u \\
235.6247 & 18.664$\pm$0.143 & PO & u \\
235.6271 & 18.434$\pm$0.128 & PO & u \\
235.6296 & 18.779$\pm$0.174 & PO & u \\
235.6321 & 17.277$\pm$0.060 & PO & g \\
235.6345 & 17.270$\pm$0.060 & PO & g \\
235.6370 & 17.401$\pm$0.064 & PO & g \\
235.6395 & 17.358$\pm$0.063 & PO & g \\
235.6419 & 17.345$\pm$0.062 & PO & g \\
235.6443 & 17.090$\pm$0.061 & PO & r \\
235.6468 & 17.227$\pm$0.065 & PO & r \\
235.6492 & 17.215$\pm$0.064 & PO & r \\
235.6517 & 17.252$\pm$0.066 & PO & r \\
235.6541 & 16.805$\pm$0.051 & PO & i \\
235.6567 & 16.803$\pm$0.050 & PO & i \\
235.6591 & 16.757$\pm$0.049 & PO & i \\
235.6616 & 16.771$\pm$0.049 & PO & i \\
235.6640 & 15.992$\pm$0.064 & PO & z \\
235.6665 & 16.151$\pm$0.068 & PO & z \\
235.6689 & 16.042$\pm$0.064 & PO & z \\
235.6713 & 16.053$\pm$0.066 & PO & z \\
235.6876 & 16.905$\pm$0.036 & ZTF & g \\
235.6876 & 16.905$\pm$0.036 & ZTF & g \\
236.6284 & 17.003$\pm$0.054 & ZTF & r \\
236.6284 & 17.003$\pm$0.054 & ZTF & r \\
236.6308 & 18.526$\pm$0.134 & PO & u \\
236.6332 & 18.881$\pm$0.172 & PO & u \\
236.6356 & 18.658$\pm$0.141 & PO & u \\
236.6381 & 18.709$\pm$0.145 & PO & u \\
236.6405 & 18.896$\pm$0.154 & PO & u \\
236.6430 & 18.646$\pm$0.143 & PO & u \\
236.6455 & 17.156$\pm$0.056 & PO & g \\
236.6479 & 17.145$\pm$0.056 & PO & g \\
236.6503 & 17.163$\pm$0.056 & PO & g \\
236.6528 & 17.188$\pm$0.057 & PO & g \\
236.6553 & 17.165$\pm$0.056 & PO & g \\
236.6577 & 17.114$\pm$0.060 & PO & r \\
236.6602 & 17.122$\pm$0.060 & PO & r \\
236.6626 & 17.115$\pm$0.060 & PO & r \\
236.6650 & 17.133$\pm$0.061 & PO & r \\
236.6677 & 16.790$\pm$0.048 & PO & i \\
236.6701 & 16.751$\pm$0.047 & PO & i \\
236.6725 & 16.721$\pm$0.047 & PO & i \\
236.6750 & 16.743$\pm$0.049 & PO & i \\
236.6774 & 16.047$\pm$0.064 & PO & z \\
236.6799 & 16.019$\pm$0.065 & PO & z \\
236.6823 & 16.012$\pm$0.064 & PO & z \\
236.6847 & 16.105$\pm$0.065 & PO & z \\
237.6600 & 18.584$\pm$0.123 & PO & u \\
237.6625 & 18.383$\pm$0.111 & PO & u \\
237.6649 & 18.839$\pm$0.142 & PO & u \\
237.6722 & 18.688$\pm$0.136 & PO & u \\
237.6746 & 17.049$\pm$0.047 & ZTF & r \\
237.6746 & 17.049$\pm$0.047 & ZTF & r \\
237.6748 & 17.275$\pm$0.059 & PO & g \\
237.6772 & 17.269$\pm$0.059 & PO & g \\
237.6797 & 17.253$\pm$0.059 & PO & g \\
237.6821 & 17.291$\pm$0.060 & PO & g \\
237.6845 & 17.276$\pm$0.060 & PO & g \\
237.6872 & 17.163$\pm$0.062 & PO & r \\
237.6896 & 17.063$\pm$0.059 & PO & r \\
237.6920 & 17.166$\pm$0.062 & PO & r \\
237.6945 & 17.181$\pm$0.062 & PO & r \\
237.6969 & 16.772$\pm$0.049 & PO & i \\
237.6993 & 16.794$\pm$0.050 & PO & i \\
237.7018 & 16.869$\pm$0.053 & PO & i \\
237.7042 & 16.843$\pm$0.052 & PO & i \\
237.7068 & 16.116$\pm$0.074 & PO & z \\
237.7093 & 15.935$\pm$0.069 & PO & z \\
237.7117 & 16.111$\pm$0.071 & PO & z \\
237.7142 & 15.838$\pm$0.067 & PO & z \\
238.6188 & 18.444$\pm$0.114 & PO & u \\
238.6212 & 18.504$\pm$0.121 & PO & u \\
238.6237 & 18.582$\pm$0.124 & PO & u \\
238.6261 & 18.620$\pm$0.130 & PO & u \\
238.6285 & 18.589$\pm$0.127 & PO & u \\
238.6310 & 18.944$\pm$0.158 & PO & u \\
238.6335 & 17.350$\pm$0.061 & PO & g \\
238.6359 & 17.263$\pm$0.059 & PO & g \\
238.6384 & 17.246$\pm$0.058 & PO & g \\
238.6408 & 17.272$\pm$0.059 & PO & g \\
238.6432 & 17.270$\pm$0.059 & PO & g \\
238.6457 & 17.174$\pm$0.062 & PO & r \\
238.6481 & 17.153$\pm$0.062 & PO & r \\
238.6506 & 17.135$\pm$0.061 & PO & r \\
238.6530 & 17.116$\pm$0.060 & PO & r \\
238.6556 & 16.794$\pm$0.049 & PO & i \\
238.6581 & 16.605$\pm$0.046 & PO & i \\
238.6605 & 16.829$\pm$0.050 & PO & i \\
238.6630 & 16.831$\pm$0.051 & PO & i \\
238.6654 & 16.063$\pm$0.067 & PO & z \\
238.6679 & 16.024$\pm$0.069 & PO & z \\
238.6703 & 16.147$\pm$0.067 & PO & z \\
238.6728 & 16.119$\pm$0.068 & PO & z \\
240.5565 & 18.547$\pm$0.122 & PO & u \\
240.5589 & 18.461$\pm$0.126 & PO & u \\
240.5613 & 18.655$\pm$0.131 & PO & u \\
240.5638 & 18.689$\pm$0.128 & PO & u \\
240.5662 & 18.547$\pm$0.118 & PO & u \\
240.5687 & 18.498$\pm$0.118 & PO & u \\
240.5711 & 18.710$\pm$0.128 & PO & u \\
240.5737 & 17.180$\pm$0.056 & PO & g \\
240.5762 & 17.192$\pm$0.057 & PO & g \\
240.5786 & 17.189$\pm$0.057 & PO & g \\
240.5811 & 17.203$\pm$0.057 & PO & g \\
240.5835 & 17.211$\pm$0.057 & PO & g \\
240.5860 & 17.132$\pm$0.060 & PO & r \\
240.5884 & 17.158$\pm$0.061 & PO & r \\
240.5909 & 17.139$\pm$0.060 & PO & r \\
240.5933 & 17.118$\pm$0.060 & PO & r \\
240.5959 & 17.118$\pm$0.060 & PO & r \\
240.5984 & 16.836$\pm$0.050 & PO & i \\
240.6009 & 16.839$\pm$0.050 & PO & i \\
240.6033 & 16.844$\pm$0.049 & PO & i \\
240.6058 & 16.808$\pm$0.049 & PO & i \\
240.6082 & 16.839$\pm$0.049 & PO & i \\
240.6107 & 16.882$\pm$0.050 & PO & i \\
240.6131 & 16.147$\pm$0.064 & PO & z \\
240.6156 & 16.162$\pm$0.064 & PO & z \\
240.6180 & 16.200$\pm$0.065 & PO & z \\
240.6204 & 16.269$\pm$0.065 & PO & z \\
240.6229 & 16.205$\pm$0.064 & PO & z \\
240.6253 & 16.180$\pm$0.064 & PO & z \\
240.6285 & 18.476$\pm$0.119 & PO & u \\
240.6309 & 18.559$\pm$0.128 & PO & u \\
240.6333 & 18.623$\pm$0.142 & PO & u \\
240.6358 & 18.861$\pm$0.152 & PO & u \\
240.6382 & 18.738$\pm$0.152 & PO & u \\
240.6406 & 18.731$\pm$0.143 & PO & u \\
240.6430 & 18.797$\pm$0.145 & PO & u \\
240.6456 & 17.219$\pm$0.057 & PO & g \\
240.6480 & 17.191$\pm$0.057 & PO & g \\
240.6505 & 17.225$\pm$0.060 & PO & g \\
240.6529 & 17.222$\pm$0.059 & PO & g \\
240.6553 & 17.193$\pm$0.057 & PO & g \\
240.6578 & 17.257$\pm$0.081 & PO & r \\
240.6602 & 17.290$\pm$0.085 & PO & r \\
240.6628 & 17.177$\pm$0.066 & PO & r \\
240.6653 & 17.113$\pm$0.061 & PO & r \\
240.6677 & 17.205$\pm$0.064 & PO & r \\
240.6702 & 16.779$\pm$0.050 & PO & i \\
240.6726 & 16.871$\pm$0.052 & PO & i \\
240.6750 & 16.939$\pm$0.053 & PO & i \\
240.6775 & 16.866$\pm$0.052 & PO & i \\
240.6799 & 16.905$\pm$0.054 & PO & i \\
240.6823 & 16.878$\pm$0.052 & PO & i \\
240.6848 & 16.192$\pm$0.068 & PO & z \\
240.6872 & 16.140$\pm$0.066 & PO & z \\
240.6898 & 16.086$\pm$0.067 & PO & z \\
240.6923 & 16.040$\pm$0.065 & PO & z \\
240.6947 & 16.057$\pm$0.067 & PO & z \\
240.6971 & 16.128$\pm$0.066 & PO & z \\
241.5630 & 18.358$\pm$0.119 & PO & u \\
241.5679 & 18.948$\pm$0.170 & PO & u \\
241.5703 & 18.718$\pm$0.143 & PO & u \\
241.5753 & 18.670$\pm$0.162 & PO & u \\
241.5777 & 18.494$\pm$0.138 & PO & u \\
241.5802 & 17.286$\pm$0.062 & PO & g \\
241.5827 & 17.307$\pm$0.063 & PO & g \\
241.5852 & 17.197$\pm$0.060 & PO & g \\
241.5877 & 17.326$\pm$0.067 & PO & g \\
241.5901 & 17.359$\pm$0.068 & PO & g \\
241.5926 & 17.169$\pm$0.070 & PO & r \\
241.5950 & 17.295$\pm$0.074 & PO & r \\
241.5975 & 17.138$\pm$0.069 & PO & r \\
241.5999 & 17.491$\pm$0.086 & PO & r \\
241.6024 & 17.213$\pm$0.071 & PO & r \\
241.6048 & 16.834$\pm$0.066 & PO & i \\
241.6073 & 16.775$\pm$0.077 & PO & i \\
241.6097 & 16.915$\pm$0.096 & PO & i \\
241.6121 & 16.395$\pm$0.084 & PO & i \\
241.6148 & 16.351$\pm$0.097 & PO & i \\
241.6172 & 16.455$\pm$0.143 & PO & i \\
245.2854 & 17.049$\pm$0.137 & ATLAS & o \\
245.2881 & 17.200$\pm$0.117 & ATLAS & o \\
245.2974 & 16.975$\pm$0.055 & ATLAS & o \\
247.5361 & 16.976$\pm$0.146 & ATLAS & o \\
247.5628 & 16.941$\pm$0.061 & ATLAS & o \\
247.5927 & 18.502$\pm$0.162 & PO & u \\
247.5951 & 18.105$\pm$0.125 & PO & u \\
247.5975 & 18.362$\pm$0.144 & PO & u \\
247.5999 & 18.260$\pm$0.129 & PO & u \\
247.6023 & 18.593$\pm$0.182 & PO & u \\
247.6048 & 18.624$\pm$0.186 & PO & u \\
247.6072 & 18.208$\pm$0.148 & PO & u \\
247.6098 & 17.140$\pm$0.057 & PO & g \\
247.6122 & 17.105$\pm$0.057 & PO & g \\
247.6146 & 17.108$\pm$0.055 & PO & g \\
247.6171 & 17.119$\pm$0.056 & PO & g \\
247.6195 & 17.133$\pm$0.056 & PO & g \\
247.6220 & 17.108$\pm$0.060 & PO & r \\
247.6244 & 17.080$\pm$0.061 & PO & r \\
247.6269 & 17.147$\pm$0.062 & PO & r \\
247.6293 & 17.155$\pm$0.063 & PO & r \\
247.6319 & 17.064$\pm$0.060 & PO & r \\
247.6344 & 16.784$\pm$0.051 & PO & i \\
247.6368 & 16.729$\pm$0.049 & PO & i \\
247.6393 & 16.753$\pm$0.050 & PO & i \\
247.6417 & 16.862$\pm$0.054 & PO & i \\
247.6441 & 16.783$\pm$0.050 & PO & i \\
247.6466 & 16.845$\pm$0.051 & PO & i \\
247.6491 & 16.066$\pm$0.065 & PO & z \\
247.6515 & 16.060$\pm$0.067 & PO & z \\
247.6540 & 16.126$\pm$0.067 & PO & z \\
247.6564 & 16.023$\pm$0.065 & PO & z \\
247.6588 & 16.180$\pm$0.065 & PO & z \\
247.6615 & 16.066$\pm$0.069 & PO & z \\
247.6646 & 18.295$\pm$0.145 & PO & u \\
247.6670 & 18.644$\pm$0.192 & PO & u \\
247.6695 & 18.811$\pm$0.282 & PO & u \\
247.6819 & 17.211$\pm$0.068 & PO & g \\
247.6844 & 17.214$\pm$0.066 & PO & g \\
247.6868 & 17.065$\pm$0.064 & PO & g \\
247.6892 & 17.224$\pm$0.065 & PO & g \\
247.6917 & 17.133$\pm$0.067 & PO & g \\
248.5788 & 18.264$\pm$0.136 & PO & u \\
248.5812 & 18.804$\pm$0.205 & PO & u \\
248.5836 & 18.187$\pm$0.137 & PO & u \\
248.5861 & 18.430$\pm$0.153 & PO & u \\
248.5885 & 18.570$\pm$0.169 & PO & u \\
248.5909 & 18.705$\pm$0.220 & PO & u \\
248.5933 & 18.509$\pm$0.187 & PO & u \\
248.5958 & 17.141$\pm$0.057 & PO & g \\
248.5983 & 17.125$\pm$0.059 & PO & g \\
248.6007 & 17.269$\pm$0.064 & PO & g \\
248.6032 & 17.226$\pm$0.060 & PO & g \\
248.6056 & 17.176$\pm$0.061 & PO & g \\
248.6080 & 17.101$\pm$0.062 & PO & r \\
248.6105 & 17.126$\pm$0.062 & PO & r \\
248.6131 & 17.109$\pm$0.062 & PO & r \\
248.6155 & 17.080$\pm$0.061 & PO & r \\
248.6180 & 17.140$\pm$0.063 & PO & r \\
248.6205 & 16.609$\pm$0.047 & PO & i \\
248.6229 & 16.879$\pm$0.053 & PO & i \\
248.6254 & 16.754$\pm$0.049 & PO & i \\
248.6278 & 16.749$\pm$0.050 & PO & i \\
248.6302 & 16.786$\pm$0.051 & PO & i \\
248.6326 & 16.797$\pm$0.052 & PO & i \\
248.6351 & 16.078$\pm$0.065 & PO & z \\
248.6375 & 16.083$\pm$0.066 & PO & z \\
248.6400 & 16.097$\pm$0.066 & PO & z \\
248.6424 & 16.103$\pm$0.066 & PO & z \\
248.6451 & 16.083$\pm$0.073 & PO & z \\
248.6475 & 15.952$\pm$0.071 & PO & z \\
249.3360 & 16.960$\pm$0.056 & ATLAS & o \\
249.3402 & 16.998$\pm$0.059 & ATLAS & o \\
249.3461 & 17.058$\pm$0.082 & ATLAS & o \\
249.3689 & 16.985$\pm$0.076 & ATLAS & o \\
249.5571 & 18.154$\pm$0.126 & PO & u \\
249.5595 & 18.424$\pm$0.137 & PO & u \\
249.5620 & 18.803$\pm$0.196 & PO & u \\
249.5644 & 18.103$\pm$0.130 & PO & u \\
249.5693 & 18.516$\pm$0.196 & PO & u \\
249.5718 & 18.653$\pm$0.200 & PO & u \\
249.5743 & 17.199$\pm$0.062 & PO & g \\
249.5768 & 17.329$\pm$0.065 & PO & g \\
249.5792 & 17.294$\pm$0.067 & PO & g \\
249.5817 & 17.259$\pm$0.062 & PO & g \\
249.5841 & 17.281$\pm$0.064 & PO & g \\
249.5890 & 17.221$\pm$0.068 & PO & r \\
249.5914 & 17.220$\pm$0.066 & PO & r \\
249.5938 & 17.136$\pm$0.062 & PO & r \\
249.5965 & 17.202$\pm$0.064 & PO & r \\
249.5989 & 16.819$\pm$0.051 & PO & i \\
249.6014 & 16.859$\pm$0.052 & PO & i \\
249.6038 & 16.714$\pm$0.050 & PO & i \\
249.6062 & 16.777$\pm$0.049 & PO & i \\
249.6087 & 16.747$\pm$0.050 & PO & i \\
249.6111 & 16.781$\pm$0.050 & PO & i \\
249.6136 & 16.112$\pm$0.066 & PO & z \\
249.6160 & 16.110$\pm$0.067 & PO & z \\
249.6184 & 16.156$\pm$0.067 & PO & z \\
249.6209 & 16.190$\pm$0.068 & PO & z \\
249.6234 & 16.031$\pm$0.066 & PO & z \\
249.6258 & 16.157$\pm$0.066 & PO & z \\
250.5788 & 17.241$\pm$0.069 & PO & g \\
250.5813 & 17.329$\pm$0.065 & PO & g \\
250.5837 & 17.230$\pm$0.086 & PO & g \\
250.5861 & 17.302$\pm$0.070 & PO & g \\
250.5885 & 17.301$\pm$0.068 & PO & g \\
250.5911 & 17.176$\pm$0.067 & PO & r \\
250.5935 & 17.237$\pm$0.069 & PO & r \\
250.5960 & 17.203$\pm$0.068 & PO & r \\
250.5984 & 17.211$\pm$0.066 & PO & r \\
250.6008 & 17.223$\pm$0.068 & PO & r \\
250.6033 & 16.887$\pm$0.055 & PO & i \\
250.6057 & 16.907$\pm$0.054 & PO & i \\
250.6082 & 16.838$\pm$0.055 & PO & i \\
250.6106 & 16.903$\pm$0.054 & PO & i \\
250.6130 & 16.915$\pm$0.060 & PO & i \\
250.6154 & 16.874$\pm$0.056 & PO & i \\
250.6181 & 16.293$\pm$0.073 & PO & z \\
250.6205 & 16.261$\pm$0.075 & PO & z \\
251.5897 & 18.170$\pm$0.130 & PO & u \\
251.5927 & 18.415$\pm$0.205 & PO & u \\
251.5958 & 18.140$\pm$0.132 & PO & u \\
251.6018 & 18.931$\pm$0.296 & PO & u \\
251.6110 & 17.134$\pm$0.128 & PO & g \\
251.6134 & 17.197$\pm$0.122 & PO & g \\
251.6159 & 17.218$\pm$0.093 & PO & g \\
251.6183 & 17.265$\pm$0.110 & PO & g \\
251.6208 & 17.110$\pm$0.091 & PO & g \\
251.6234 & 17.426$\pm$0.111 & PO & r \\
251.6259 & 16.976$\pm$0.117 & PO & r \\
251.6283 & 17.077$\pm$0.106 & PO & r \\
251.6305 & 17.140$\pm$0.052 & ZTF & g \\
251.6305 & 17.140$\pm$0.052 & ZTF & g \\
251.6308 & 17.171$\pm$0.097 & PO & r \\
251.6332 & 17.433$\pm$0.100 & PO & r \\
251.6357 & 17.056$\pm$0.116 & PO & i \\
251.6381 & 17.002$\pm$0.093 & PO & i \\
251.6405 & 17.122$\pm$0.085 & PO & i \\
251.6430 & 16.889$\pm$0.068 & PO & i \\
251.6456 & 16.906$\pm$0.066 & PO & i \\
251.6480 & 16.727$\pm$0.062 & PO & i \\
251.6505 & 16.124$\pm$0.080 & PO & z \\
251.6530 & 16.142$\pm$0.085 & PO & z \\
251.6554 & 16.131$\pm$0.086 & PO & z \\
251.6578 & 16.188$\pm$0.090 & PO & z \\
251.6594 & 17.172$\pm$0.035 & ZTF & r \\
251.6594 & 17.172$\pm$0.035 & ZTF & r \\
251.6599 & 17.266$\pm$0.053 & ZTF & r \\
251.6599 & 17.266$\pm$0.053 & ZTF & r \\
251.6602 & 16.005$\pm$0.077 & PO & z \\
251.6627 & 15.957$\pm$0.078 & PO & z \\
252.5569 & 18.955$\pm$0.179 & PO & u \\
252.5599 & 18.560$\pm$0.134 & PO & u \\
252.5629 & 18.937$\pm$0.168 & PO & u \\
252.5659 & 18.736$\pm$0.171 & PO & u \\
252.5689 & 19.095$\pm$0.231 & PO & u \\
252.5719 & 19.066$\pm$0.222 & PO & u \\
252.5780 & 17.475$\pm$0.071 & PO & g \\
252.5805 & 17.316$\pm$0.064 & PO & g \\
252.5829 & 17.351$\pm$0.065 & PO & g \\
252.5854 & 17.310$\pm$0.063 & PO & g \\
252.5878 & 17.350$\pm$0.065 & PO & g \\
252.5902 & 17.215$\pm$0.065 & PO & r \\
252.5927 & 17.209$\pm$0.064 & PO & r \\
252.5953 & 17.278$\pm$0.066 & PO & r \\
252.5977 & 17.230$\pm$0.065 & PO & r \\
252.6002 & 17.280$\pm$0.066 & PO & r \\
252.6027 & 16.940$\pm$0.053 & PO & i \\
252.6051 & 16.914$\pm$0.053 & PO & i \\
252.6075 & 17.016$\pm$0.055 & PO & i \\
252.6099 & 16.996$\pm$0.055 & PO & i \\
252.6124 & 16.956$\pm$0.054 & PO & i \\
252.6148 & 16.934$\pm$0.054 & PO & i \\
252.6173 & 16.229$\pm$0.065 & PO & z \\
252.6197 & 16.233$\pm$0.065 & PO & z \\
252.6221 & 16.191$\pm$0.065 & PO & z \\
252.6246 & 16.244$\pm$0.066 & PO & z \\
252.6272 & 16.263$\pm$0.069 & PO & z \\
252.6296 & 16.193$\pm$0.068 & PO & z \\
253.5631 & 17.401$\pm$0.063 & PO & g \\
253.5661 & 17.343$\pm$0.062 & PO & g \\
253.5691 & 17.393$\pm$0.063 & PO & g \\
253.5721 & 17.349$\pm$0.062 & PO & g \\
253.5751 & 17.486$\pm$0.071 & PO & g \\
253.5781 & 17.224$\pm$0.064 & PO & r \\
253.5806 & 17.313$\pm$0.068 & PO & r \\
253.5830 & 17.310$\pm$0.068 & PO & r \\
253.5854 & 17.301$\pm$0.066 & PO & r \\
253.5878 & 17.309$\pm$0.068 & PO & r \\
253.5904 & 17.041$\pm$0.059 & PO & i \\
253.5928 & 17.025$\pm$0.057 & PO & i \\
253.5952 & 16.954$\pm$0.054 & PO & i \\
253.5977 & 17.041$\pm$0.057 & PO & i \\
253.6003 & 16.890$\pm$0.054 & PO & i \\
253.6027 & 16.905$\pm$0.054 & PO & i \\
253.6052 & 16.221$\pm$0.072 & PO & z \\
253.6076 & 16.143$\pm$0.071 & PO & z \\
253.6100 & 16.220$\pm$0.070 & PO & z \\
253.6125 & 16.193$\pm$0.067 & PO & z \\
253.6149 & 16.237$\pm$0.071 & PO & z \\
253.6173 & 16.120$\pm$0.071 & PO & z \\
254.5564 & 17.408$\pm$0.063 & PO & g \\
254.5594 & 17.458$\pm$0.067 & PO & g \\
254.5624 & 17.436$\pm$0.064 & PO & g \\
254.5655 & 17.437$\pm$0.065 & PO & g \\
254.5685 & 17.461$\pm$0.065 & PO & g \\
254.5715 & 17.395$\pm$0.070 & PO & r \\
254.5739 & 17.290$\pm$0.067 & PO & r \\
254.5764 & 17.292$\pm$0.066 & PO & r \\
254.5788 & 17.349$\pm$0.067 & PO & r \\
254.5812 & 17.343$\pm$0.067 & PO & r \\
254.5837 & 17.059$\pm$0.057 & PO & i \\
254.5862 & 17.016$\pm$0.057 & PO & i \\
254.5888 & 16.954$\pm$0.054 & PO & i \\
254.5912 & 16.973$\pm$0.054 & PO & i \\
254.5936 & 16.974$\pm$0.055 & PO & i \\
254.5960 & 16.935$\pm$0.053 & PO & i \\
254.5985 & 16.206$\pm$0.069 & PO & z \\
254.6009 & 16.264$\pm$0.070 & PO & z \\
254.6034 & 16.202$\pm$0.067 & PO & z \\
254.6058 & 16.184$\pm$0.069 & PO & z \\
254.6082 & 16.217$\pm$0.067 & PO & z \\
254.6107 & 16.280$\pm$0.067 & PO & z \\
255.5565 & 17.357$\pm$0.063 & PO & g \\
255.5595 & 17.348$\pm$0.062 & PO & g \\
255.5625 & 17.465$\pm$0.067 & PO & g \\
255.5655 & 17.512$\pm$0.067 & PO & g \\
255.5685 & 17.333$\pm$0.063 & PO & g \\
255.5715 & 17.205$\pm$0.071 & PO & r \\
255.5739 & 17.318$\pm$0.082 & PO & r \\
255.5764 & 17.501$\pm$0.117 & PO & r \\
255.5788 & 17.412$\pm$0.105 & PO & r \\
255.5812 & 17.361$\pm$0.084 & PO & r \\
255.5837 & 17.169$\pm$0.127 & PO & i \\
255.5862 & 17.315$\pm$0.156 & PO & i \\
255.5886 & 17.275$\pm$0.146 & PO & i \\
255.5912 & 16.765$\pm$0.078 & PO & i \\
255.5936 & 16.980$\pm$0.083 & PO & i \\
255.5960 & 16.963$\pm$0.083 & PO & i \\
255.5986 & 16.126$\pm$0.122 & PO & z \\
255.6010 & 16.099$\pm$0.096 & PO & z \\
255.6034 & 16.162$\pm$0.105 & PO & z \\
255.6058 & 16.227$\pm$0.101 & PO & z \\
255.6083 & 16.151$\pm$0.083 & PO & z \\
255.6107 & 16.240$\pm$0.080 & PO & z \\
256.5565 & 17.618$\pm$0.071 & PO & g \\
256.5595 & 17.571$\pm$0.069 & PO & g \\
256.5625 & 17.583$\pm$0.069 & PO & g \\
256.5655 & 17.297$\pm$0.061 & PO & g \\
256.5685 & 17.479$\pm$0.066 & PO & g \\
256.5716 & 17.379$\pm$0.069 & PO & r \\
256.5740 & 17.381$\pm$0.069 & PO & r \\
256.5764 & 17.322$\pm$0.067 & PO & r \\
256.5789 & 17.330$\pm$0.067 & PO & r \\
256.5813 & 17.341$\pm$0.067 & PO & r \\
256.5838 & 17.034$\pm$0.057 & PO & i \\
256.5862 & 17.057$\pm$0.057 & PO & i \\
256.5886 & 17.059$\pm$0.061 & PO & i \\
256.5911 & 17.070$\pm$0.060 & PO & i \\
256.5935 & 17.128$\pm$0.060 & PO & i \\
256.5959 & 17.061$\pm$0.060 & PO & i \\
256.5986 & 16.541$\pm$0.094 & PO & z \\
256.6010 & 16.613$\pm$0.110 & PO & z \\
256.6035 & 16.487$\pm$0.092 & PO & z \\
256.6060 & 16.402$\pm$0.087 & PO & z \\
256.6084 & 16.354$\pm$0.086 & PO & z \\
256.6108 & 16.302$\pm$0.087 & PO & z \\
256.6299 & 17.308$\pm$0.042 & ZTF & r \\
256.6299 & 17.308$\pm$0.042 & ZTF & r \\
256.9953 & 16.552$\pm$0.006 & Mephisto & i \\
256.9953 & 18.421$\pm$0.046 & Mephisto & v \\
257.0026 & 16.521$\pm$0.006 & Mephisto & i \\
257.0026 & 18.321$\pm$0.041 & Mephisto & v \\
257.0052 & 16.540$\pm$0.006 & Mephisto & i \\
257.0052 & 18.327$\pm$0.041 & Mephisto & v \\
257.0086 & 19.120$\pm$0.060 & Mephisto & u \\
257.0086 & 17.079$\pm$0.034 & Mephisto & z \\
257.0110 & 19.118$\pm$0.060 & Mephisto & u \\
257.0110 & 17.083$\pm$0.035 & Mephisto & z \\
257.0133 & 19.128$\pm$0.060 & Mephisto & u \\
257.0133 & 17.064$\pm$0.034 & Mephisto & z \\
257.5664 & 17.438$\pm$0.065 & PO & g \\
257.5694 & 17.447$\pm$0.065 & PO & g \\
257.5725 & 17.388$\pm$0.063 & PO & g \\
257.5755 & 17.407$\pm$0.063 & PO & g \\
257.5785 & 17.382$\pm$0.063 & PO & g \\
257.5815 & 17.323$\pm$0.067 & PO & r \\
257.5840 & 17.278$\pm$0.065 & PO & r \\
257.5864 & 17.301$\pm$0.066 & PO & r \\
257.5888 & 17.312$\pm$0.066 & PO & r \\
257.5912 & 17.299$\pm$0.065 & PO & r \\
257.5937 & 16.995$\pm$0.055 & PO & i \\
257.5962 & 17.044$\pm$0.056 & PO & i \\
257.5988 & 16.989$\pm$0.054 & PO & i \\
257.6012 & 16.988$\pm$0.054 & PO & i \\
257.6036 & 16.948$\pm$0.054 & PO & i \\
257.6061 & 16.952$\pm$0.053 & PO & i \\
257.6086 & 16.202$\pm$0.068 & PO & z \\
257.6110 & 16.199$\pm$0.069 & PO & z \\
257.6134 & 16.266$\pm$0.069 & PO & z \\
257.6159 & 16.193$\pm$0.067 & PO & z \\
257.6183 & 16.285$\pm$0.068 & PO & z \\
257.6206 & 17.208$\pm$0.087 & P60 & i \\
257.6207 & 16.259$\pm$0.068 & PO & z \\
257.6634 & 17.327$\pm$0.071 & ZTF & r \\
257.6634 & 17.327$\pm$0.071 & ZTF & r \\
257.6957 & 17.360$\pm$0.099 & P60 & r \\
257.9871 & 18.099$\pm$0.034 & Mephisto & v \\
257.9871 & 16.395$\pm$0.006 & Mephisto & i \\
257.9896 & 18.192$\pm$0.037 & Mephisto & v \\
257.9897 & 16.385$\pm$0.006 & Mephisto & i \\
257.9920 & 16.388$\pm$0.006 & Mephisto & i \\
257.9920 & 18.209$\pm$0.037 & Mephisto & v \\
257.9959 & 18.792$\pm$0.044 & Mephisto & u \\
257.9960 & 16.725$\pm$0.025 & Mephisto & z \\
257.9984 & 16.720$\pm$0.025 & Mephisto & z \\
257.9984 & 18.785$\pm$0.043 & Mephisto & u \\
258.0010 & 16.767$\pm$0.026 & Mephisto & z \\
258.0011 & 18.731$\pm$0.041 & Mephisto & u \\
258.6200 & 17.065$\pm$0.055 & ZTF & g \\
258.6200 & 17.065$\pm$0.055 & ZTF & g \\
258.6332 & 17.139$\pm$0.040 & ZTF & r \\
258.6332 & 17.139$\pm$0.040 & ZTF & r \\
258.9873 & 16.279$\pm$0.006 & Mephisto & i \\
258.9873 & 18.075$\pm$0.033 & Mephisto & v \\
258.9900 & 18.103$\pm$0.034 & Mephisto & v \\
258.9930 & 18.150$\pm$0.036 & Mephisto & v \\
258.9981 & 18.711$\pm$0.041 & Mephisto & u \\
259.0013 & 18.785$\pm$0.043 & Mephisto & u \\
259.0036 & 18.759$\pm$0.042 & Mephisto & u \\
259.0071 & 16.344$\pm$0.006 & Mephisto & i \\
259.0095 & 16.338$\pm$0.006 & Mephisto & i \\
259.0132 & 16.665$\pm$0.024 & Mephisto & z \\
259.0155 & 16.539$\pm$0.022 & Mephisto & z \\
259.0178 & 16.570$\pm$0.022 & Mephisto & z \\
259.5814 & 17.264$\pm$0.059 & PO & g \\
259.5844 & 17.301$\pm$0.060 & PO & g \\
259.5875 & 17.241$\pm$0.058 & PO & g \\
259.5905 & 17.249$\pm$0.059 & PO & g \\
259.5936 & 17.291$\pm$0.060 & PO & g \\
259.5966 & 17.229$\pm$0.064 & PO & r \\
259.5990 & 17.243$\pm$0.064 & PO & r \\
259.6015 & 17.178$\pm$0.063 & PO & r \\
259.6039 & 17.264$\pm$0.065 & PO & r \\
259.6063 & 17.133$\pm$0.062 & PO & r \\
259.6088 & 16.815$\pm$0.050 & PO & i \\
259.6114 & 16.764$\pm$0.049 & PO & i \\
259.6139 & 16.820$\pm$0.051 & PO & i \\
259.6163 & 16.818$\pm$0.051 & PO & i \\
259.6187 & 16.821$\pm$0.051 & PO & i \\
259.6211 & 16.880$\pm$0.058 & PO & i \\
259.6236 & 16.094$\pm$0.068 & PO & z \\
259.6260 & 15.916$\pm$0.070 & PO & z \\
259.6285 & 16.032$\pm$0.072 & PO & z \\
259.6309 & 16.019$\pm$0.070 & PO & z \\
259.6333 & 15.744$\pm$0.064 & PO & z \\
259.6357 & 16.054$\pm$0.072 & PO & z \\
259.9881 & 16.271$\pm$0.006 & Mephisto & i \\
259.9881 & 18.049$\pm$0.032 & Mephisto & v \\
259.9931 & 18.068$\pm$0.033 & Mephisto & v \\
259.9931 & 16.249$\pm$0.006 & Mephisto & i \\
259.9962 & 16.567$\pm$0.022 & Mephisto & z \\
259.9986 & 16.506$\pm$0.022 & Mephisto & z \\
260.0009 & 16.516$\pm$0.022 & Mephisto & z \\
260.7094 & 17.035$\pm$0.041 & ATLAS & o \\
260.7126 & 16.956$\pm$0.037 & ATLAS & o \\
260.7371 & 17.011$\pm$0.030 & ATLAS & o \\
260.9919 & 18.006$\pm$0.031 & Mephisto & v \\
260.9983 & 18.047$\pm$0.032 & Mephisto & v \\
261.9929 & 16.334$\pm$0.005 & Mephisto & i \\
261.9929 & 18.038$\pm$0.033 & Mephisto & v \\
261.9952 & 18.047$\pm$0.033 & Mephisto & v \\
261.9952 & 16.313$\pm$0.005 & Mephisto & i \\
261.9975 & 18.059$\pm$0.034 & Mephisto & v \\
261.9975 & 16.332$\pm$0.005 & Mephisto & i \\
262.0010 & 16.667$\pm$0.023 & Mephisto & z \\
262.0033 & 16.673$\pm$0.023 & Mephisto & z \\
262.0056 & 16.649$\pm$0.023 & Mephisto & z \\
262.9900 & 17.937$\pm$0.029 & Mephisto & v \\
262.9900 & 16.238$\pm$0.005 & Mephisto & i \\
263.0004 & 16.282$\pm$0.005 & Mephisto & i \\
263.0004 & 17.947$\pm$0.029 & Mephisto & v \\
263.0037 & 16.566$\pm$0.021 & Mephisto & z \\
263.0037 & 18.472$\pm$0.033 & Mephisto & u \\
263.0062 & 18.434$\pm$0.032 & Mephisto & u \\
263.0062 & 16.557$\pm$0.021 & Mephisto & z \\
263.0085 & 18.467$\pm$0.033 & Mephisto & u \\
263.0085 & 16.503$\pm$0.021 & Mephisto & z \\
263.0138 & 16.297$\pm$0.005 & Mephisto & i \\
263.0138 & 17.907$\pm$0.028 & Mephisto & v \\
263.5785 & 17.080$\pm$0.054 & PO & g \\
263.5809 & 17.068$\pm$0.053 & PO & g \\
263.5834 & 17.082$\pm$0.053 & PO & g \\
263.5858 & 17.110$\pm$0.054 & PO & g \\
263.5882 & 17.136$\pm$0.055 & PO & g \\
263.5906 & 17.127$\pm$0.055 & PO & g \\
263.5931 & 17.136$\pm$0.061 & PO & r \\
263.5955 & 17.170$\pm$0.062 & PO & r \\
263.5980 & 17.072$\pm$0.059 & PO & r \\
263.6004 & 17.130$\pm$0.060 & PO & r \\
263.6029 & 17.086$\pm$0.059 & PO & r \\
263.6053 & 17.114$\pm$0.060 & PO & r \\
263.6080 & 16.540$\pm$0.043 & PO & i \\
263.6104 & 16.558$\pm$0.044 & PO & i \\
263.6128 & 16.655$\pm$0.046 & PO & i \\
263.6153 & 16.702$\pm$0.047 & PO & i \\
263.6177 & 16.656$\pm$0.046 & PO & i \\
263.6201 & 16.684$\pm$0.047 & PO & i \\
263.6226 & 16.037$\pm$0.064 & PO & z \\
263.6250 & 16.048$\pm$0.064 & PO & z \\
263.6274 & 16.093$\pm$0.066 & PO & z \\
263.6299 & 16.065$\pm$0.065 & PO & z \\
263.6325 & 16.085$\pm$0.070 & PO & z \\
263.6349 & 15.974$\pm$0.066 & PO & z \\
263.9897 & 16.285$\pm$0.005 & Mephisto & i \\
263.9897 & 17.827$\pm$0.026 & Mephisto & v \\
263.9919 & 16.293$\pm$0.005 & Mephisto & i \\
263.9919 & 17.837$\pm$0.026 & Mephisto & v \\
263.9942 & 17.844$\pm$0.027 & Mephisto & v \\
263.9942 & 16.311$\pm$0.005 & Mephisto & i \\
263.9973 & 16.665$\pm$0.023 & Mephisto & z \\
263.9973 & 18.449$\pm$0.032 & Mephisto & u \\
263.9996 & 18.435$\pm$0.032 & Mephisto & u \\
263.9996 & 16.652$\pm$0.023 & Mephisto & z \\
264.0024 & 18.391$\pm$0.030 & Mephisto & u \\
264.0024 & 16.649$\pm$0.023 & Mephisto & z \\
264.0057 & 16.677$\pm$0.023 & Mephisto & z \\
264.0058 & 18.450$\pm$0.032 & Mephisto & u \\
264.0123 & 17.876$\pm$0.027 & Mephisto & v \\
264.0123 & 16.331$\pm$0.005 & Mephisto & i \\
264.3062 & 17.009$\pm$0.062 & ATLAS & c \\
264.5669 & 17.266$\pm$0.060 & PO & g \\
264.5694 & 17.247$\pm$0.060 & PO & g \\
264.5718 & 17.266$\pm$0.059 & PO & g \\
264.5742 & 17.308$\pm$0.061 & PO & g \\
264.5766 & 17.295$\pm$0.061 & PO & g \\
264.5791 & 17.341$\pm$0.062 & PO & g \\
264.5816 & 17.194$\pm$0.064 & PO & r \\
264.5840 & 17.198$\pm$0.066 & PO & r \\
264.5864 & 17.242$\pm$0.068 & PO & r \\
264.5888 & 17.253$\pm$0.067 & PO & r \\
264.5913 & 17.315$\pm$0.068 & PO & r \\
264.5937 & 17.229$\pm$0.065 & PO & r \\
264.5962 & 16.851$\pm$0.053 & PO & i \\
264.5988 & 16.675$\pm$0.049 & PO & i \\
264.6012 & 16.844$\pm$0.058 & PO & i \\
264.6036 & 16.781$\pm$0.052 & PO & i \\
264.6061 & 16.779$\pm$0.052 & PO & i \\
264.6086 & 16.864$\pm$0.054 & PO & i \\
264.6110 & 16.231$\pm$0.076 & PO & z \\
264.6135 & 16.163$\pm$0.073 & PO & z \\
264.6159 & 16.227$\pm$0.074 & PO & z \\
264.6185 & 16.244$\pm$0.083 & PO & z \\
264.6210 & 16.043$\pm$0.076 & PO & z \\
264.6234 & 16.068$\pm$0.074 & PO & z \\
264.7094 & 16.971$\pm$0.051 & ATLAS & o \\
265.5670 & 17.361$\pm$0.063 & PO & g \\
265.5694 & 17.337$\pm$0.062 & PO & g \\
265.5718 & 17.310$\pm$0.060 & PO & g \\
265.5742 & 17.326$\pm$0.061 & PO & g \\
265.5766 & 17.296$\pm$0.060 & PO & g \\
265.5790 & 17.311$\pm$0.060 & PO & g \\
265.5815 & 17.258$\pm$0.065 & PO & r \\
265.5839 & 17.330$\pm$0.067 & PO & r \\
265.5864 & 17.280$\pm$0.065 & PO & r \\
265.5888 & 17.279$\pm$0.066 & PO & r \\
265.5912 & 17.276$\pm$0.065 & PO & r \\
265.5937 & 17.202$\pm$0.063 & PO & r \\
265.5963 & 16.851$\pm$0.054 & PO & i \\
265.5987 & 16.929$\pm$0.056 & PO & i \\
265.6012 & 16.927$\pm$0.055 & PO & i \\
265.6036 & 16.905$\pm$0.059 & PO & i \\
265.6060 & 16.947$\pm$0.055 & PO & i \\
265.6084 & 16.929$\pm$0.054 & PO & i \\
265.6109 & 16.193$\pm$0.067 & PO & z \\
265.6134 & 16.253$\pm$0.069 & PO & z \\
265.6160 & 16.206$\pm$0.087 & PO & z \\
265.6184 & 16.032$\pm$0.084 & PO & z \\
265.6208 & 16.156$\pm$0.084 & PO & z \\
265.6232 & 16.084$\pm$0.086 & PO & z \\
265.9983 & 18.039$\pm$0.032 & Mephisto & v \\
266.5670 & 17.340$\pm$0.061 & PO & g \\
266.5694 & 17.311$\pm$0.060 & PO & g \\
266.5719 & 17.308$\pm$0.060 & PO & g \\
266.5743 & 17.344$\pm$0.061 & PO & g \\
266.5767 & 17.367$\pm$0.062 & PO & g \\
266.5792 & 17.319$\pm$0.060 & PO & g \\
266.5816 & 17.302$\pm$0.065 & PO & r \\
266.5840 & 17.361$\pm$0.067 & PO & r \\
266.5865 & 17.399$\pm$0.069 & PO & r \\
266.5889 & 17.318$\pm$0.066 & PO & r \\
266.5914 & 17.318$\pm$0.065 & PO & r \\
266.5940 & 17.371$\pm$0.067 & PO & r \\
266.5964 & 16.950$\pm$0.053 & PO & i \\
266.5989 & 16.960$\pm$0.053 & PO & i \\
266.6013 & 17.008$\pm$0.056 & PO & i \\
266.6037 & 17.025$\pm$0.056 & PO & i \\
266.6061 & 17.081$\pm$0.058 & PO & i \\
266.6086 & 17.123$\pm$0.065 & PO & i \\
266.6110 & 16.320$\pm$0.068 & PO & z \\
266.6134 & 16.262$\pm$0.069 & PO & z \\
266.6161 & 16.130$\pm$0.083 & PO & z \\
266.6185 & 16.131$\pm$0.080 & PO & z \\
266.6209 & 16.178$\pm$0.080 & PO & z \\
266.6234 & 16.186$\pm$0.074 & PO & z \\
267.5567 & 17.606$\pm$0.076 & PO & g \\
267.5592 & 17.611$\pm$0.077 & PO & g \\
267.5617 & 17.483$\pm$0.067 & PO & g \\
267.5641 & 17.440$\pm$0.064 & PO & g \\
267.5665 & 17.486$\pm$0.066 & PO & g \\
267.5690 & 17.506$\pm$0.067 & PO & g \\
267.5715 & 17.441$\pm$0.071 & PO & r \\
267.5739 & 17.438$\pm$0.070 & PO & r \\
267.5763 & 17.420$\pm$0.073 & PO & r \\
267.5787 & 17.455$\pm$0.071 & PO & r \\
267.5814 & 17.427$\pm$0.070 & PO & r \\
267.5838 & 17.449$\pm$0.071 & PO & r \\
267.5862 & 17.088$\pm$0.061 & PO & i \\
267.5887 & 17.131$\pm$0.059 & PO & i \\
267.5911 & 17.129$\pm$0.059 & PO & i \\
267.5935 & 17.175$\pm$0.063 & PO & i \\
267.5960 & 17.174$\pm$0.062 & PO & i \\
267.5984 & 17.198$\pm$0.065 & PO & i \\
267.6225 & 17.399$\pm$0.065 & ZTF & r \\
267.6225 & 17.399$\pm$0.065 & ZTF & r \\
268.6552 & 17.509$\pm$0.063 & ZTF & r \\
269.9925 & 16.729$\pm$0.013 & Mephisto & i \\
269.9930 & 16.629$\pm$0.014 & Mephisto & i \\
269.9936 & 16.698$\pm$0.013 & Mephisto & i \\
269.9950 & 17.053$\pm$0.040 & Mephisto & z \\
269.9956 & 17.082$\pm$0.036 & Mephisto & z \\
269.9961 & 17.358$\pm$0.048 & Mephisto & z \\
270.5785 & 17.627$\pm$0.073 & PO & g \\
270.5809 & 17.610$\pm$0.074 & PO & g \\
270.5833 & 17.787$\pm$0.082 & PO & g \\
270.5858 & 17.630$\pm$0.074 & PO & g \\
270.5882 & 17.663$\pm$0.075 & PO & g \\
270.5907 & 17.596$\pm$0.078 & PO & r \\
270.5932 & 17.671$\pm$0.080 & PO & r \\
270.5956 & 17.627$\pm$0.077 & PO & r \\
270.5980 & 17.643$\pm$0.080 & PO & r \\
270.6006 & 17.589$\pm$0.076 & PO & r \\
270.6031 & 17.390$\pm$0.070 & PO & i \\
270.6055 & 17.455$\pm$0.074 & PO & i \\
270.6080 & 17.503$\pm$0.077 & PO & i \\
271.5641 & 17.770$\pm$0.082 & PO & g \\
271.5665 & 17.773$\pm$0.084 & PO & g \\
271.5690 & 17.717$\pm$0.076 & PO & g \\
271.5715 & 17.971$\pm$0.100 & PO & g \\
271.5739 & 17.742$\pm$0.077 & PO & g \\
271.5763 & 17.614$\pm$0.081 & PO & r \\
271.5788 & 17.677$\pm$0.084 & PO & r \\
271.5812 & 17.699$\pm$0.087 & PO & r \\
271.5837 & 17.534$\pm$0.077 & PO & r \\
271.5861 & 17.688$\pm$0.086 & PO & r \\
271.5887 & 17.612$\pm$0.082 & PO & i \\
271.5912 & 17.700$\pm$0.087 & PO & i \\
271.5936 & 17.692$\pm$0.088 & PO & i \\
271.5960 & 17.816$\pm$0.103 & PO & i \\
271.5984 & 17.686$\pm$0.087 & PO & i \\
272.5637 & 18.021$\pm$0.112 & PO & g \\
272.5662 & 17.984$\pm$0.099 & PO & g \\
272.5686 & 17.967$\pm$0.095 & PO & g \\
272.5711 & 17.985$\pm$0.102 & PO & g \\
272.5736 & 17.798$\pm$0.086 & PO & g \\
272.5760 & 17.710$\pm$0.091 & PO & r \\
272.5784 & 17.927$\pm$0.104 & PO & r \\
272.5809 & 17.558$\pm$0.087 & PO & r \\
272.5833 & 17.675$\pm$0.096 & PO & r \\
272.5857 & 18.197$\pm$0.130 & PO & r \\
272.5884 & 17.676$\pm$0.101 & PO & i \\
272.5908 & 17.732$\pm$0.109 & PO & i \\
272.5932 & 18.177$\pm$0.177 & PO & i \\
272.5957 & 18.087$\pm$0.148 & PO & i \\
272.5981 & 18.059$\pm$0.148 & PO & i \\
272.6043 & 17.840$\pm$0.104 & P60 & r \\
272.6097 & 17.936$\pm$0.108 & P60 & i \\
273.5637 & 17.865$\pm$0.085 & PO & g \\
273.5662 & 17.965$\pm$0.096 & PO & g \\
273.5686 & 18.022$\pm$0.094 & PO & g \\
273.5710 & 18.111$\pm$0.095 & PO & g \\
273.5735 & 18.096$\pm$0.098 & PO & g \\
273.5759 & 17.846$\pm$0.087 & PO & r \\
273.5784 & 17.976$\pm$0.098 & PO & r \\
273.5810 & 18.040$\pm$0.100 & PO & r \\
273.5834 & 17.929$\pm$0.095 & PO & r \\
273.5859 & 17.929$\pm$0.094 & PO & r \\
273.5883 & 17.730$\pm$0.088 & PO & i \\
273.5908 & 17.618$\pm$0.086 & PO & i \\
273.5932 & 17.724$\pm$0.089 & PO & i \\
273.5958 & 17.560$\pm$0.080 & PO & i \\
273.5982 & 17.477$\pm$0.081 & PO & i \\
273.6053 & 18.010$\pm$0.114 & P60 & r \\
274.5636 & 18.004$\pm$0.097 & PO & g \\
274.5666 & 18.026$\pm$0.100 & PO & g \\
274.5696 & 17.936$\pm$0.088 & PO & g \\
274.5726 & 18.166$\pm$0.100 & PO & g \\
274.5756 & 18.085$\pm$0.097 & PO & g \\
274.5786 & 18.037$\pm$0.091 & PO & g \\
274.5840 & 17.988$\pm$0.097 & PO & r \\
274.5870 & 18.136$\pm$0.100 & PO & r \\
274.5902 & 17.991$\pm$0.094 & PO & r \\
274.5932 & 18.053$\pm$0.098 & PO & r \\
274.5962 & 18.005$\pm$0.095 & PO & r \\
274.5993 & 17.923$\pm$0.093 & PO & r \\
275.0025 & 19.521$\pm$0.084 & Mephisto & u \\
275.0025 & 17.341$\pm$0.012 & Mephisto & i \\
275.0074 & 18.657$\pm$0.146 & Mephisto & z \\
275.0074 & 18.958$\pm$0.073 & Mephisto & v \\
275.5688 & 18.325$\pm$0.111 & PO & g \\
275.5718 & 18.133$\pm$0.103 & PO & g \\
275.5748 & 18.282$\pm$0.114 & PO & g \\
275.5778 & 18.287$\pm$0.108 & PO & g \\
275.5808 & 18.194$\pm$0.101 & PO & g \\
275.5838 & 18.088$\pm$0.097 & PO & g \\
275.5871 & 18.059$\pm$0.100 & PO & r \\
275.5901 & 18.004$\pm$0.093 & PO & r \\
275.5931 & 18.028$\pm$0.100 & PO & r \\
275.5961 & 18.452$\pm$0.131 & PO & r \\
275.5991 & 18.235$\pm$0.112 & PO & r \\
275.6021 & 17.861$\pm$0.098 & PO & r \\
276.5664 & 18.212$\pm$0.114 & PO & r \\
276.5694 & 18.084$\pm$0.136 & PO & r \\
276.5724 & 18.083$\pm$0.115 & PO & r \\
276.5754 & 18.232$\pm$0.116 & PO & r \\
276.5784 & 18.669$\pm$0.172 & PO & r \\
276.5814 & 18.409$\pm$0.156 & PO & r \\
276.5845 & 18.472$\pm$0.176 & PO & g \\
276.5876 & 18.363$\pm$0.127 & PO & g \\
276.5907 & 18.303$\pm$0.123 & PO & g \\
276.5937 & 18.674$\pm$0.169 & PO & g \\
276.5967 & 18.268$\pm$0.120 & PO & g \\
276.5996 & 18.219$\pm$0.119 & PO & g \\
277.5667 & 18.327$\pm$0.125 & PO & g \\
277.5697 & 18.459$\pm$0.125 & PO & g \\
277.5727 & 18.347$\pm$0.120 & PO & g \\
277.5757 & 18.298$\pm$0.113 & PO & g \\
277.5787 & 18.113$\pm$0.101 & PO & g \\
278.5667 & 18.239$\pm$0.114 & PO & g \\
278.5697 & 18.594$\pm$0.140 & PO & g \\
278.5727 & 18.668$\pm$0.150 & PO & g \\
278.5757 & 18.632$\pm$0.158 & PO & g \\
278.5787 & 18.440$\pm$0.132 & PO & g \\
279.0017 & 19.693$\pm$0.146 & Mephisto & v \\
279.0017 & 18.220$\pm$0.096 & Mephisto & z \\
279.0068 & 19.889$\pm$0.122 & Mephisto & u \\
279.0068 & 17.535$\pm$0.032 & Mephisto & i \\
279.9991 & 20.190$\pm$0.188 & Mephisto & u \\
279.9991 & 17.792$\pm$0.019 & Mephisto & i \\
280.0042 & 19.431$\pm$0.113 & Mephisto & v \\
280.0042 & 18.932$\pm$0.183 & Mephisto & z \\
280.5673 & 18.744$\pm$0.214 & PO & g \\
280.5703 & 18.905$\pm$0.209 & PO & g \\
280.5733 & 18.473$\pm$0.147 & PO & g \\
280.5763 & 18.449$\pm$0.170 & PO & g \\
280.5795 & 19.048$\pm$0.208 & PO & g \\
281.5671 & 19.196$\pm$0.305 & PO & g \\
281.5701 & 18.581$\pm$0.170 & PO & g \\
281.5731 & 18.800$\pm$0.184 & PO & g \\
281.5761 & 19.051$\pm$0.225 & PO & g \\
281.5791 & 18.826$\pm$0.207 & PO & g \\
282.5708 & 18.916$\pm$0.208 & PO & r \\
282.5737 & 18.985$\pm$0.228 & PO & r \\
282.5767 & 18.843$\pm$0.185 & PO & r \\
282.5798 & 19.247$\pm$0.209 & PO & g \\
282.5828 & 19.703$\pm$0.295 & PO & g \\
282.5858 & 19.787$\pm$0.415 & PO & g \\
283.6109 & 18.520$\pm$0.153 & P60 & r \\
283.6178 & 18.825$\pm$0.164 & P60 & i \\
284.5707 & 19.293$\pm$0.221 & PO & g \\
284.5737 & 19.869$\pm$0.315 & PO & g \\
284.5767 & 19.908$\pm$0.321 & PO & g \\
285.6121 & 19.400$\pm$0.321 & P60 & r \\
286.5707 & 20.520$\pm$0.745 & PO & g \\
286.5737 & 20.083$\pm$0.433 & PO & g \\
286.5767 & 19.875$\pm$0.269 & PO & g \\
288.5742 & 20.129$\pm$0.457 & PO & g \\
290.5743 & 20.178$\pm$0.698 & PO & r \\
290.5773 & 20.331$\pm$0.616 & PO & r \\
290.5803 & 19.757$\pm$0.362 & PO & r \\
\end{tabular}
\end{table}


==> tables/sn2022jli_phot_short.tex <==
\begin{deluxetable}{cccc}
\tablecaption{SN\,2022jli photometry}
\tablehead{\colhead{Epoch} & \colhead{AB Magnitude} & \colhead{Source } & \colhead{Filter}
\\ (JD-2,459,700) &  & & }
\tabletypesize{\footnotesize}  %\small
\tablewidth{0pt}
\startdata
8.9154 & 15.366$\pm$0.053 & ASAS-SN & g \\
12.6611 & 15.386$\pm$0.053 & ASAS-SN & g \\
14.6775 & 15.602$\pm$0.171 & ASAS-SN & g \\
16.6692 & 15.737$\pm$0.120 & ASAS-SN & g \\
22.8739 & 15.477$\pm$0.060 & ASAS-SN & g \\
25.6585 & 14.786$\pm$0.007 & ATLAS & o \\
25.6657 & 14.775$\pm$0.007 & ATLAS & o \\
25.6826 & 14.796$\pm$0.012 & ATLAS & o \\
27.6503 & 16.140$\pm$0.113 & ASAS-SN & g \\
31.6665 & 16.245$\pm$0.078 & ASAS-SN & g \\
33.0868 & 15.751$\pm$0.013 & ATLAS & c \\
33.0953 & 15.696$\pm$0.011 & ATLAS & c \\
33.1092 & 15.707$\pm$0.013 & ATLAS & c \\
33.1134 & 15.718$\pm$0.017 & ATLAS & c \\
33.6136 & 16.092$\pm$0.063 & ASAS-SN & g \\
34.6683 & 16.324$\pm$0.125 & ASAS-SN & g \\
35.6096 & 16.005$\pm$0.082 & ASAS-SN & g \\
37.0850 & 15.568$\pm$0.011 & ATLAS & c \\
37.1016 & 15.540$\pm$0.011 & ATLAS & c \\
37.1042 & 15.920$\pm$0.072 & ASAS-SN & g \\
37.1044 & 15.529$\pm$0.010 & ATLAS & c \\
37.1150 & 15.579$\pm$0.018 & ATLAS & c \\
37.6023 & 15.944$\pm$0.066 & ASAS-SN & g \\
37.6553 & 14.867$\pm$0.007 & ATLAS & o \\
37.6739 & 14.861$\pm$0.008 & ATLAS & o \\
37.6854 & 14.882$\pm$0.015 & ATLAS & o \\
38.8515 & 15.774$\pm$0.051 & ASAS-SN & g \\
41.5805 & 15.720$\pm$0.053 & ASAS-SN & g \\
42.9147 & 15.482$\pm$0.039 & ASAS-SN & g \\
45.0839 & 14.578$\pm$0.009 & ATLAS & o \\
45.0959 & 14.517$\pm$0.009 & ATLAS & o \\
45.1065 & 14.563$\pm$0.008 & ATLAS & o \\
45.1101 & 14.538$\pm$0.008 & ATLAS & o \\
47.0924 & 14.489$\pm$0.009 & ATLAS & o \\
47.0965 & 14.520$\pm$0.009 & ATLAS & o \\
47.1034 & 14.494$\pm$0.008 & ATLAS & o \\
47.1159 & 14.496$\pm$0.019 & ATLAS & o \\
47.8300 & 15.275$\pm$0.047 & ASAS-SN & g \\
49.8793 & 15.202$\pm$0.049 & ASAS-SN & g \\
54.0836 & 14.482$\pm$0.005 & ATLAS & o \\
54.0868 & 14.464$\pm$0.006 & ATLAS & o \\
54.0966 & 14.463$\pm$0.005 & ATLAS & o \\
54.1023 & 14.454$\pm$0.005 & ATLAS & o \\
55.0878 & 14.434$\pm$0.006 & ATLAS & o \\
55.0925 & 14.483$\pm$0.006 & ATLAS & o \\
55.1004 & 14.475$\pm$0.006 & ATLAS & o \\
55.1018 & 14.464$\pm$0.006 & ATLAS & o \\
55.1105 & 14.455$\pm$0.006 & ATLAS & o \\
55.1119 & 14.427$\pm$0.006 & ATLAS & o \\
55.1183 & 14.481$\pm$0.009 & ATLAS & o \\
55.1197 & 14.467$\pm$0.011 & ATLAS & o \\
57.9530 & 15.244$\pm$0.024 & ZTF & g \\
57.9530 & 15.244$\pm$0.024 & ZTF & g \\
57.9540 & 15.220$\pm$0.029 & ZTF & g \\
57.9540 & 15.220$\pm$0.029 & ZTF & g \\
57.9540 & 15.220$\pm$0.029 & ZTF & g \\
58.9335 & 15.217$\pm$0.035 & ASAS-SN & g \\
\enddata
\label{tab:phot}
\tablecomments{Only part of the photometry is shown here for guidance regarding the form and content of the table.}
\end{deluxetable}

==> tables/spec_log.tex <==
\begin{deluxetable}{lcccc}
\tablecaption{Summary of Spectroscopic Observations of SN\,2022jli}
%\tablecolumns{5}
\tabletypesize{\footnotesize}  %\small
\tablewidth{0pt}
\tablehead{
\colhead{Date (UTC)} &
\colhead{Phase (d)} &
\colhead{Telescope} &
\colhead{Spectrograph} &
\colhead{Exp (s)}
}
\startdata 
2022-06-29.423 &  55.254 &       P60 &       SEDM &    1800 \\
2022-07-07.424 &  63.254 &       P60 &       SEDM &    1800 \\
2022-07-19.453 &  75.284 &       P60 &       SEDM &    1800 \\
2022-07-26.338 &  82.169 &       P60 &       SEDM &    1800 \\
2022-08-04.418 &  91.249 &       P60 &       SEDM &    1800 \\
2022-08-06.196 &  93.027 &       NOT &     ALFOSC &     600 \\
2022-08-11.310 &  98.141 &       P60 &       SEDM &    1800 \\
2022-08-16.288 & 103.119 &       P60 &       SEDM &    1800 \\
2022-08-18.325 & 105.155 &       P60 &       SEDM &    1800 \\
  2022-08-20.0 & 106.830 &      P200 &       DBSP &     300 \\
2022-08-23.371 & 110.202 &       P60 &       SEDM &    1800 \\
2022-08-26.824 & 113.154 &  Magellan &       FIRE &    507  \\
2022-08-28.254 & 115.084 &       P60 &       SEDM &    1800 \\
2022-09-08.387 & 126.217 &       P60 &       SEDM &    1800 \\
2022-09-16.216 & 134.046 &       P60 &       SEDM &    1800 \\
2022-09-21.221 & 139.052 &       NOT &     ALFOSC &     1200 \\
2022-10-02.305 & 150.136 &       P60 &       SEDM &    1800 \\
2022-10-05.149 & 152.980 &       P60 &       SEDM &    1800 \\
2022-10-11.159 & 158.989 &       P60 &       SEDM &    1800 \\
2022-10-11.274 & 159.104 &      P200 &       DBSP &    600 \\
2022-10-14.199 & 162.029 &       P60 &       SEDM &    1800 \\
2022-10-21.179 & 169.009 &       P60 &       SEDM &    1800 \\
2022-10-22.372 & 170.202 &       P60 &       SEDM &    1800 \\
2022-10-30.337 & 178.168 &       P60 &       SEDM &    1800 \\
2022-10-31.997 & 179.828 &       NOT &     ALFOSC &    1200 \\
  2022-11-02.0 & 180.830 &      P200 &       DBSP &     420 \\
2022-11-15.133 & 193.964 &       P60 &       SEDM &    1800 \\
  2022-11-25.1 & 203.831 &       NOT &     ALFOSC &    1200 \\
 2022-11-27.78 & 205.909 &       P60 &       SEDM &    1800 \\
 2022-12-11.119 & 219.949 &      P60 &       SEDM &    1800 \\
2022-12-15.137 & 223.967 & Magellan &      IMACS &     900 \\
2022-12-15.560 & 223.890 & Magellan &       FIRE &     2832\\ % 4*708
 2022-12-20.98 & 228.929 &      P60 &       SEDM &    1800 \\
 2022-12-27.91 & 235.921 &      MMT &   BINOSPEC &    2400 \\
 2023-01-12.77 & 251.907 &      MMT &   BINOSPEC &     450 \\
 2023-01-13.71 & 252.902 &      MMT &   BINOSPEC &    1350 \\
2023-01-13.172 & 253.003 &      P60 &       SEDM &    1800 \\
 2023-01-14.50 & 253.881 &      VLT &   XSHOOTER &     900 \\
 2023-01-18.44 & 257.874 &      VLT &   XSHOOTER &     900 \\
 2023-01-21.45 & 260.875 &      VLT &   XSHOOTER &     900 \\
2023-01-21.111 & 260.941 &      MMT &   BINOSPEC &    1800 \\
 2023-01-22.90 & 261.921 &      MMT &   BINOSPEC &    2250 \\
 2023-01-31.89 & 270.920 &      MMT &   BINOSPEC &    1350 \\
2023-02-02.108 & 272.938 &      P60 &       SEDM &    1800 \\
2023-02-03.829 & 274.660 &      NOT &     ALFOSC &    1200 \\
2023-02-08.824 & 279.654 &      NOT &     ALFOSC &    1200 \\
\enddata
\label{tab:spec}
\tablecomments{The phase is calculated with respect to the discovery date of JD= 2459704.67.}
\end{deluxetable}

